Multi-AAV Cooperative Path Planning using Nonlinear Model Predictive Control with Localization Constraints

In this paper, we solve a joint cooperative localization and path planning problem for a group of Autonomous Aerial Vehicles (AAVs) in GPS-denied areas using nonlinear model predictive control (NMPC). A moving horizon estimator (MHE) is used to estimate the vehicle states with the help of relative bearing information to known landmarks and other vehicles. The goal of the NMPC is to devise optimal paths for each vehicle between a given source and destination while maintaining desired localization accuracy. Estimating localization covariance in the NMPC is computationally intensive, hence we develop an approximate analytical closed form expression based on the relationship between covariance and path lengths to landmarks. Using this expression while computing NMPC commands reduces the computational complexity significantly. We present numerical simulations to validate the proposed approach for different numbers of vehicles and landmark configurations. We also compare the results with EKF-based estimation to show the superiority of the proposed closed form approach.

==> Cooperative localization MPC/Introduction.tex <==
\section{Introduction}\label{sec:intro}
Urban air mobility (UAM) is expected to have highly automated, cooperative, passenger, and cargo-carrying aerial vehicles in urban areas \cite{faa}, and the use of autonomous aerial vehicles (AAVs) for various activities are expected to rise substantially in the near future \cite{sesar}. Cargo delivery drones operate in urban canyons with high-rise buildings and other obstructions, which calls for significant localization accuracy. However, operating in such environments pose an additional challenge in localization since Global navigation satellite systems (GNSS) are unreliable in such scenarios. A solution to this problem is to use alternate localization schemes such as relative localization \cite{betke1997mobile,thrun1998finding}, vision-based methods \cite{lategahn2014vision,kim2005vision}, and ultra-wide-band (UWB) localization schemes \cite{krishnan2007uwb,zhang2018linear}. As the urban airspace is expected to contain a large number of AAVs, relative localization between vehicles can also be used in addition to localization with respect to known landmarks. 

Cooperative path planning with localization constraints involves the following components: (i) localization -- vehicles estimate their position by using relative measurements obtained with respect to other vehicles or landmarks, and (ii) cooperative path planning -- localization constraints have to be considered while planning the optimal path from source to destination, and hence the agents must cooperate with each other to  generate motion commands that  improve the localization accuracy of the entire group while reducing the path length to reach their destination. Several works have studied the problem separately. For instance, \cite{Kurazume1998,Roumeliotis2000,Spletzer2001,Mourikis2006,Nerurkar2009,wan2014cooperative,minaeian2016vision,frohle2018cooperative,pierre2018range,liu2018multi,guo2019ultra,zhu2019cooperative} on cooperative localization and \cite{zheng2005evolutionary,Agha-Mohammadi2014,Mathew2015,mac2016heuristic} on path planning. However, the collection of works on cooperative path planning with the localization constraints is limited, which we will review below.

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
		\caption{}
		\label{fig:scenario}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
		\caption{}
		\label{fig:rpmg}
	\end{subfigure}\hfil 
	\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
	\label{fig:path_graph}
\end{figure}  

Bopardikar et al.~\cite{bopardikar2015multiobjective} presented a graph-based probabilistic roadmap approach to tackle the path planning problem subject to localization constraints. A time-optimal path planner satisfying the covariance bounds was given in \cite{singh2016landmarks} using a swarm optimization technique coupled with a rabbit-carrot based path follower. An approach to optimally place landmarks to satisfy localization constraints was proposed in \cite{sundar2019path}. The algorithm computes an optimal path for the vehicle and the locations where the landmarks should be placed. A localizability constrained path planning method for autonomous vehicles which takes into account the laser range finder (LRF) sensor model of the vehicle is proposed in \cite{irani2018localizability} to maintain a satisfactory level of localizability throughout the path. Kassas et al. \cite{kassas2021uav} present a multi-objective motion planning algorithm in which the vehicle tries to balance the objectives of navigating to the waypoint and reducing its position estimate uncertainty. In \cite{manoharan2019nonlinear}, a nonlinear model predictive control scheme was used to find optimal paths that ensured the required localization accuracy for a group of cooperative UAVs without analysis.

Urban air mobility calls for improved localization accuracy due to its innate nature involving close structures, narrow pathways, and a large number of vehicles. Moving horizon estimation (MHE) has been suggested as an alternate to EKF for increasing the accuracy of nonlinear estimation problems by \cite{rawlings2006particle,wang2014optimization,mehrez2017optimization}. Erunsal et al. \cite{erunsal2019decentralized} proposed an approach combining NMPC and pose-graph-MHE for 3D formation control of micro aerial vehicles with relative sensing capability. In \cite{liu2020decentralized}, a decentralized MHE technique is proposed for networked navigation with packet dropouts.    

In this paper, we extend the  work in ~\cite{manoharan2019nonlinear} and propose a complete cooperative localization and path planning framework with moving horizon estimation (MHE) for estimating the vehicle position, and a nonlinear model predictive control (NMPC) framework for cooperative path planning, and a closed formulation for covariance calculation to  predicting the uncertainty. This framework uses a nonlinear vehicle model in both the controller and the estimator, which mitigates the linearization errors. The analytical expression used for the covariance calculation speeds up the computations and is derived by exploiting the relationship between the vehicle-landmark path lengths to the localization uncertainty. In most of the literature for multi-agent systems, the studies are formulated either as a control problem or an estimation problem \cite{Mourikis2006,Nerurkar2009,Roumeliotis2000,wan2014cooperative,wang2014optimization}. We propose a method that combines both and looks at the multi-agent problem in a holistic sense.

Previous studies \cite{Agha-Mohammadi2014,Mathew2015,wan2014cooperative} used algorithms that were not optimal and were based on conventional path planners, whereas nonlinear model predictive control (NMPC) provides optimal paths while satisfying imposed state and input constraints. The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. Also, most of the works based on graph-based planning give discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, eliminating the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2006maximizing} and \cite{de2006decentralized}. We also use a Laplacian matrix based solution, but we calculate Laplacian matrices for each vehicle instead of forming a single matrix for the whole group. This helps in identifying connectivity at an individual level, and each vehicle can decide to maintain, lose, or gain connections depending on their covariance estimates. This is not possible in the single matrix case because a single vehicle with more connections will increase the Laplacian, even though the other vehicles may be out of the required number of connections. 
Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy. The works on path planning with localization constraints \cite{singh2016landmarks,sundar2019path,kassas2021uav,irani2018localizability} consider only single vehicles and fixed landmarks in most cases, whereas our approach includes multiple vehicles, and each vehicle is considered a moving landmark. Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobians, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. Now, we can summarize the major contributions of this paper as follows:
\begin{itemize}
	\item A complete framework for control and estimation of multi-vehicle cooperative path planning problem with localization constraints using NMPC and MHE.
	\item An analysis on the relation of path lengths between vehicles and landmarks on the estimation covariance, from which an approximate expression for predicting the uncertainty was derived.
\end{itemize}

The rest of the paper is organized as follows. The problem formulation is given in Section \ref{sec:problem}. Moving horizon estimation (MHE) is explained in Section \ref{sec:MHE}. The derivation of the analytic expression for covariance is given in Section \ref{sec:analysis}. The NMPC formulation is given in Section \ref{sec:NMPC}. Simulation results are presented in Section \ref{sec:results}, and the conclusions are given in Section \ref{sec:conclusions}. 

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%	\caption{Block diagram showing the proposed NMPC-MHE control scheme.}
%	\label{fig:block}
%\end{figure} 

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=8cm]{figs/BlockDiagram.eps}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=8cm]{figs/covariance.eps}		
	\end{subfigure}\hfil 
	\caption{Block diagram and a graphical representation of the proposed NMPC-MHE control scheme. }
	\label{fig:block}
\end{figure}  

\section{Problem formulation}\label{sec:problem}	
%Around-the-clock delivery of essential supplies like medicines from one location to another is an important application of autonomous aerial vehicles \cite{ups2}. 
We consider a scenario where a group of AAVs need to navigate from their source location ($S$) to destination ($D$), as shown in Fig.~\ref{fig:scenario}. These vehicles need to transit in a GPS-denied area and we assume that any kind of GNSS are not available. In such scenarios, known landmarks or other vehicles in the area can be used for relative localization using range or bearing measurements. This structure involving landmarks and vehicles can be modeled as a dynamic relative position measurement graph (RPMG) \cite{sharma2011graph} with vehicles and landmarks as nodes and connections/measurements as edges.
\begin{definition}
	A relative position measurement graph (RPMG) for $n_v(t)$ vehicles with $n_l(t)$ landmarks is a graph $G_{n_v}^{n_l}(t)~\triangleq~\{\mathcal{V}_{n_v}^{n_l}(t),\mathcal{E}_{n_v}^{n_l}(t) \}$, where $\mathcal{V}_{n_v}^{n_l}$ is the node set consisting of $n_v(t)$ vehicle nodes and $n_l(t)$ landmark nodes (which makes a total of $n_v(t)+n_l(t)$ nodes), and $\mathcal{E}_{n_v}^{n_l}(t)$ is the edge set representing available relative measurements. The number of edges is denoted by $n_e(t)= |\mathcal{E}_{n_v}^{n_l}(t)|$.   
\end{definition}
\begin{definition}
	A path from a vehicle node to a landmark node is a finite sequence of edges which joins a sequence of distinct vertices between them. Let $\mathcal{G} \triangleq \{\mathcal{V},\mathcal{E},\phi\} $ be a graph. A path $\phi$ from vertex $i$ to vertex $j$ is a sequence of edges $\{\epsilon_1,\epsilon_2, \ldots, \epsilon_{n-1} \}$ for which there is a sequence of distinct vertices $\{\nu_1,\nu_2, \ldots, \nu_n \}$ such that $\phi \triangleq \{ \nu_1,\nu_n \}$ where $\nu_1 = i$ and $\nu_n = j$.
\end{definition}
An example RPMG ($G_{5}^{3}$ with $n_e=7$) is shown in Fig.~\ref{fig:rpmg}. A path from the vehicle $5$ to the landmark $a$ is represented by the edge set $\phi \triangleq \{\epsilon_6,\epsilon_5,\epsilon_3 \}$ which can also be represented using the vertices as $5-4-2-a$. 

Previous studies show that for cooperative localization to work, each vehicle should have a direct or indirect path to at least two known landmarks \cite{sharma2014observability}. This condition is very limiting in environments with a low number of landmarks. Hence in this paper, we find a relationship between vehicle uncertainty and path length to the landmarks and then use that relationship to formulate and solve an NMPC problem to guarantee that the covariance does not exceed a specified threshold and desired localization accuracy is achieved while performing individual missions. A moving horizon estimation (MHE) scheme is used to estimate the vehicle states. A block diagram and a graphical representation of the proposed solution using nonlinear model predictive control (NMPC) combined with MHE to tackle the cooperative localization and path planning problem is shown in Fig.~\ref{fig:block}. The optimal path is different from the shortest path since the latter does not satisfy localization constraints. The components of the block diagram are explained in the subsequent sections. In the first step of the control scheme, vehicle states are estimated by the MHE block using available measurements from the sensors (Sec.~\ref{sec:MHE}). The second step is the calculation of estimation covariances for the NMPC prediction window, which is accomplished by the covariance calculator block that contains the derived analytical expression (Sec.~\ref{sec:analysis}). In the third and final step, the NMPC controller computes the control actions for the vehicles (Sec.~\ref{sec:NMPC}). 


% 	\begin{figure}
	% 		\centering
	% 		\includegraphics[width=8cm]{figs/coop_scenario.eps}
	% 		\caption{Path planning scenario. }
	% 		\label{fig:scenario}
	% 	\end{figure}

%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
	%		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
	%		\caption{}
	%		\label{fig:scenario}
	%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
	%		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
	%		\caption{}
	%		\label{fig:rpmg}
	%	\end{subfigure}\hfil 
%		\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
%		\label{fig:path_graph}
%\end{figure}  

==> Cooperative localization MPC/Introduction_old.tex <==
\section{Introduction}\label{sec:intro}
Urban air mobility (UAM) deals with highly automated, cooperative, passenger, and cargo-carrying aerial vehicles in urban areas \cite{faa}. Major companies like UPS \cite{ups1}, DHL \cite{dhl}, Amazon \cite{prime}, and Wing \cite{wing} are developing autonomous transportation systems for delivering cargo and medicines.
% Uber \cite{uber} and Airbus \cite{airbus} are working on autonomous aerial systems that can transport people. 
The use of autonomous aerial vehicles (AAVs) for various activities is expected to rise substantially in the near future \cite{sesar}.   

AAVs depend on Global navigation satellite systems (GNSS) for localization. However, there are situations in which GNSS is either unreliable or unavailable, such as urban canyon environments, intentional denial/jamming
of GNSS services \cite{van1996selective}, etc. In such scenarios, alternative localization schemes such as relative localization with respect to known landmarks \cite{betke1997mobile,thrun1998finding}, vision-based localization schemes \cite{lategahn2014vision,kim2005vision}, radio-frequency (RF), and ultra-wide-band (UWB) based methods \cite{seco2016robot,krishnan2007uwb,zhang2018linear}, and techniques using lidar \cite{xu2019indoor,wang2020intelligent,levinson2010robust} become important for AAVs to accomplish their tasks. The urban airspace is expected to contain a large number of AAVs, making the multi-vehicle localization and path planning a challenging task. Cooperative localization for multiple vehicles and path planning for a single vehicle with localization constraints have been studied~\cite{Kurazume1998,Roumeliotis2000,Spletzer2001,minaeian2016vision,sundar2019path,zheng2005evolutionary,mac2016heuristic}. However, cooperative path planning with localization constraints for multiple vehicles has not been adequately addressed in the literature.

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=0.45\linewidth]{figs/coop_scenario.eps}
		\caption{}
		\label{fig:scenario}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=0.45\linewidth]{figs/rpmg.eps}		
		\caption{}
		\label{fig:rpmg}
	\end{subfigure}
	\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
	\label{fig:path_graph}
\end{figure}  

In Cooperative localization, the agents localize using measurements obtained with respect to other agents or known features. The agents move in such a fashion as to help each other and improve the localization accuracy of the entire group. This idea has been studied by several researchers for the past decade and different techniques like treating the other agents as moving landmarks \cite{Kurazume1998,Roumeliotis2000,Spletzer2001,minaeian2016vision}, using features in the environment \cite{frohle2018cooperative}, and combining both static and moving objects for relative measurements \cite{pierre2018range} have been employed to achieve cooperative localization. Kurazume and Hirose \cite{Kurazume1998} proposed a localization scheme for multi-robot systems in which the robots alternatively act as landmarks and moving agents. When one group is in motion, the other group remains stationary and acts as landmarks for the other group. Roumeliotis and Bekey \cite{Roumeliotis2000} used a decentralized Kalman filter to optimally combine sensor information from each robot to localize a group of cooperative robots moving in a given space.
% Vision-based techniques were used in \cite{Spletzer2001} to localize a group of robots moving in a formation. 
Minaeian et al. \cite{minaeian2016vision} used a vision-based localization system for target detection and tracking. The formulation involves AAVs and ground vehicles in which the latter is used as moving landmarks for localizing the AAVs.
% Koohifar et al. \cite{koohifar2017receding} used a receding horizon scheme, which employs the Fisher information matrix to localize a moving target using AAVs. In \cite{frohle2018cooperative}, a cooperative localization method without explicit inter-vehicle measurements is proposed, where vehicles track mobile features in the environment to improve localization accuracy. 
% The papers \cite{liu2018multi,pierre2018range} proposed a cooperative localization algorithm based on range measurements using ultra wide band (UWB) sensors, where \cite{liu2018multi} used EKF for estimation, and in \cite{pierre2018range}, every static or mobile object was considered beacons for localization, and a split intersection covariance filter was used to estimate the poses. 
In \cite{liu2018multi}, a cooperative localization algorithm based on range measurements using ultra wide band (UWB) sensors and EKF for estimation is developed. In \cite{guo2019ultra}, a cooperative relative localization technique for AAVs based on UWB and odometry is proposed for multi-AAV formation control. An approach for cooperative localization under limited connectivity for multi-agent systems is given in \cite{zhu2019cooperative}. Each agent localizes in a global frame using a local filter, which uses local dead reckoning and intermittent absolute measurement updates and corrects its pose estimate whenever relative measurements with respect to
other agents are received. Rathinam and Sharma \cite{Rathinam2015}, and Wang et al. \cite{wang2019landmark} proposed an approach to optimally place landmarks to aid cooperative localization. The path from the source to the goal is fixed, and the algorithm is used to place the minimum number of landmarks along the way to achieve the required localization accuracy. In \cite{Mourikis2006}, the accuracy of position estimation
for groups of mobile robots performing cooperative localization is studied. The analysis is based on the eigenvalues of the relative position measurement graph (RPMG) of the system. 
% In \cite{piperigkos2020graph}, a graph-based cooperative localization scheme is given for semi-autonomous vehicles.
% The network of cars is modeled as an undirected relative position graph, and the solution is based on the Laplacian method. Our approach is also based on the relative position measurement graph, with relative bearing measurements obtained from vehicles and landmarks. But, instead of using a single adjacency matrix and Laplacian for all the vehicles, we define individual adjacency matrices for each vehicle. This helps in identifying connectivity at individual level, and each vehicle can decide to maintain, loose or gain connections depending on their covariance estimates. This is not possible in the single matrix case, because a single vehicle with more number of connections will increase the Laplacian, even though the other vehicles maybe out of required number of connections. 
 
% Previous studies on path planning were mainly based on genetic algorithms \cite{ismail2008mobile,dai2009path,albab2017path,panda2015effective,lu2016path,germi2018adaptive,roberge2012comparison}, artificial potential fields \cite{rimon1992exact,barraquand1992numerical,ge2000new,chen2016uav}, rapidly-exploring random trees (RRT) \cite{kuffner2000rrt}, and A* methods \cite{dolgov2010path,wang2018partitioning}. Kavraki et al. \cite{kavraki1996probabilistic} gave a solution based on probabilistic road-maps for path planning of holonomic robots. A broad survey on classical and heuristic path planning techniques is given in \cite{mac2016heuristic}.

%Sundar et al. \cite{sundar2019path} presented a path planning algorithm with localization constraints which ensured the vehicle is always connected to the required number of landmarks for localization. Scenarios involving multiple vehicles pose additional constraints/opportunities in the path planning problem, such as keeping a formation while in transit. Sometimes, vehicles need to maintain connections for information sharing or do cooperative tasks that a single vehicle cannot achieve.      
 
After the vehicle is accurately localized, the next challenge in urban mobility is planning the optimal path from one point to another. In \cite{Agha-Mohammadi2014,Mathew2015,bopardikar2015multiobjective}, the AAV transportation problem where the vehicles move between waypoints subject to different constraints were studied. Agha-Mohammadi et al.~\cite{Agha-Mohammadi2014} used graph based methods and forward search to generate real-time policies for the delivery drones, Mathew et al.~\cite{Mathew2015} proposed a solution using a novel reduction to the generalized traveling salesman problem, and Bopardikar et al.~\cite{bopardikar2015multiobjective} presented a graph-based probabilistic roadmap approach to tackle the multi-agent path planning problem.  
% Yun et al. \cite{Yun2013} also formulated an integrated navigation system to tackle the unavailability of GNSS by combining various sensor measurements. Another strategy for localization without GPS is given in \cite{wan2014cooperative}, where the AAVs exchanged relative range measurement information, and a posterior distribution was calculated using a dynamic nonparametric belief propagation (DNBP) scheme. In \cite{he2008planning}, a belief road map (BRM) algorithm was used to plan trajectories for a quadcopter without GPS. In \cite{zheng2005evolutionary}, a genetic algorithm-based route planner is proposed for cooperative path planning of AAVs.     

% Cooperative multi-agent algorithms need connectivity between agents for measurements, which is not easy to maintain over time due to constraints such as sensor range and goal-reaching objective. In \cite{kim2005maximizing}, an algorithm for maximizing the second smallest eigenvalue (algebraic connectivity) of the proximity graph Laplacian for multi-agent systems was proposed. A similar approach based on algebraic connectivity was proposed in \cite{de2006decentralized} to increase the connectivity of a multi-robot system. A decentralized potential-based control law was used to achieve the inter-robot distances dictated by a supergradient
% algorithm.
 
% Another critical aspect of the cooperative estimation problem is to satisfy the conditions for observability of the system. Perera et al. \cite{Perera2009} provide rigorous proofs for the observability properties of the general two dimensional SLAM problem with a number of landmarks in the context of piece-wise constant systems theory and non-linear Lie derivative theory. Yu et al.~\cite{yu2011observability} proposed an observability-based path planning algorithm for AAV navigation with obstacle avoidance. A nonlinear observability analysis was performed to obtain the necessary conditions for complete observability of the system, and these conditions were used to explicitly design a path that enhances observability while simultaneously avoiding collisions with obstacles.   
 
Urban air mobility calls for improved localization accuracy due to its innate nature involving close structures, narrow pathways, and a large number of vehicles. Moving horizon estimation (MHE) has been suggested as an alternate to EKF for increasing the accuracy of nonlinear estimation problems by \cite{rawlings2006particle,wang2014optimization,kayacan2014learning,mehrez2017optimization}.
% with \cite{wang2014optimization} proposing a cooperative localization approach for autonomous underwater vehicles, and \cite{mehrez2017optimization} for multi-robot systems.
Erunsal et al. \cite{erunsal2019decentralized} proposed an approach combining NMPC and pose-graph-MHE for 3D formation control of micro aerial vehicles with relative sensing capability. In \cite{liu2020decentralized}, a decentralized MHE technique is proposed for networked navigation with packet dropouts.    

% Cooperative localization with multiple vehicles and path planning with localization constraints is not adequately addressed in the literature. 
In this paper, we extend our work presented in \cite{manoharan2019nonlinear} on cooperative localization and path planning using NMPC by combining a moving horizon estimation (MHE) scheme for determining the vehicle states. Through this mechanism, the nonlinear vehicle model can be used on both the controller and the estimator, while mitigating linearization errors. Also, we replace the covariance calculation using the EKF-update with an analytical expression derived by exploiting the relationship between the vehicle-landmark path lengths to the localization uncertainty to speed up the computations. In most of the literature for multi-agent systems, the studies are formulated either as a control problem or an estimation problem \cite{Mourikis2006,Nerurkar2009,Roumeliotis2000,wan2014cooperative,wang2014optimization,brinon2014cooperative,shi2015cooperative,dong2008cooperative,khazaeni2016event,movric2013cooperative}. We propose a method that combines both and tries to look at the multi-agent problem in a holistic sense. Also, model predictive control is generally used to track a reference created using an auxiliary path planner. In contrast, we try to exploit the full potential of the NMPC as a planner and a controller without using any low-level controllers or auxiliary path planners. 
 
Previous studies \cite{Agha-Mohammadi2014,Mathew2015,Rathinam2015,Yun2013,wan2014cooperative} used algorithms that are not optimal and were based on conventional path planners, whereas nonlinear model predictive control (NMPC) provides optimal paths while satisfying imposed state and input constraints. The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. Also, most of the works based on graph-based planning gives discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, which eliminates the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2005maximizing} and \cite{de2006decentralized}. We also use a graph-based solution, but with smaller sub-graphs instead of a single graph. This helps in identifying connectivity at individual level, and each vehicle can decide to maintain, loose or gain connections depending on their covariance estimates. This is not possible in the single matrix case, because a single vehicle with more number of connections will increase the Laplacian, even though the other vehicles maybe out of required number of connections. 
Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{Rathinam2015,wang2019landmark,sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy.         

Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobians, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. 
The rest of the paper is organized as follows. The problem formulation is given in Section \ref{sec:problem}. Moving horizon estimation (MHE) is explained in Section \ref{sec:MHE}. The derivation of the analytic expression for covariance is given in Section \ref{sec:analysis}. The NMPC formulation is given in Section \ref{sec:NMPC}. Simulation results are presented in Section \ref{sec:results}, and the conclusions are given in Section \ref{sec:conclusions}. 

	\begin{figure}[h]
	\centering
	\includegraphics[width=8cm]{figs/BlockDiagram.eps}
	\caption{Block diagram showing the proposed NMPC-MHE control scheme.}
	\label{fig:block}
\end{figure} 

\section{Problem formulation}\label{sec:problem}	
%Around-the-clock delivery of essential supplies like medicines from one location to another is an important application of autonomous aerial vehicles \cite{ups2}. 
We consider a scenario where a group of AAVs need to navigate from their source location ($S$) to destination ($D$), as shown in Fig.~\ref{fig:scenario}. These vehicles need to transit in a GPS-denied area and we assume that any kind of GNSS are not available. In such scenarios, known landmarks or other vehicles in the area can be used for relative localization using range or bearing measurements. This structure involving landmarks and vehicles can be modeled as a dynamic relative position measurement graph (RPMG) \cite{sharma2011graph} with vehicles and landmarks as nodes and connections/measurements as edges.
\begin{definition}
A relative position measurement graph (RPMG) for $n_v(t)$ vehicles with $n_l(t)$ landmarks is a graph $G_{n_v}^{n_l}(t)~\triangleq~\{\mathcal{V}_{n_v}^{n_l}(t),\mathcal{E}_{n_v}^{n_l}(t) \}$, where $\mathcal{V}_{n_v}^{n_l}$ is the node set consisting of $n_v(t)$ vehicle nodes and $n_l(t)$ landmark nodes (which makes a total of $n_v(t)+n_l(t)$ nodes), and $\mathcal{E}_{n_v}^{n_l}(t)$ is the edge set representing available relative measurements. The number of edges is denoted by $n_e(t)= |\mathcal{E}_{n_v}^{n_l}(t)|$.   
\end{definition}
\begin{definition}
A path from a vehicle node to a landmark node is a finite sequence of edges which joins a sequence of distinct vertices between them. Let $\mathcal{G} \triangleq \{\mathcal{V},\mathcal{E},\phi\} $ be a graph. A path $\phi$ from vertex $i$ to vertex $j$ is a sequence of edges $\{\epsilon_1,\epsilon_2, \ldots, \epsilon_{n-1} \}$ for which there is a sequence of distinct vertices $\{\nu_1,\nu_2, \ldots, \nu_n \}$ such that $\phi \triangleq \{ \nu_1,\nu_n \}$ where $\nu_1 = i$ and $\nu_n = j$.
\end{definition}
An example RPMG ($G_{5}^{3}$ with $n_e=7$) is shown in Fig.~\ref{fig:rpmg}. A path from the vehicle $5$ to the landmark $a$ is represented by the edge set $\phi \triangleq \{\epsilon_6,\epsilon_5,\epsilon_3 \}$ which can also be represented using the vertices as $5-4-2-a$. 

Previous studies show that for cooperative localization to work, each vehicle should have a direct or indirect path to at least two known landmarks \cite{sharma2014observability}. This condition is very limiting in environments with a low number of landmarks. Hence in this paper, we find a relationship between vehicle uncertainty and path length to the landmarks and then use that relationship to formulate and solve an NMPC problem to guarantee that the covariance does not go beyond a specified threshold and desired localization accuracy is achieved while performing individual missions. A moving horizon estimation (MHE) scheme is used to estimate the vehicle states. A block diagram of the proposed solution using nonlinear model predictive control (NMPC) combined with MHE to tackle the cooperative path planning and localization problem is shown in Fig.~\ref{fig:block}, and is explained in the subsequent sections. In the first step of the control scheme, vehicle states are estimated by the MHE block using available measurements from the sensors (Sec.~\ref{sec:MHE}). Second step is the calculation of estimation covariances for the NMPC prediction window. This is accomplished by the covariance calculator block, which contains the derived analytical expression (Sec.~\ref{sec:analysis}). In the third and final step, the NMPC controller computes the control actions for the vehicles (Sec.~\ref{sec:NMPC}). 


% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/coop_scenario.eps}
% 		\caption{Path planning scenario. }
% 		\label{fig:scenario}
% 	\end{figure}

%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
%		\caption{}
%		\label{fig:scenario}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
%		\caption{}
%		\label{fig:rpmg}
%	\end{subfigure}\hfil 
%		\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
%		\label{fig:path_graph}
%\end{figure}  

==> Cooperative localization MPC/MHE.tex <==
\section{Moving horizon estimation}\label{sec:MHE}
Moving horizon estimation (MHE) uses optimization techniques to find state trajectories that best fit a series of measurements acquired over a finite time interval. It uses the exact nonlinear models of the available measurements and system dynamics for estimation. Also, there is another advantage of including the state/control constraints in the formulation, which helps in bounding the estimates. Like NMPC, MHE also has three main components, 1) an internal dynamic model of the process, 2) a history of past measurements, and 3) an optimization cost function over the estimation horizon.
%In MHE, an iterative approach based on linear or nonlinear programming is used to find the estimates. 
%MHE is superior to the extended Kalman filter (EKF), the most commonly used nonlinear estimator for multi-agent systems~\cite{haseltine2005critical} since the EKF linearizes nonlinear models at operating points.  
%Also, EKF is based on the Markov assumption that the current state estimate is based only on the most recent measurements and the previous state estimate. Since the MHE minimizes the deviation of the model from the past interval of measurements, the Markov assumption is relaxed.  

The model used for estimation is given as:
\begin{eqnarray}
X(k)&=&f\left( X(k-1),\boldsymbol{\omega}(k),k\right) +q(k), \label{eq:f}\\
z(k)&=&h\left( X(k),\boldsymbol{\omega}(k),k\right) + \mu(k), \label{eq:z}
\end{eqnarray}	
where, $f(\cdot)$ and $h(\cdot) $ represent the state model and the observation model respectively. ${X}(k)$ and $ z(k) $ are the system states and measurements at the $k^{\mathrm{th}}$ time instant. The vectors $ q(k) $ and $ \mu(k) $ are the process and measurement noises which are assumed to be additive and zero mean white Gaussian noises with covariance $ Q $ and $ \Gamma $ respectively. $ f(\cdot) $ is defined as
	\begin{equation}
	f=\begin{bmatrix}
	x_{1}(k)\\
	y_{1}(k)\\
	\psi_{1}(k)\\
	\vdots\\
	x_{n_v}(k)\\
	y_{n_v}(k)\\
	\psi_{n_v}(k)
	\end{bmatrix}=
	\begin{bmatrix}
	x_{1}(k-1)+T_sv\cos\psi_{1}(k-1)\\
	y_{1}(k-1)+T_sv\sin\psi_{1}(k-1)\\
	\psi_{1}(k-1)+T_s\omega_1(k-1)\\
	\vdots\\
	x_{n_v}(k-1)+T_sv\cos\psi_{n_v}(k-1)\\
	y_{n_v}(k-1)+T_sv\sin\psi_{n_v}(k-1)\\
	\psi_{n_v}(k-1)+T_s\omega_{n_v}(k-1)
	\end{bmatrix},
	\end{equation}
where $ T_s $ is the sampling time used for discretization.

The moving horizon estimation problem can be formulated as:
\begin{equation}
\min_{X}J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{P^{-1}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2 , 
\label{eq:MHE_cost}
\end{equation} 
	subject to:
	\begin{align*}
	X_{k+1}&= f(X_{k},\boldsymbol{\omega}_{k}),\\
	\boldsymbol{\omega}&\in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
where $m$ is the current time step, $N_E$ is the estimation horizon, $\hat{X}$ is the estimated states, $P$ is the estimation covariance matrix, and $\Gamma$ is the measurement covariance. It is assumed that each vehicle can measure relative bearing to other vehicles and landmarks that are in the sensor's field-of-view. Relative bearing from the $i^{th}$ vehicle to the $j^{th}$ vehicle or landmark is given by the measurement model:
\begin{equation}
h(X)=\tan^{-1} \left( \frac{y_{j}-y_{i}}{x_{j}-x_{i}}\right)-\psi_i.
\end{equation} 

The first term in (\ref{eq:MHE_cost}) is known as the arrival cost and it plays an important role in stabilizing the estimator. It penalizes the deviation of the first state in the moving horizon window and its previous estimate $ \hat{X}_{m-N_E} $. The weighting matrix $ P $ is given by~\cite{rao2003constrained}
\begin{equation}
P_{k+1}=Q+\nabla F_{X}( P_k-  P_k\nabla H_{X}^{T}( \nabla H_{X}P_k\nabla H_{X}^{T}+\Gamma) ^{-1}\nabla H_{X}P_k) \nabla F_{X}^{T},
\end{equation}
where $Q$ is the state covariance matrix, and $ \nabla F_{X},\nabla H_{X} $ are the Jacobians of $ f $ and $ h $. 
%given by
%	\begin{equation}
%	\nabla F_{X}=\frac{\partial f}{\partial X_i}=
%	\begin{bmatrix}
%	1 & 0 & -T_sv\sin\psi_{i}\\
%	0 & 1 & T_sv\cos\psi_{i}\\
%	0& 0&1
%	\end{bmatrix},
%	\end{equation}
%		\begin{equation}
%		\nabla H_{X}=\frac{\partial h}{\partial X_i}=\begin{bmatrix}
%		\frac{y_{j}-y_{i}}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}&
%		\frac{-(x_{j}-x_{i})}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}& -1
%		\end{bmatrix}.
%		\end{equation}
The second term in (\ref{eq:MHE_cost}) penalizes the change in predicted measurements $ h(X_{k}) $ from the actual measurements $ z_{k} $.

Now, we look into the stability of the moving horizon estimator. The following assumptions are required for proving the stability result.

%\subsection{Assumptions}
\begin{assumption}
The initial state $X_0$ and the control input $\omega$ are such that, for any noise $q$, the system trajectory $X$ lies in a compact set $\chi$ and $\omega$ in a compact set $U$.
\label{assump:MHE1}	
\end{assumption}
\begin{assumption}
	The functions $f$ and $h$ are $C^2$ functions w.r.t $X$ on $ co(\chi) $ for every $\omega \in U$, where $co(\chi)$ is the convex closure of $ \chi $.
	\label{assump:MHE2}
\end{assumption}

Observation map for a horizon $N_E+1$ can be defined as 
\begin{equation}
F^{N_E}(X,\omega,q) = \begin{bmatrix}
h(X_{m-N_E}) \\
h \circ f^{m-N_E}(X_{m-N_E})\\
\cdot\\
\cdot\\
\cdot\\
h \circ f^{m-1} \circ \cdot \cdot \cdot f^{m-N_E}(X_{m-N_E})
\end{bmatrix},
\end{equation}
where $\circ$ is function composition. Then it is possible to re-write equation (\ref{eq:z}) as
\begin{equation}
z_{m-N_E} = F^{N_E}(X,\omega,q) + \mu_{m-N_E},
\end{equation} 
and modify the cost function as
\begin{multline}
J_m(X_{m-N_E,\hat{X}_{m-N_E}})= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \lVert F^{N_E}(X_{m-N_E},\omega_{m-N_E},q_{m-N_E}) - z_{m-N_E} \rVert_{\mathbf{\Gamma}}^2,       
\end{multline} 
$ \mathbf{\Gamma} = I_{N_E+1} \otimes \Gamma^{-1} $, where $\otimes$ is the Kronecker product.

Now, let's consider the following remarks:
\begin{remark}
	System (\ref{eq:f}), (\ref{eq:z}) is said to be observable in $N_E+1$ steps if there exists a $K$-function $\phi(\cdot)$ such that
	$
		\phi\left( \lVert x_1-x_2 \rVert^2 \right) \leq \lVert F^{N_E}(x_1,\omega,0) - F^{N_E}(x_2,\omega,0) \rVert^2,  
	$   
	$\forall x_1,x_2 \in \chi$ and $\forall \omega \in U^{N_E}$.
	\label{rem:MHE1}
\end{remark}
\begin{remark}
	 If the observability matrix $ \frac{\partial F^{N_E}(X,\omega,0)}{\partial X} $ has full rank, then the system is said to be observable in $N_E+1$ steps with finite sensitivity $1/\delta$ if the $K$-function $\phi(\cdot)$ satisfies the following condition
	\begin{equation}
		\delta = \inf_{x_1,x_2\in \chi;x_1 \neq x_2} \frac{\phi\left( \lVert x_1-x_2 \rVert^2 \right)}{ \lVert x_1-x_2 \rVert^2 } \geq 0.
	\end{equation}
\label{rem:MHE2}
\end{remark} 
Let $k_f$ be an upper bound on the Lipschitz constant of $f(X,\omega)$ w.r.t $X$ on $\chi$ for every $\omega \in U$ and $\mathbb{P}$ is diagonal with $ \mathbb{P} = pI_n, p>0 $. Let
\begin{equation}
r_{\mu} = \max_{\mu\in M} \lVert \mu \rVert^2,
\end{equation}
where $M$ is a compact set with $0\in M$. 

%\subsection{Stability}
Stability of the estimator is proved using the results from \cite{alessandri1999neural,rao2003constrained,alessandri2008moving,alessandri2010advances}. 
Consider the cost function defined as: 
\begin{equation}
	J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2,
	\label{eq:stab_cost}
\end{equation}
then we can state the following theorem~\cite{alessandri2008moving,alessandri2010advances}.

\begin{theorem}
If the Assumptions \ref{assump:MHE1},\ref{assump:MHE2} are satisfied and the Remarks \ref{rem:MHE1},\ref{rem:MHE2} hold, then there exists an upper bound defined by
\begin{equation}
\lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert^2 \leq \zeta_{m-N_E},
\end{equation} 
where $\zeta_m$ is found using the equation
\begin{equation}
\zeta_{m+1} = \left(\frac{c_1k_fp}{p+c_2\delta}\right)\zeta_m + \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu},
\label{eq:bound}
\end{equation}
$c_1,c_2$, and $c_3$ are positive constants. Let
\begin{equation}
a(p,\delta) = \frac{c_1k_fp}{(p+c_2\delta)},
\end{equation}
and if $p$ is selected such that $ a(p,\delta) <1 $, then the dynamics of (\ref{eq:bound}) is asymptotically stable. 
\end{theorem}
\begin{proof}
	A summary of the proof given by~\cite{alessandri2008moving} is detailed here for completeness. The proof is based on defining upper and lower bounds on the optimal cost $J_{m}^*$, which is the cost corresponding to an optimal estimate $\hat{X}_{m-N_E}^{*}$. First, the upper bound on $J_{m}^*$ should be defined. Let us define $X_{m}^o$ as the true value of the state $X$ at time $m$ and assume that $\Gamma = I$. We have that
	\begin{equation}
	    J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert F^{N_E}(X_{k}^o) - z_{k} \rVert^2,
	\end{equation}
	which can be modified as
	\begin{equation}
	   J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C, \label{eqn:lower_bound}  
	\end{equation}
	where $C$ is a positive constant (please see Lemma. 1 from \cite{alessandri2008moving}). Next, the upper bound on $J_{m}^*$ is defined. We can write
	\begin{eqnarray*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 &=& \lVert [z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E})] - [z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,\\
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 & \leq &2 \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 + 2 \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2, \\
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 & \geq & \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2.
	\end{eqnarray*}
	From (\ref{eqn:lower_bound}), we can write
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2 < C.
	\end{equation}
	Hence, we obtain
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 \geq \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - C. 
	\end{equation}
	By using a similar procedure, we can write
	\begin{equation}
	    \lVert X_{m-N_E}^* - \hat{X}_{m-N_E} \rVert^2 \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E} \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2. 
	\end{equation}
	Now the upper bound can be defined as
	\begin{equation}
	    J_{m}^* \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C. \label{eqn:upper_bound}
	\end{equation}
	Now, by combining the bounds (\ref{eqn:lower_bound}) and (\ref{eqn:upper_bound}) we get
	\begin{multline}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C \\ \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C,
	\end{multline}
	which can be written as
	\begin{equation}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 \leq 2 \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + 2C.
	\end{equation}
	According to the Remarks \ref{rem:MHE1} and \ref{rem:MHE2}, it can be written that
	\begin{equation*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 = \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right),
	\end{equation*}
	and
	\begin{equation*}
	    \delta \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right).
	\end{equation*}
	Now, it is possible to define the bound on the estimation error as
	\begin{equation}
	    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \frac{4p}{p+\delta}\lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 + \frac{4}{p+\delta}C.
	\end{equation}
	Using the Lipschitz continuity of $f(\cdot)$, it can be written that
	\begin{equation}
	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 = 2k_f \lVert X_{m-N_E-1}^o - \hat{X}_{m-N_E-1}^* \rVert^2 + 2r_{\mu}.
	\end{equation}
Hence,
\begin{equation*}
    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \zeta_{m-N_E}.
\end{equation*}
It can also be deduced that if $\zeta_m < \zeta_{m-1}$ and $a(p,\delta)<1$, then $\zeta_m$ tends to $\frac{\beta}{1-a(p,\delta)}$ as $m \longrightarrow +\infty$ (please see Theorem~1 from~\cite{alessandri1999neural}), where $\beta~=~ \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu} $. 	
\end{proof}

The following section presents the derivation of the analytical expression for calculating the covariances using the path information. This result will be later used for predicting covariances for the NMPC cost function.

==> Cooperative localization MPC/NMPC.tex <==
\section{NMPC formulation}\label{sec:NMPC}
Nonlinear model predictive control (NMPC) is a state-of-the-art technique for real-time optimal control. At each time step, the constrained optimization problem is solved based on the plant model for a finite time horizon, and the procedure is repeated with states updated through feedback in the next iteration~\cite{MPCbook}. Fig.~\ref{fig:block} shows the block diagram of the NMPC scheme used in this paper. The optimal control sequence is computed for the prediction horizon $ \tau_h $ from which only the first action is applied to the system at each time step. 
	 
%	\begin{figure}[h]
%		\centering
%		\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%		\caption{NMPC block diagram }
%		\label{fig:block}
%	\end{figure}
	
 A point mass kinematic model is considered for the vehicles. We assume that the altitude and velocities of the AAVs remain constant during transit. 
	\begin{equation}
	\dot{X} =
	\begin{bmatrix}
	v\cos \psi_1   \\
	v\sin \psi_1\\
	\omega_1 \\
	\vdots \\
	v\cos \psi_{n_v}   \\
	v\sin \psi_{n_v}\\
	\omega_{n_v} \\        
	\end{bmatrix},
	\end{equation}  
 where  $ v $ is the linear velocity, $ \psi $ the heading angle, $ \omega $ the angular velocity, and $ n_v $ is the number of vehicles.
	
The objective function for the NMPC is defined as
	\begin{equation}
	\min_{\boldsymbol{\omega_1 \cdots \omega_{n_v}} \in \mathcal{PC}(t,t+\tau_h)}J=\int_{t}^{t+\tau_h}\sum_{i=1}^{n_v} \left[ C_{1_i}+W_iC_{2_i}\right], 
	\label{eq:PI}
	\end{equation}	
	subject to:
	\begin{align*}
	\dot{X} &= f(X,\boldsymbol{\omega}),\\
	\boldsymbol{\omega} & \in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
	where 
	\begin{equation}
	C_{1_i}=(x_i-x_{D_i})^{2}+(y_i-y_{D_i})^{2}, 
	\end{equation}
is the cost associated with minimizing the distance between the vehicle and the destination. $(x_i,y_i) $ is the position of the $ i^{th} $ vehicle and $ (x_{D_i},y_{D_i}) $ are their respective destination points. $ \boldsymbol{\omega}^{-} $ and $ \boldsymbol{\omega}^{+}$ are the lower and upper bounds of $\boldsymbol{\omega}$, and $ \mathcal{PC}(t,t+\tau_h) $ denotes the space of piece-wise continuous function defined over the time interval $ \left[ t,t+\tau_h\right]  $.
	
$C_{2_i}$ is the cost associated with keeping the estimation covariance under bound, which is defined as:
	\begin{equation}
	C_{2_i}=\begin{cases}
	0, & \text{if $\lambda_i \geq \eta$}.\\
	(\eta-\lambda_i)^{2}, & \text{ otherwise}.
	\end{cases} \label{eq:C2}
	\end{equation} 
where $ \eta $ is a tuning parameter related to the number of connections required. Increasing $ \eta $ will result in vehicles moving closer to the landmarks and increase the connections. For satisfactory localization, observability conditions should be satisfied, which require connections with at least two landmarks~\cite{sharma2014observability}. Hence, the value of $\eta$ should be selected as~$ \eta \geq 2 $. The parameter $\lambda_i $ is the second smallest eigenvalue of the Laplacian matrix which is formed as:
	\begin{equation}
	L_i(X)=\Delta_i(X)-A_i(X),
	\end{equation} 
where $ A_i(X) $ is the adjacency matrix defined similar to~\cite{de2006decentralized} as
	\begin{equation}
	A_{i_{mn}}=\begin{cases}
	e^{\frac{-\kappa(||R_{mn}||-\rho)}{R_{s}-\rho}}, & \text{$\left| \left| R_{mn}\right| \right| \leq R_s$}.\\
	0, & \text{$\left| \left| R_{mn}\right| \right| > R_s$}.
	\end{cases}
	\end{equation} 
	and
	$ \Delta_i(X) $ is a diagonal matrix with elements
	\begin{equation}
	\Delta_{i_{mm}}=\sum_{n=1}^{N}A_{i_{mn}}
	\end{equation}
where $ m,n= 1  $ to $ N $, and $ N $ is the number of nodes of the graph connecting the vehicles and landmarks. $ \kappa $ is a constant which determines the convergence rate of the exponential function, and $\rho$ is used to set a minimum distance between the landmarks and the vehicles to avoid collisions. $ ||R_{mn}|| $ is the distance between the $ m^{th} $ and $ n^{th} $ nodes, and $ R_s $ is the sensor range of the vehicles. This formulation of the adjacency matrices, rather than updating it with binary values, helps drive the vehicles closer to the landmarks than just maintaining the connections by keeping them in the sensor range and lowering the distance between the landmarks and the vehicles help in decreasing the estimation covariance as explained in sec.~\ref{sec:analysis}. The maximum value $ \lambda_i $ can take is equal to the number of connections of each vehicle, and this insight is used in formulating (\ref{eq:C2}).   
	
The weight $W_i$ associated with $ C_{2_i} $ is defined in the following way
	\begin{equation}
	W_i=\begin{cases}
	W, & \text{if $3\sigma_{p_i} \geq \sigma_c$}.\\
	0, & \text{ otherwise}.
	\end{cases}
	\end{equation} 
where $\sigma_{p_i}$ is the standard deviation in the estimated position of the $ i^{th} $ vehicle and the constant $\sigma_c$ is the specified critical value. This adaptive weight formulation is used to get a trade-off between the two objectives. $\sigma_{p_i} $s are calculated using the expression
\begin{equation}
\sigma_{p_i}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_i-\theta_g))} \right)+(R_g^2+R_g^4)\csc^2(\psi_i-\theta_g), 
\label{eq:s_bearing_i}
\end{equation} 
which is explained in detail in section \ref{sec:b_measurement}. The terms $C_1$ and $ C_2 $ of the objective function (\ref{eq:PI}) is normalized as follows:
	\begin{eqnarray}
	C_1(t)&=&\left(\frac{C_1(t) - \min(C_1(t))}{\max(C_1(t)) - \min(C_1(t))}\right),\\
	C_2(t)&=&\left(\frac{C_2(t) - \min(C_2(t))}{\max(C_2(t)) - \min(C_2(t))}\right).
	\end{eqnarray}
	

==> Cooperative localization MPC/conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}
A nonlinear model predictive control scheme combined with moving horizon estimation was proposed to aid cooperative localization of a group of AAVs in transit. The controller used an approximate analytical expression for calculating the expected covariance of the vehicles through the prediction horizon, which was derived using the insights obtained from analyzing the observability and the path information from the landmark-vehicle graph. The controller determined near optimal paths for the vehicles while satisfying various state and localization constraints.
We analyzed through simulations the role of prediction horizon on the optimality of the vehicle paths and the required computation time.  The proposed moving horizon estimator also outperformed the EKF with lower estimation error values at a small additional computation time. A comparison was performed between cooperative and non-cooperative vehicles to show the significance of cooperation in determining paths under localization constraints. 

The approached proposed in this paper can be extended in several direction. One potential analysis is to determine how many landmarks are sufficient for a given vehicle to reach the destination meeting localization constraints. Another extension can be to include obstacle avoidance which reaching their destination as part of the problem. Experimental validation is another direction to implement the algorithms in real-world vehicle.%A limitation of inter-vehicle localization is that the errors propagate from vehicle to vehicle since the relative position reference is estimated and not a known true value like the landmarks. This problem can only be overcome by ensuring that the reference vehicle is always connected to the number of landmarks required for maintaining near-true accuracy. Finding the exact number of landmarks and their positions required for finding a feasible trajectory with a given source and destination points, the number of vehicles, and the size of the area under consideration is still an open problem for research. Also, since the urban environment contains structures and other obstructions, another prospect is to incorporate obstacle avoidance techniques into the path planning algorithm.   

==> Cooperative localization MPC/intro_2c.tex <==
\section{Introduction}\label{sec:intro}
\IEEEPARstart{U}{rban}  air mobility (UAM) is expected to have highly automated, cooperative, passenger, and cargo-carrying aerial vehicles in urban areas \cite{faa}, and the use of autonomous aerial vehicles (AAVs) for various activities are expected to rise substantially in the near future \cite{sesar}. Cargo delivery drones operate in urban canyons with high-rise buildings and other obstructions, which calls for significant localization accuracy. However, operating in such environments pose an additional challenge in localization since Global navigation satellite systems (GNSS) are unreliable in such scenarios. A solution to this problem is to use alternate localization schemes such as relative localization \cite{betke1997mobile,thrun1998finding}, vision-based methods \cite{lategahn2014vision,kim2005vision}, and ultra-wide-band (UWB) localization schemes \cite{krishnan2007uwb,zhang2018linear}. As the urban airspace is expected to contain a large number of AAVs, relative localization between vehicles can also be used in addition to known landmarks localization. 

Cooperative path planning with localization constraints involves the following components: (i) localization -- vehicles estimate their position by using relative measurements obtained with respect to other vehicles or landmarks, and (ii) cooperative path planning -- determine  optimal paths for each vehicle from a given source to destination. To achieve (ii), the agents must cooperate with each other to  generate motion commands that  improves the localization accuracy of the entire group while reducing the path length to reach their respected destinations. Several works have studied (i) and (ii)  separately. For instance, \cite{Kurazume1998,Roumeliotis2000,Spletzer2001,Mourikis2006,Nerurkar2009,wan2014cooperative,minaeian2016vision,frohle2018cooperative,pierre2018range,liu2018multi,guo2019ultra,zhu2019cooperative} address the problem of cooperative localization, while  \cite{zheng2005evolutionary,Agha-Mohammadi2014,Mathew2015,mac2016heuristic} focus on cooperative path planning problem. However, the collection of works that jointly address cooperative path planning with the localization constraints is limited. Below,  we will review some of the works in this domain.

\begin{figure}
	\centering 
	\begin{subfigure}{4cm}
		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
		\caption{}
		\label{fig:scenario}
	\end{subfigure}
	\begin{subfigure}{4cm}
		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
		\caption{}
		\label{fig:rpmg}
	\end{subfigure}
	\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
	\label{fig:path_graph}
\end{figure}  

Bopardikar et al.~\cite{bopardikar2015multiobjective} presented a graph-based probabilistic roadmap approach to tackle the path planning problem subject to localization constraints. The generated path is a discretized path while we are addressing a continuous path problem. A time-optimal path planner satisfying the covariance bounds was given in \cite{singh2016landmarks} using a swarm optimization technique coupled with a rabbit-carrot based path follower. An approach to optimally place landmarks to satisfy localization constraints was proposed in \cite{sundar2019path}. The algorithm computes an optimal path for the vehicle and the locations where the landmarks should be placed. A localizability constrained path planning method for autonomous vehicles which takes into account the laser range finder (LRF) sensor model of the vehicle is proposed in \cite{irani2018localizability} to maintain a satisfactory level of localizability throughout the path. Kassas et al. \cite{kassas2021uav} present a multi-objective motion planning algorithm in which the vehicle tries to balance the objectives of navigating to the waypoint and reducing its position estimate uncertainty. All the above works are limited to one vehicle only. %In \cite{manoharan2019nonlinear}, a nonlinear model predictive control scheme was used to find optimal paths  for a group of cooperative UAVs satisfying the  required localization accuracy.

Urban air mobility calls for improved localization accuracy due to its innate nature involving close structures, narrow pathways, and a large number of vehicles. Moving horizon estimation (MHE) has been suggested as an alternate to EKF for increasing the accuracy of nonlinear estimation problems by \cite{rawlings2006particle,wang2014optimization,mehrez2017optimization}. Erunsal et al. \cite{erunsal2019decentralized} proposed an approach combining NMPC and pose-graph-MHE for 3D formation control of micro aerial vehicles with relative sensing capability. In \cite{liu2020decentralized}, a decentralized MHE technique is proposed for networked navigation with packet dropouts.    

In this paper, we extend the  work in ~\cite{manoharan2019nonlinear} and propose a joint cooperative localization and path planning framework with MHE for estimating the vehicle position, and NMPC  framework for cooperative path planning, and a closed formulation for covariance calculation to  predict the uncertainty. This framework uses a nonlinear vehicle model in both the controller and the estimator, which mitigates the linearization errors. The analytical expression used for the covariance calculation speeds up the computations and is derived by exploiting the relationship between the vehicle-landmark path lengths to the localization uncertainty. The proposed approach provides a flexibility, where each vehicle can decide to maintain, lose, or gain connections depending on their covariance estimates.In most of the literature for multi-agent systems, the studies are formulated either as a control problem or an estimation problem \cite{Mourikis2006,Nerurkar2009,Roumeliotis2000,wan2014cooperative,wang2014optimization}. We propose a method that combines both and looks at the multi-agent problem in a holistic sense.



%Previous studies \cite{Agha-Mohammadi2014,Mathew2015,wan2014cooperative} used algorithms that were not optimal and were based on conventional path planners, whereas NMPC provides optimal paths while satisfying imposed state and input constraints. %The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. 
%Also, most of the works based on graph-based planning give discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, eliminating the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2006maximizing} and \cite{de2006decentralized}. We also use a Laplacian matrix based solution, but we calculate Laplacian matrices for each vehicle instead of forming a single matrix for the whole group. This helps in identifying connectivity at an individual level, and each vehicle can decide to maintain, lose, or gain connections depending on their covariance estimates. %This is not possible in the single matrix case because a single vehicle with more connections will increase the Laplacian, even though the other vehicles may be out of the required number of connections. 
%Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. %So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. 
% This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy. The works on path planning with localization constraints \cite{singh2016landmarks,sundar2019path,kassas2021uav,irani2018localizability} consider only single vehicles and fixed landmarks in most cases, whereas our approach includes multiple vehicles, and each vehicle is considered a moving landmark. Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobian, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. Now, we can summarize 


















%Previous studies \cite{Agha-Mohammadi2014,Mathew2015,wan2014cooperative} used algorithms that were not optimal and were based on conventional path planners, whereas NMPC provides optimal paths while satisfying imposed state and input constraints. %The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. 
%Also, most of the works based on graph-based planning give discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, eliminating the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2006maximizing} and \cite{de2006decentralized}. We also use a Laplacian matrix based solution, but we calculate Laplacian matrices for each vehicle instead of forming a single matrix for the whole group. This helps in identifying connectivity at an individual level, and each vehicle can decide to maintain, lose, or gain connections depending on their covariance estimates. %This is not possible in the single matrix case because a single vehicle with more connections will increase the Laplacian, even though the other vehicles may be out of the required number of connections. 
%Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. %So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. 
% This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy. The works on path planning with localization constraints \cite{singh2016landmarks,sundar2019path,kassas2021uav,irani2018localizability} consider only single vehicles and fixed landmarks in most cases, whereas our approach includes multiple vehicles, and each vehicle is considered a moving landmark. Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobian, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. Now, we can summarize 
The major contributions of this paper as follows:
\begin{itemize}
	\item A complete framework for control and estimation of multi-vehicle cooperative path planning problem with localization constraints using NMPC and MHE.
	\item An analysis on the relation of path lengths between vehicles and landmarks on the estimation covariance
\item An approximate closed form analytical expression to compute localization error covariance
\item Evaluation of the proposed joint cooperative path planning with localization constraints framework through numerical simulations and comparison with EKF-based estimation framework
\end{itemize}

The rest of the paper is organized as follows. The problem formulation is given in Section \ref{sec:problem}. Moving horizon estimation (MHE) is explained in Section \ref{sec:MHE}. The derivation of the analytic expression for covariance is given in Section \ref{sec:analysis}. The NMPC formulation is given in Section \ref{sec:NMPC}. Simulation results are presented in Section \ref{sec:results}, and the conclusions are given in Section \ref{sec:conclusions}. 

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%	\caption{Block diagram showing the proposed NMPC-MHE control scheme.}
%	\label{fig:block}
%\end{figure} 

\begin{figure*}
	\centering 
	\begin{subfigure}{7cm}
		\includegraphics[width=7cm]{figs/BlockDiagram.eps}
	\end{subfigure}
	\begin{subfigure}{7cm}
		\includegraphics[width=7cm]{figs/covariance.eps}		
	\end{subfigure}\hfil 
	\caption{Block diagram and a graphical representation of the proposed NMPC-MHE control scheme. }
	\label{fig:block}
\end{figure*}  

\section{Problem formulation}\label{sec:problem}	
%Around-the-clock delivery of essential supplies like medicines from one location to another is an important application of autonomous aerial vehicles \cite{ups2}. 
We consider a scenario where a group of AAVs need to navigate from their source location ($S$) to destination ($D$), as shown in Fig.~\ref{fig:scenario}. These vehicles need to transit in a GPS-denied area and we assume that any kind of GNSS are not available. In such scenarios, known landmarks or other vehicles in the area can be used for relative localization using range or bearing measurements. This structure involving landmarks and vehicles can be modeled as a dynamic relative position measurement graph (RPMG) \cite{sharma2011graph} with vehicles and landmarks as nodes and connections/measurements as edges.
\begin{definition}
	A relative position measurement graph (RPMG) for $n_v(t)$ vehicles with $n_l(t)$ landmarks is a graph $G_{n_v}^{n_l}(t)~\triangleq~\{\mathcal{V}_{n_v}^{n_l}(t),\mathcal{E}_{n_v}^{n_l}(t) \}$, where $\mathcal{V}_{n_v}^{n_l}$ is the node set consisting of $n_v(t)$ vehicle nodes and $n_l(t)$ landmark nodes (which makes a total of $n_v(t)+n_l(t)$ nodes), and $\mathcal{E}_{n_v}^{n_l}(t)$ is the edge set representing available relative measurements. The number of edges is denoted by $n_e(t)= |\mathcal{E}_{n_v}^{n_l}(t)|$.   
\end{definition}
\begin{definition}
	A path from a vehicle node to a landmark node is a finite sequence of edges which joins a sequence of distinct vertices between them. Let $\mathcal{G} \triangleq \{\mathcal{V},\mathcal{E},\phi\} $ be a graph. A path $\phi$ from vertex $i$ to vertex $j$ is a sequence of edges $\{\epsilon_1,\epsilon_2, \ldots, \epsilon_{n-1} \}$ for which there is a sequence of distinct vertices $\{\nu_1,\nu_2, \ldots, \nu_n \}$ such that $\phi \triangleq \{ \nu_1,\nu_n \}$ where $\nu_1 = i$ and $\nu_n = j$.
\end{definition}
An example RPMG ($G_{5}^{3}$ with $n_e=7$) is shown in Fig.~\ref{fig:rpmg}. A path from the vehicle $5$ to the landmark $a$ is represented by the edge set $\phi \triangleq \{\epsilon_6,\epsilon_5,\epsilon_3 \}$ which can also be represented using the vertices as $5-4-2-a$. 

Previous studies show that for cooperative localization to work, each vehicle should have a direct or indirect path to at least two known landmarks \cite{sharma2014observability}. This condition is very limiting in environments with a low number of landmarks. Hence in this paper, we find a relationship between vehicle uncertainty and path length to the landmarks and then use that relationship to formulate and solve an NMPC problem to guarantee that the covariance does not exceed a specified threshold and desired localization accuracy is achieved while performing individual missions. A moving horizon estimation (MHE) scheme is used to estimate the vehicle states. 

A graphical representation of the proposed solution using NMPC combined with MHE to tackle the cooperative localization and path planning problem is shown in Fig.~\ref{fig:block}. The optimal path is different from the shortest path since the latter may not satisfy localization constraints. The components of the block diagram are explained in the subsequent sections. In the first step of the control scheme, vehicle states are estimated by the MHE block using available measurements from the sensors (Sec.~\ref{sec:MHE}). The second step is the calculation of estimation covariances for the NMPC prediction window, which is accomplished by the covariance calculator block that contains the derived analytical expression (Sec.~\ref{sec:analysis}). In the third and final step, the NMPC controller computes the control actions for the vehicles (Sec.~\ref{sec:NMPC}). 



==> Cooperative localization MPC/mhe_2c.tex <==
\section{Moving horizon estimation}\label{sec:MHE}
Moving horizon estimation (MHE) uses optimization techniques to find state trajectories that best fit a series of measurements acquired over a finite time interval. It uses the exact nonlinear models of the available measurements and system dynamics for estimation. Also, there is another advantage of including the state/control constraints in the formulation, which helps in bounding the estimates. Like NMPC, MHE also has three main components, 1) an internal dynamic model of the process, 2) a history of past measurements, and 3) an optimization cost function over the estimation horizon.
%In MHE, an iterative approach based on linear or nonlinear programming is used to find the estimates. 
%MHE is superior to the extended Kalman filter (EKF), the most commonly used nonlinear estimator for multi-agent systems~\cite{haseltine2005critical} since the EKF linearizes nonlinear models at operating points.  
%Also, EKF is based on the Markov assumption that the current state estimate is based only on the most recent measurements and the previous state estimate. Since the MHE minimizes the deviation of the model from the past interval of measurements, the Markov assumption is relaxed.  

The model used for estimation is given as:
\begin{eqnarray}
X(k)&=&f\left( X(k-1),\boldsymbol{\omega}(k),k\right) +q(k), \label{eq:f}\\
z(k)&=&h\left( X(k),\boldsymbol{\omega}(k),k\right) + \mu(k), \label{eq:z}
\end{eqnarray}	
where, $f(\cdot)$ and $h(\cdot) $ represent the state model and the observation model respectively. ${X}(k)$ and $ z(k) $ are the system states and measurements at the $k^{\mathrm{th}}$ time instant. The vectors $ q(k) $ and $ \mu(k) $ are the process and measurement noises which are assumed to be additive and zero mean white Gaussian noises with covariance $ Q $ and $ \Gamma $ respectively. $ f(\cdot) $ is defined as
	\begin{equation}
	f=\begin{bmatrix}
	x_{1}(k)\\
	y_{1}(k)\\
	\psi_{1}(k)\\
	\vdots\\
	x_{n_v}(k)\\
	y_{n_v}(k)\\
	\psi_{n_v}(k)
	\end{bmatrix}=
	\begin{bmatrix}
	x_{1}(k-1)+T_sv\cos\psi_{1}(k-1)\\
	y_{1}(k-1)+T_sv\sin\psi_{1}(k-1)\\
	\psi_{1}(k-1)+T_s\omega_1(k-1)\\
	\vdots\\
	x_{n_v}(k-1)+T_sv\cos\psi_{n_v}(k-1)\\
	y_{n_v}(k-1)+T_sv\sin\psi_{n_v}(k-1)\\
	\psi_{n_v}(k-1)+T_s\omega_{n_v}(k-1)
	\end{bmatrix},
	\end{equation}
where $ T_s $ is the sampling time used for discretization.

The moving horizon estimation problem can be formulated as:
\begin{equation}
\min_{X}J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{P^{-1}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2 , 
\label{eq:MHE_cost}\nonumber
\end{equation} 
	subject to:
	\begin{align*}
	X_{k+1}&= f(X_{k},\boldsymbol{\omega}_{k}),\\
	\boldsymbol{\omega}&\in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
where $m$ is the current time step, $N_E$ is the estimation horizon, $\hat{X}$ is the estimated states, $P$ is the estimation covariance matrix, and $\Gamma$ is the measurement covariance. It is assumed that each vehicle can measure relative bearing to other vehicles and landmarks that are in the sensor's field-of-view. Relative bearing from the $i^{th}$ vehicle to the $j^{th}$ vehicle or landmark is given by the measurement model:
\begin{equation}
h(X)=\tan^{-1} \left( \frac{y_{j}-y_{i}}{x_{j}-x_{i}}\right)-\psi_i.
\end{equation} 

The first term in (\ref{eq:MHE_cost}) is known as the arrival cost and it plays an important role in stabilizing the estimator. It penalizes the deviation of the first state in the moving horizon window and its previous estimate $ \hat{X}_{m-N_E} $. The weighting matrix $ P $ is given by~\cite{rao2003constrained}
\begin{eqnarray}
P_{k+1}&=&Q+\nabla F_{X}( P_k-  P_k\nabla H_{X}^{T}( \nabla H_{X}P_k\nabla H_{X}^{T}+\Gamma) ^{-1}\nonumber\\
&&\nabla H_{X}P_k) \nabla F_{X}^{T},\nonumber
\end{eqnarray}
where $Q$ is the state covariance matrix, and $ \nabla F_{X},\nabla H_{X} $ are the Jacobians of $ f $ and $ h $. 
%given by
%	\begin{equation}
%	\nabla F_{X}=\frac{\partial f}{\partial X_i}=
%	\begin{bmatrix}
%	1 & 0 & -T_sv\sin\psi_{i}\\
%	0 & 1 & T_sv\cos\psi_{i}\\
%	0& 0&1
%	\end{bmatrix},
%	\end{equation}
%		\begin{equation}
%		\nabla H_{X}=\frac{\partial h}{\partial X_i}=\begin{bmatrix}
%		\frac{y_{j}-y_{i}}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}&
%		\frac{-(x_{j}-x_{i})}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}& -1
%		\end{bmatrix}.
%		\end{equation}
The second term in (\ref{eq:MHE_cost}) penalizes the change in predicted measurements $ h(X_{k}) $ from the actual measurements $ z_{k} $.

Now, we look into the stability of the moving horizon estimator. The following assumptions are required for proving the stability result.

%\subsection{Assumptions}
\begin{assumption}
The initial state $X_0$ and the control input $\omega$ are such that, for any noise $q$, the system trajectory $X$ lies in a compact set $\chi$ and $\omega$ in a compact set $U$.
\label{assump:MHE1}	
\end{assumption}
\begin{assumption}
	The functions $f$ and $h$ are $C^2$ functions w.r.t $X$ on $ co(\chi) $ for every $\omega \in U$, where $co(\chi)$ is the convex closure of $ \chi $.
	\label{assump:MHE2}
\end{assumption}

Observation map for a horizon $N_E+1$ can be defined as 
\begin{equation}
F^{N_E}(X,\omega,q) = \begin{bmatrix}
h(X_{m-N_E}) \\
h \circ f^{m-N_E}(X_{m-N_E})\\
\cdot\\
\cdot\\
\cdot\\
h \circ f^{m-1} \circ \cdot \cdot \cdot f^{m-N_E}(X_{m-N_E})
\end{bmatrix},
\end{equation}
where $\circ$ is function composition. Then it is possible to re-write equation (\ref{eq:z}) as
\begin{equation}
z_{m-N_E} = F^{N_E}(X,\omega,q) + \mu_{m-N_E},
\end{equation} 
and modify the cost function as
\begin{multline}
J_m(X_{m-N_E,\hat{X}_{m-N_E}})= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  +\\ \lVert F^{N_E}(X_{m-N_E},\omega_{m-N_E},q_{m-N_E}) - z_{m-N_E} \rVert_{\mathbf{\Gamma}}^2,       
\end{multline} 
$ \mathbf{\Gamma} = I_{N_E+1} \otimes \Gamma^{-1} $, where $\otimes$ is the Kronecker product.

Now, let's consider the following remarks:
\begin{remark}
	System (\ref{eq:f}), (\ref{eq:z}) is said to be observable in $N_E+1$ steps if there exists a $K$-function $\phi(\cdot)$ such that
	$
		\phi\left( \lVert x_1-x_2 \rVert^2 \right) \leq \lVert F^{N_E}(x_1,\omega,0) - F^{N_E}(x_2,\omega,0) \rVert^2,  
	$   
	$\forall x_1,x_2 \in \chi$ and $\forall \omega \in U^{N_E}$.
	\label{rem:MHE1}
\end{remark}
\begin{remark}
	 If the observability matrix $ \frac{\partial F^{N_E}(X,\omega,0)}{\partial X} $ has full rank, then the system is said to be observable in $N_E+1$ steps with finite sensitivity $1/\delta$ if the $K$-function $\phi(\cdot)$ satisfies the following condition
	\begin{equation}
		\delta = \inf_{x_1,x_2\in \chi;x_1 \neq x_2} \frac{\phi\left( \lVert x_1-x_2 \rVert^2 \right)}{ \lVert x_1-x_2 \rVert^2 } \geq 0.
	\end{equation}
\label{rem:MHE2}
\end{remark} 
Let $k_f$ be an upper bound on the Lipschitz constant of $f(X,\omega)$ w.r.t $X$ on $\chi$ for every $\omega \in U$ and $\mathbb{P}$ is diagonal with $ \mathbb{P} = pI_n, p>0 $. Let
\begin{equation}
r_{\mu} = \max_{\mu\in M} \lVert \mu \rVert^2,
\end{equation}
where $M$ is a compact set with $0\in M$. 

%\subsection{Stability}
Stability of the estimator is proved using the results from \cite{alessandri1999neural,rao2003constrained,alessandri2008moving,alessandri2010advances}. 
Consider the cost function defined as: 
\begin{equation}
	J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2,
	\label{eq:stab_cost}
\end{equation}
then we can state the following theorem~\cite{alessandri2008moving,alessandri2010advances}.

\begin{theorem}
If the Assumptions \ref{assump:MHE1},\ref{assump:MHE2} are satisfied and the Remarks \ref{rem:MHE1},\ref{rem:MHE2} hold, then there exists an upper bound defined by
\begin{equation}
\lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert^2 \leq \zeta_{m-N_E},
\end{equation} 
where $\zeta_m$ is found using the equation
\begin{equation}
\zeta_{m+1} = \left(\frac{c_1k_fp}{p+c_2\delta}\right)\zeta_m + \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu},
\label{eq:bound}
\end{equation}
$c_1,c_2$, and $c_3$ are positive constants. Let
\begin{equation}
a(p,\delta) = \frac{c_1k_fp}{(p+c_2\delta)},
\end{equation}
and if $p$ is selected such that $ a(p,\delta) <1 $, then the dynamics of (\ref{eq:bound}) is asymptotically stable. 
\end{theorem}
\begin{proof}
	A summary of the proof given by~\cite{alessandri2008moving} is detailed here for completeness. The proof is based on defining upper and lower bounds on the optimal cost $J_{m}^*$, which is the cost corresponding to an optimal estimate $\hat{X}_{m-N_E}^{*}$. First, the upper bound on $J_{m}^*$ should be defined. Let us define $X_{m}^o$ as the true value of the state $X$ at time $m$ and assume that $\Gamma = I$. We have that
	\begin{equation}
	    J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert F^{N_E}(X_{k}^o) - z_{k} \rVert^2,
	\end{equation}
	which can be modified as
	\begin{equation}
	   J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C, \label{eqn:lower_bound}  
	\end{equation}
	where $C$ is a positive constant (please see Lemma. 1 from \cite{alessandri2008moving}). Next, the upper bound on $J_{m}^*$ is defined. We can write
	{\tiny
	\begin{eqnarray}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 =&& \nonumber\\
	    \lVert [z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E})] - [z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,&&\\
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2  \leq&& \nonumber\\ 2 \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 + 2 \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,&& \\
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2  \geq&& \nonumber \\ \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2.&&
	\end{eqnarray}
}
	From (\ref{eqn:lower_bound}), we can write
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2 < C.
	\end{equation}
	Hence, we obtain
	{\scriptsize	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 \geq \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - C. \nonumber
	\end{equation}}
	By using a similar procedure, we can write
		{\scriptsize
	\begin{equation}
	    \lVert X_{m-N_E}^* - \hat{X}_{m-N_E} \rVert^2 \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E} \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2. \nonumber
	\end{equation}}
	Now the upper bound can be defined as
	\begin{eqnarray}
	    J_{m}^* &\geq& \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \nonumber \\&&\frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \nonumber \\
&&	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C. \label{eqn:upper_bound}
	\end{eqnarray}
	Now, by combining the bounds (\ref{eqn:lower_bound}) and (\ref{eqn:upper_bound}), and rewriting we get
%	\begin{multline}
%	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C \\ \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C,
%	\end{multline}
%	which can be written as
{\scriptsize
	\begin{eqnarray}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 +  \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) -  F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 \nonumber && \\\leq 2 \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + 2C.\nonumber
	\end{eqnarray}}
	According to the Remarks \ref{rem:MHE1} and \ref{rem:MHE2}, the above equation can be written as
	{\footnotesize
	\begin{equation*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 = \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right),
	\end{equation*}}
	and
	\begin{equation*}
	    \delta \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right).\nonumber
	\end{equation*}
	Now, it is possible to define the bound on the estimation error as
	\begin{equation}
	    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \frac{4p}{p+\delta}\lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 + \frac{4}{p+\delta}C.\nonumber
	\end{equation}
	Using the Lipschitz continuity of $f(\cdot)$, it can be written that
	\begin{equation}
	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 = 2k_f \lVert X_{m-N_E-1}^o - \hat{X}_{m-N_E-1}^* \rVert^2 + 2r_{\mu}.\nonumber
	\end{equation}
Hence,
\begin{equation*}
    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \zeta_{m-N_E}.
\end{equation*}
It can also be deduced that if $\zeta_m < \zeta_{m-1}$ and $a(p,\delta)<1$, then $\zeta_m$ tends to $\frac{\beta}{1-a(p,\delta)}$ as $m \longrightarrow +\infty$ (please see Theorem~1 from~\cite{alessandri1999neural}), where $\beta~=~ \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu} $. 	
\end{proof}

The following section presents the derivation of the analytical expression for calculating the covariances using the path information. This result will be later used for predicting covariances for the NMPC cost function.

==> Cooperative localization MPC/mhe_2c_v1.tex <==
\section{Moving horizon estimation}\label{sec:MHE}
Moving horizon estimation (MHE) uses optimization techniques to determine state trajectories that best fit a series of measurements acquired over a finite time interval. It uses the exact nonlinear models of the available measurements and system dynamics for estimation. Also, there is another advantage of including the state/control constraints in the formulation, which helps in bounding the estimates. Like NMPC, MHE also has three main components, 1) an internal dynamic model of the process, 2) a history of past measurements, and 3) an optimization cost function over the estimation horizon.
%In MHE, an iterative approach based on linear or nonlinear programming is used to find the estimates. 
%MHE is superior to the extended Kalman filter (EKF), the most commonly used nonlinear estimator for multi-agent systems~\cite{haseltine2005critical} since the EKF linearizes nonlinear models at operating points.  
%Also, EKF is based on the Markov assumption that the current state estimate is based only on the most recent measurements and the previous state estimate. Since the MHE minimizes the deviation of the model from the past interval of measurements, the Markov assumption is relaxed.  

The model used for estimation is given as:
\begin{eqnarray}
X(k)&=&f\left( X(k-1),\boldsymbol{\omega}(k),k\right) +q(k), \label{eq:f}\\
z(k)&=&h\left( X(k),\boldsymbol{\omega}(k),k\right) + \mu(k), \label{eq:z}
\end{eqnarray}	
where, $f(\cdot)$ and $h(\cdot) $ represent the state model and the observation model respectively. ${X}(k)$ and $ z(k) $ are the system states and measurements at the $k^{\mathrm{th}}$ time instant. The vectors $ q(k) $ and $ \mu(k) $ are the process and measurement noises which are assumed to be additive and zero mean white Gaussian noises with covariance $ Q $ and $ \Gamma $ respectively. $ f(\cdot) $ is defined as
	\begin{equation}
	f=\begin{bmatrix}
	x_{1}(k)\\
	y_{1}(k)\\
	\psi_{1}(k)\\
	\vdots\\
	x_{n_v}(k)\\
	y_{n_v}(k)\\
	\psi_{n_v}(k)
	\end{bmatrix}=
	\begin{bmatrix}
	x_{1}(k-1)+T_sv\cos\psi_{1}(k-1)\\
	y_{1}(k-1)+T_sv\sin\psi_{1}(k-1)\\
	\psi_{1}(k-1)+T_s\omega_1(k-1)\\
	\vdots\\
	x_{n_v}(k-1)+T_sv\cos\psi_{n_v}(k-1)\\
	y_{n_v}(k-1)+T_sv\sin\psi_{n_v}(k-1)\\
	\psi_{n_v}(k-1)+T_s\omega_{n_v}(k-1)
	\end{bmatrix},
	\end{equation}
where $ T_s $ is the sampling time used for discretization.

Let $m$ be the current time step, $N_E$ is the estimation horizon, and  we denote $\tau=m-N_E$ for simplicity. We  formulate the moving horizon estimation problem 
\begin{equation}
\min_{X}J= \lVert X_{\tau} - \hat{X}_{\tau} \rVert_{P^{-1}_{\tau}}^2  + \sum_{k=\tau}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2 , 
\label{eq:MHE_cost}
\end{equation} 
	subject to:
	\begin{align*}
	X_{k+1}&= f(X_{k},\boldsymbol{\omega}_{k}),\\
	\boldsymbol{\omega}&\in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
where  $\hat{X}$ is the estimated states, $P$ is the estimation covariance matrix, and $\Gamma$ is the measurement covariance. It is assumed that each vehicle can measure relative bearing to other vehicles and landmarks that are in the sensor's field-of-view ($R_s$). Relative bearing from the $i^{th}$ vehicle to the $j^{th}$ vehicle or landmark is given by the measurement model:
\begin{equation}
h(X)=\tan^{-1} \left( \frac{y_{j}-y_{i}}{x_{j}-x_{i}}\right)-\psi_i.
\end{equation} 

The first term in (\ref{eq:MHE_cost}) is known as the arrival cost and it plays an important role in stabilizing the estimator. It penalizes the deviation of the first state in the moving horizon window and its previous estimate $ \hat{X}_{\tau} $. The weighting matrix $ P $ is given by~\cite{rao2003constrained}
\begin{eqnarray}
P_{k+1}&=&Q+\nabla F_{X}( P_k-  P_k\nabla H_{X}^{T}( \nabla H_{X}P_k\nabla H_{X}^{T}+\Gamma) ^{-1}\nonumber\\
&&\nabla H_{X}P_k) \nabla F_{X}^{T},\nonumber
\end{eqnarray}
where $Q$ is the state covariance matrix, and $ \nabla F_{X},\nabla H_{X} $ are the Jacobians of $ f $ and $ h $. 
%given by
%	\begin{equation}
%	\nabla F_{X}=\frac{\partial f}{\partial X_i}=
%	\begin{bmatrix}
%	1 & 0 & -T_sv\sin\psi_{i}\\
%	0 & 1 & T_sv\cos\psi_{i}\\
%	0& 0&1
%	\end{bmatrix},
%	\end{equation}
%		\begin{equation}
%		\nabla H_{X}=\frac{\partial h}{\partial X_i}=\begin{bmatrix}
%		\frac{y_{j}-y_{i}}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}&
%		\frac{-(x_{j}-x_{i})}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}& -1
%		\end{bmatrix}.
%		\end{equation}
The second term in (\ref{eq:MHE_cost}) penalizes the change in predicted measurements $ h(X_{k}) $ from the actual measurements $ z_{k} $.

Now, we look into the stability of the moving horizon estimator. The following assumptions are required for proving the stability result.

%\subsection{Assumptions}
\begin{assumption}
The initial state $X_0$ and the control input $\omega$ are such that, for any noise $q$, the system trajectory $X$ lies in a compact set $\chi$ and $\omega$ in a compact set $U$.
\label{assump:MHE1}	
\end{assumption}
\begin{assumption}
	The functions $f$ and $h$ are $C^2$ functions w.r.t $X$ on $ co(\chi) $ for every $\omega \in U$, where $co(\chi)$ is the convex closure of $ \chi $.
	\label{assump:MHE2}
\end{assumption}

Observation map for a horizon $N_E+1$ can be defined as 
\begin{equation}
F^{N_E}(X,\omega,q) = \begin{bmatrix}
h(X_{\tau}) \\
h \circ f^{\tau}(X_{\tau})\\
\cdot\\
\cdot\\
\cdot\\
h \circ f^{m-1} \circ \cdot \cdot \cdot f^{\tau}(X_{\tau})
\end{bmatrix},
\end{equation}
where $\circ$ is function composition. Then it is possible to re-write equation (\ref{eq:z}) as
\begin{equation}
z_{\tau} = F^{N_E}(X,\omega,q) + \mu_{\tau},
\end{equation} 
and modify the cost function as
\begin{equation}
J_m(X_{\tau,\hat{X}_{\tau}})= \lVert X_{\tau} - \hat{X}_{\tau} \rVert_{\mathbb{P}_{\tau}}^2  +\lVert F^{N_E}(X_{\tau},\omega_{\tau},q_{\tau}) - z_{\tau} \rVert_{\mathbf{\Gamma}}^2,       
\end{equation} 
where, $ \mathbf{\Gamma} = I_{N_E+1} \otimes \Gamma^{-1} $, where $\otimes$ is the Kronecker product.

Now, let's consider the following remarks:
\begin{remark}
	System (\ref{eq:f}), (\ref{eq:z}) is said to be observable in $N_E+1$ steps if there exists a $K$-function $\phi(\cdot)$ such that
	$
		\phi\left( \lVert x_1-x_2 \rVert^2 \right) \leq \lVert F^{N_E}(x_1,\omega,0) - F^{N_E}(x_2,\omega,0) \rVert^2,  
	$   
	$\forall x_1,x_2 \in \chi$ and $\forall \omega \in U^{N_E}$.
	\label{rem:MHE1}
\end{remark}
\begin{remark}
	 If the observability matrix $ \frac{\partial F^{N_E}(X,\omega,0)}{\partial X} $ has full rank, then the system is said to be observable in $N_E+1$ steps with finite sensitivity $1/\delta$ if the $K$-function $\phi(\cdot)$ satisfies the following condition
	\begin{equation}
		\delta = \inf_{x_1,x_2\in \chi;x_1 \neq x_2} \frac{\phi\left( \lVert x_1-x_2 \rVert^2 \right)}{ \lVert x_1-x_2 \rVert^2 } \geq 0.
	\end{equation}
\label{rem:MHE2}
\end{remark} 
Let $k_f$ be an upper bound on the Lipschitz constant of $f(X,\omega)$ w.r.t $X$ on $\chi$ for every $\omega \in U$ and $\mathbb{P}$ is diagonal with $ \mathbb{P} = pI_n, p>0 $. Let
\begin{equation}
r_{\mu} = \max_{\mu\in M} \lVert \mu \rVert^2,
\end{equation}
where $M$ is a compact set with $0\in M$. 

%\subsection{Stability}
Stability of the estimator is proved using the results from \cite{alessandri1999neural,rao2003constrained,alessandri2008moving,alessandri2010advances}. 
Consider the cost function defined as: 
\begin{equation}
	J= \lVert X_{\tau} - \hat{X}_{\tau} \rVert_{\mathbb{P}_{\tau}}^2  + \sum_{k=\tau}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2,
	\label{eq:stab_cost}
\end{equation}
then we can state the following theorem~\cite{alessandri2008moving,alessandri2010advances}.

\begin{theorem}
If the Assumptions \ref{assump:MHE1},\ref{assump:MHE2} are satisfied and the Remarks \ref{rem:MHE1},\ref{rem:MHE2} hold, then there exists an upper bound defined by
\begin{equation}
\lVert X_{\tau} - \hat{X}_{\tau} \rVert^2 \leq \zeta_{\tau},
\end{equation} 
where $\zeta_m$ is found using the equation
\begin{equation}
\zeta_{m+1} = \left(\frac{c_1k_fp}{p+c_2\delta}\right)\zeta_m + \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu},
\label{eq:bound}
\end{equation}
$c_1,c_2$, and $c_3$ are positive constants. Let
\begin{equation}
a(p,\delta) = \frac{c_1k_fp}{(p+c_2\delta)},
\end{equation}
and if $p$ is selected such that $ a(p,\delta) <1 $, then the dynamics of (\ref{eq:bound}) is asymptotically stable. 
\end{theorem}
\begin{proof}
	A summary of the proof given by~\cite{alessandri2008moving} is detailed here for completeness. The proof is based on defining upper and lower bounds on the optimal cost $J_{m}^*$, which is the cost corresponding to an optimal estimate $\hat{X}_{\tau}^{*}$. First, the upper bound on $J_{m}^*$ should be defined. Let us define $X_{m}^o$ as the true value of the state $X$ at time $m$ and assume that $\Gamma = I$. We have that
	\begin{equation}
	    J_{m}^* \leq \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2  + \sum_{k=\tau}^{m} \lVert F^{N_E}(X_{k}^o) - z_{k} \rVert^2,
	\end{equation}
	which can be modified as
	\begin{equation}
	   J_{m}^* \leq \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 + C, \label{eqn:lower_bound}  
	\end{equation}
	where $C$ is a positive constant (please see Lemma. 1 from \cite{alessandri2008moving}). Next, the upper bound on $J_{m}^*$ is defined. We can write
	{
	\begin{eqnarray}
	    \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}) \rVert^2 =&& \nonumber\\
	    \lVert [z_{\tau} - F^{N_E}(\hat{X}_{\tau})] - [z_{\tau} - F^{N_E}(X_{\tau}^o)] \rVert^2,&&\\
	    \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}) \rVert^2  \leq&& \nonumber\\ 2 \lVert z_{\tau} - F^{N_E}(\hat{X}_{\tau}) \rVert^2 + 2 \lVert z_{\tau} - F^{N_E}(X_{\tau}^o)] \rVert^2,&& \\
	    \lVert z_{\tau} - F^{N_E}(\hat{X}_{\tau}) \rVert^2  \geq&& \nonumber \\ \frac{1}{2} \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}) \rVert^2 - \lVert z_{\tau} - F^{N_E}(X_{\tau}^o)] \rVert^2.&&
	\end{eqnarray}
}
	From (\ref{eqn:lower_bound}), we can write
	\begin{equation}
	    \lVert z_{\tau} - F^{N_E}(X_{\tau}^o)] \rVert^2 < C.
	\end{equation}
	Hence, we obtain
	{	\begin{equation}
	    \lVert z_{\tau} - F^{N_E}(\hat{X}_{\tau}) \rVert^2 \geq \frac{1}{2} \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}) \rVert^2 - C. \nonumber
	\end{equation}}
	By using a similar procedure, we can write
		{
	\begin{equation}
	    \lVert X_{\tau}^* - \hat{X}_{\tau} \rVert^2 \geq \frac{1}{2} \lVert X_{\tau}^o - \hat{X}_{\tau} \rVert^2 - \lVert X_{\tau}^o - X_{\tau}^* \rVert^2. \nonumber
	\end{equation}}
	Now the upper bound can be defined as
	\begin{eqnarray}
	    J_{m}^* &\geq& \frac{1}{2} \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}^*) \rVert^2 - \nonumber \\
&&	    \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 - C. \label{eqn:upper_bound}
	\end{eqnarray}
	Now, by combining the bounds (\ref{eqn:lower_bound}) and (\ref{eqn:upper_bound}), and rewriting we get
%	\begin{multline}
%	    \frac{1}{2} \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}^*) \rVert^2 - \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 - C \\ \leq \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 + C,
%	\end{multline}
%	which can be written as
{
	\begin{eqnarray}
	    \frac{1}{2} \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 +  \frac{1}{2} \lVert F^{N_E}(X_{\tau}^o) -  F^{N_E}(\hat{X}_{\tau}^*) \rVert^2 \nonumber && \\\leq 2 \lVert X_{\tau}^o - X_{\tau}^* \rVert_{\mathbb{P}_{\tau}}^2 + 2C.\nonumber
	\end{eqnarray}}
	According to the Remarks \ref{rem:MHE1} and \ref{rem:MHE2}, the above equation can be written as
	{
	\begin{equation*}
	    \lVert F^{N_E}(X_{\tau}^o) - F^{N_E}(\hat{X}_{\tau}^*) \rVert^2 = \phi \left( \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert^2 \right),
	\end{equation*}}
	and
	\begin{equation*}
	    \delta \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert^2 \leq \phi \left( \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert^2 \right).\nonumber
	\end{equation*}
	Now, it is possible to define the bound on the estimation error as
	\begin{equation}
	    \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert^2 \leq \frac{4p}{p+\delta}\lVert X_{\tau}^o - X_{\tau}^* \rVert^2 + \frac{4}{p+\delta}C.\nonumber
	\end{equation}
	Using the Lipschitz continuity of $f(\cdot)$, it can be written that
	\begin{equation}
	    \lVert X_{\tau}^o - X_{\tau}^* \rVert^2 = 2k_f \lVert X_{\tau-1}^o - \hat{X}_{\tau-1}^* \rVert^2 + 2r_{\mu}.\nonumber
	\end{equation}
Hence,
\begin{equation*}
    \lVert X_{\tau}^o - \hat{X}_{\tau}^* \rVert^2 \leq \zeta_{\tau}.
\end{equation*}
It can also be deduced that if $\zeta_m < \zeta_{m-1}$ and $a(p,\delta)<1$, then $\zeta_m$ tends to $\frac{\beta}{1-a(p,\delta)}$ as $m \longrightarrow +\infty$ (please see Theorem~1 from~\cite{alessandri1999neural}), where $\beta~=~ \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu} $. 	
\end{proof}

The following section presents the derivation of the analytical expression for calculating the covariances using the path information. This result will be later used for predicting covariances for the NMPC cost function.

==> Cooperative localization MPC/nmpc_2c.tex <==
\section{NMPC formulation}\label{sec:NMPC}
NMPC is a state-of-the-art technique for real-time optimal control. At each time step, the constrained optimization problem is solved based on the plant model for a finite time horizon, and the procedure is repeated with states updated through feedback in the next iteration~\cite{MPCbook}. Fig.~\ref{fig:block} shows the block diagram of the NMPC scheme used in this paper. The optimal control sequence is computed for the prediction horizon $ \tau_h $ from which only the first action is applied to the system at each time step. 
	 
%	\begin{figure}[h]
%		\centering
%		\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%		\caption{NMPC block diagram }
%		\label{fig:block}
%	\end{figure}
	
 A point mass kinematic model is considered for the vehicles. We assume that the altitude and velocities of the AAVs remain constant during transit. The general kinematic model is given as
	\begin{equation}
	\dot{X} =
	\begin{bmatrix}
	v\cos \psi_1   \\
	v\sin \psi_1\\
	\omega_1 \\
	\vdots \\
	v\cos \psi_{n_v}   \\
	v\sin \psi_{n_v}\\
	\omega_{n_v} \\        
	\end{bmatrix},
	\end{equation}  
 where  $ v $ is the linear velocity, $ \psi $ the heading angle, $ \omega $ the angular velocity, and $ n_v $ is the number of vehicles.
	
The objective function for the NMPC is defined as
	\begin{equation}
	\min_{\boldsymbol{\omega_1 \cdots \omega_{n_v}} \in \mathcal{PC}(t,t+\tau_h)}J=\int_{t}^{t+\tau_h}\sum_{i=1}^{n_v} \left[ C_{1_i}+W_iC_{2_i}\right], 
	\label{eq:PI}
	\end{equation}	
	subject to:
	\begin{align*}
	\dot{X} &= f(X,\boldsymbol{\omega}),\\
	\boldsymbol{\omega} & \in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
	where 
	\begin{equation}
	C_{1_i}=(x_i-x_{D_i})^{2}+(y_i-y_{D_i})^{2}, \label{eq:C1}
	\end{equation}
is the cost associated with minimizing the distance between the vehicle and the destination. $(x_i,y_i) $ is the position of the $ i^{th} $ vehicle and $ (x_{D_i},y_{D_i}) $ are their respective destination points. $ \boldsymbol{\omega}^{-} $ and $ \boldsymbol{\omega}^{+}$ are the lower and upper bounds of $\boldsymbol{\omega}$, and $ \mathcal{PC}(t,t+\tau_h) $ denotes the space of piece-wise continuous function defined over the time interval $ \left[ t,t+\tau_h\right]  $. 
$C_{2_i}$ is the cost to ensure the estimation covariance is within a  bound. It is defined as:
	\begin{equation}
	C_{2_i}=\begin{cases}
	0, & \text{if $\lambda_i \geq \eta$}.\\
	(\eta-\lambda_i)^{2}, & \text{ otherwise}.
	\end{cases} \label{eq:C2}
	\end{equation} 
where $ \eta $ is a tuning parameter related to the number of connections required. Increasing $ \eta $ will result in vehicles moving closer to the landmarks and increase the connections. For satisfactory localization, observability conditions should be satisfied, which require connections with at least two landmarks~\cite{sharma2014observability}. Hence, the value of $\eta$ should be selected as~$ \eta \geq 2 $. The parameter $\lambda_i $ is the second smallest eigenvalue of the Laplacian matrix which is formed as:
	\begin{equation}
	L_i(X)=\Delta_i(X)-A_i(X),
	\end{equation} 
where $ A_i(X) $ is the adjacency matrix defined similar to~\cite{de2006decentralized} as
	\begin{equation}
	A_{i_{mn}}=\begin{cases}
	e^{\frac{-\kappa(||R_{mn}||-\rho)}{R_{s}-\rho}}, & \text{$\left| \left| R_{mn}\right| \right| \leq R_s$}.\\
	0, & \text{$\left| \left| R_{mn}\right| \right| > R_s$}.
	\end{cases}
	\end{equation} 
	and
	$ \Delta_i(X) $ is a diagonal matrix with elements
	\begin{equation}
	\Delta_{i_{mm}}=\sum_{n=1}^{N}A_{i_{mn}}
	\end{equation}
where $ m,n= 1  $ to $ N $, and $ N $ is the number of nodes of the graph connecting the vehicles and landmarks. $ \kappa $ is a constant which determines the convergence rate of the exponential function, and $\rho$ is used to set a minimum distance between the landmarks and the vehicles to avoid collisions. $ ||R_{mn}|| $ is the distance between the $ m^{th} $ and $ n^{th} $ nodes, and $ R_s $ is the sensor range of the vehicles. This formulation of the adjacency matrices, rather than updating it with binary values, helps drive the vehicles closer to the landmarks than just maintaining the connections by keeping them in the sensor range and reducing the distance between the landmarks and the vehicles help in decreasing the estimation covariance as explained in sec.~\ref{sec:analysis}. The maximum value $ \lambda_i $ can take is equal to the number of connections of each vehicle, and this insight is used in formulating (\ref{eq:C2}).   
	
The weight $W_i$ associated with $ C_{2_i} $ is defined in the following way
	\begin{equation}
	W_i=\begin{cases}
	W, & \text{if $3\sigma_{p_i} \geq \sigma_c$}.\\
	0, & \text{ otherwise}.
	\end{cases}\label{eq:Wi}
	\end{equation} 
where $\sigma_{p_i}$ is the standard deviation in the estimated position of the $ i^{th} $ vehicle and the constant $\sigma_c$ is the specified critical value. This adaptive weight formulation is used to obtain a trade-off between the two objectives. $\sigma_{p_i} $s are calculated using the expression
\begin{eqnarray}
\sigma_{p_i}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_i-\theta_g))} \right)+\nonumber\\(R_g^2+R_g^4)\csc^2(\psi_i-\theta_g), \nonumber
\label{eq:s_bearing_i}
\end{eqnarray} 
which is explained in detail in section \ref{sec:b_measurement}. The terms $C_1$ and $ C_2 $ of the objective function (\ref{eq:PI}) is normalized as follows:
	\begin{eqnarray}
	C_1(t)&=&\left(\frac{C_1(t) - \min(C_1(t))}{\max(C_1(t)) - \min(C_1(t))}\right),\label{eq:c1t}\\
	C_2(t)&=&\left(\frac{C_2(t) - \min(C_2(t))}{\max(C_2(t)) - \min(C_2(t))}\right).\label{eq:c2t}
	\end{eqnarray}
The NMPC objective function given equation \eqref{eq:PI} uses the expressions given in equations \eqref{eq:C1}\eqref{eq:C2}\eqref{eq:Wi}\eqref{eq:c1t} and equation \eqref{eq:c2t}. The NMPC objective function is solved along with state and control constraints. 
	

==> Cooperative localization MPC/obs_2c.tex <==
\section{Covariance calculation}\label{sec:analysis}
% We show in Theorem.~\ref{thm:covariance} that the covariance of the vehicle states $ p_{ij} $ is proportional to the sum of edges leading to the landmarks as $ p_{ij} = \sum \frac{1}{\epsilon_s} $. Since information matrices can be added together (see the proof for Corollaries \ref{cor:path} and \ref{cor:landmark}), it is possible to combine the split sections of the graph, and hence the analysis carried out for the individual sections can be generalized for the complete graph.

% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config2.eps}
% 		\caption{Example configuration of two vehicles and two landmarks.}
% 		\label{fig:config2}
% 	\end{figure}

Consider an example configuration of two vehicles as shown   in Fig.~\ref{fig:3a}(i), where the vehicles are represented by $1$ and $2$ and two landmarks by $a$ and $b$. In order to understand how the paths/connections/measurements from a landmark to a vehicle influence the uncertainty of the vehicle states, we consider each landmark separately and analyze. Consider the segment $a-1-2$ of the graph in Fig.~\ref{fig:3a}(i), as shown in Fig.~\ref{fig:3a}(ii). The observability matrix for the system can be written as
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 \\
o12 & -o12
\end{bmatrix},
\end{equation}
where $oa1,o12$, and $-o12$ are the derivatives of the measurements with respect to the vehicle states. For example, $oa1$ is the derivative of the measurement between the landmark $a$ and the vehicle-$1$ with respect to the vehicle-$1$. Since there is no measurement between the landmark $a$ and the vehicle-$2$, the corresponding entry ($O_{12}$) is zero. Note that the size of $O$ depends on the number of edges and it may not be a square matrix. Assuming the measurement covariance matrix $ \Gamma = I $, and zero-mean white Gaussian noise, the observability grammian is defined as $ O^TO $ and the covariance matrix $ P $ is written as %\cite{hinson2014observability,crassidis2004optimal}
\begin{eqnarray}
P &\leq& (O^T\Gamma^{-1}O)^{-1}, \\
%&\leq& (O^TO)^{-1},\\
 &\leq& \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2} \\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \label{eq:p2a}
\end{bmatrix}.
\end{eqnarray}
The first element of the $P$ matrix corresponds to the vehicle-$1$ connecting to the landmark $a$, hence $oa1$ (let us discard the square and fraction for easy understanding). The element $ \frac{1}{o12^2}+\frac{1}{oa1^2} $ of the $P$ matrix corresponds to the vehicle-$2$. Observing that it is connected to the landmark $a$ through vehicle-$1$, we can see both $oa1$ and $o12$ are present in the entry. Next, we consider the section $1-2-b$ of the graph, as shown in Fig.~\ref{fig:3a}(iii). The observability and covariance matrices for the system are written as
\begin{eqnarray}
O = \begin{bmatrix}
0 & ob2 \\
o12 & -o12 
\end{bmatrix},
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} \\
\frac{1}{ob2^2} & \frac{1}{ob2^2}  \label{eq:p2b}
\end{bmatrix}.
\end{eqnarray}
%\begin{equation}
%P \leq \begin{bmatrix}
%\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} \\
%\frac{1}{ob2^2} & \frac{1}{ob2^2}  \label{eq:p2b}
%\end{bmatrix}.
%\end{equation}
The first element of $P$ indicates that vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$. The last entry shows that vehicle-$2$ is directly connected to the landmark $b$ and hence  only $ob2$ is present. 
	\begin{figure*}
		\centering
		\begin{subfigure}{4cm}
		\includegraphics[width=4cm]{figs/config2.eps}
		\caption{}\label{fig:3a}
		\end{subfigure}\hspace{10mm}
			\begin{subfigure}{4cm}
		\includegraphics[width=4cm]{figs/config3.eps}
				\caption{} \label{fig:3b}
		\end{subfigure}\hspace{10mm}
%			\begin{subfigure}{3cm}
%		\includegraphics[width=4cm]{figs/config4.eps}
%				\caption{}
%		\label{fig:config4}
%	\end{subfigure}\hspace{10mm}
	\begin{subfigure}{4cm}
		\includegraphics[width=6cm]{figs/config5.eps}
				\caption{}
		\label{fig:config5}
	\end{subfigure}
		\caption{(a) Different configurations of two vehicles and two landmarks. (b) Different configuration of the system with 3 vehicles and 2 landmarks %(c) Example configuration of four vehicles and two landmarks. 
			(c) Notations for a general multi-vehicle-landmark RPMG.}
		\label{fig:config2}
	\end{figure*}



% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=6cm,height=4cm]{figs/config3.eps}
% 		\caption{Example configuration of three vehicles and two landmarks.}
% 		\label{fig:config3}
% 	\end{figure}

Next, we extend similar analysis for a three vehicle configuration  as shown in Fig.~\ref{fig:3b}(i). Consider the section $3-a-1-2$ of the graph, shown in Fig.~\ref{fig:3b}(ii). The observability matrix and covariance matrix $P $ for this configuration are 
\begin{eqnarray}
O = \begin{bmatrix}
oa1 & 0 & 0 \\
o12 & -o12 & 0\\
0 & 0 & oa3
\end{bmatrix},
\label{eq:ob_config3}
P \leq \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2}  & 0\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & 0\\
0 & 0 & \frac{1}{oa3^2}  \label{eq:p3a}
\end{bmatrix}.\nonumber
\end{eqnarray} 
%The covariance matrix $ P $ is given by
%\begin{equation}
%P \leq \begin{bmatrix}
%\frac{1}{oa1^2} & \frac{1}{oa1^2}  & 0\\
%\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & 0\\
%0 & 0 & \frac{1}{oa3^2}  \label{eq:p3a}
%\end{bmatrix}.
%\end{equation}
The first element of the $P$ matrix contain only $oa1$ since the vehicle-$1$ is directly connected to the landmark $a$. The vehicle-$2$ is connected to the landmark $a$ through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. Since vehicle-$3$ is directly connected to the landmark, the last element of $P$ contains only $oa3$ as expected. Now, let us take the section $1-2-b-3$ of the graph, shown in Fig.~\ref{fig:3b}(iii). The observability and covariance matrices are given by
\begin{eqnarray}
O = \begin{bmatrix}
0 & ob2 & 0 \\
o12 & -o12 & 0 \\
0 & 0 & ob3
\end{bmatrix},
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0 \\
\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0\\
0 & 0 & \frac{1}{ob3^2}  \label{eq:p3b}
\end{bmatrix}.\nonumber
\end{eqnarray}
%\begin{equation}
%P \leq \begin{bmatrix}
%\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0 \\
%\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0\\
%0 & 0 & \frac{1}{ob3^2}  \label{eq:p3b}
%\end{bmatrix}.
%\end{equation}
Vehicle-$2$ and vehicle-$3$ are directly connected to the landmark $b$. Therefore, the corresponding entries in the $P$ matrix contains only $ob2$ and $ob3$. The vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$ and this information is clearly reflected in the first entry of $P$.

% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config4.eps}
% 		\caption{Example configuration of four vehicles and two landmarks.}
% 		\label{fig:config4}
% 	\end{figure}

%We conclude this analysis by taking a configuration with four vehicles and two landmarks as shown in Fig.~\ref{fig:config4}(i). The observability matrix for the sub-configuration with the landmark $a$ and the vehicles $1,2,3,4$, shown in Fig.~\ref{fig:config4}(ii) is given by
%\begin{equation}
%O = \begin{bmatrix}
%oa1 & 0 & 0 & 0 \\
%o12 & -o12 & 0 & 0\\
%0 & o23 & -o23 & 0\\
%0 & o24 & 0 & -o24
%\end{bmatrix}.
%\end{equation}  
%The covariance matrix $ P $ is given by
%{\tiny
%\begin{equation}
%P \leq \begin{bmatrix*}[l]
%\frac{1}{oa1^2} & \frac{1}{oa1^2}  &  \frac{1}{oa1^2} & \frac{1}{oa1^2}\\
%\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2}\\
%\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o23^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \\ 
%\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{oa1^2}  
%\end{bmatrix*}. \label{eq:p4a}
%\end{equation}}
%
%The vehicle-$1$ is directly connected to the landmark $a$, hence the first element of the $P$ matrix contain only $oa1$. The vehicle-$2$ is connected to the landmark through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $1$ and $2$, which is reflected in the $P$ matrix by the presence of $o12,o23$, and $oa1$. It is to be noted that the term $o24$ is absent as expected since the vehicle-$4$ is not involved in the path for vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$4$, since it is connected to the landmark through the vehicles $2$ and $1$. The entry contains $o12,o24$, and $oa1$ corresponding to the path $4-2-1-a$. Next, consider the sub-configuration with the landmark $b$, shown in Fig.~\ref{fig:config4}(iii). The observability and covariance matrices for this configuration are given by
%
%{\tiny
%\begin{eqnarray}
%O &=& \begin{bmatrix}
%0 & 0 & 0 & ob4 \\
%o12 & -o12 & 0 & 0 \\
%0 & o23 & -o23 & 0 \\
%0 & o24 & 0 & -o24
%\end{bmatrix},\nonumber\\
%P &\leq& \begin{bmatrix*}[l]
%\frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
%\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2}\\
%\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o23^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
%\frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2}
%\end{bmatrix*}.   \label{eq:p4b}\nonumber
%\end{eqnarray}}
%The vehicle-$4$ is directly connected to the landmark $b$, hence the fourth diagonal element of the $P$ matrix contain only $ob4$. The vehicle-$2$ is connected to the landmark through vehicle-$4$, hence both $o24$ and $ob4$ can be seen in the second diagonal element of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $2$ and $4$, which is reflected in the third diagonal element of the $P$ matrix by the presence of $o23,024$, and $ob4$. We can see that the term $o12$ is absent as expected since the vehicle-$1$ is not involved in the path for the vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$1$, since it is connected to the landmark through the vehicles $2$ and $4$. The entry contains $o12,o24$, and $ob4$ correspondingly.

% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config5.eps}
% 		\caption{Notations for a general multi-vehicle-landmark RPMG.}
% 		\label{fig:config5}
% 	\end{figure}

Using the above example configuration analysis, we can further extend the analysis to a general result with $n_v$ vehicle and $n_l$ landmarks as shown in Fig.~\ref{fig:config5}. The landmarks are represented using stars, and the vehicles are represented using triangles. All the vehicles are denoted by  $i,i+1,\ldots,n_v$, landmarks as $j,j+1,\ldots,n_l$, and edges connecting the vehicles and landmarks as $\epsilon_s,\epsilon_{s+1},\ldots,\epsilon_{n_e}$, where $i=j=s=1$. The observability vector associated with an edge/measurement is represented using $\epsilon$ with the edge number as subscript for simplicity. For example, the observability vector between landmark-$j$ and vehicle-$i$, $oji$ is represented by $\epsilon_s$. Now, the following theorem for a general RPMG can be stated. 

\begin{theorem}\label{thm:covariance}
The covariance associated with the vehicle-$i$, $i=1,\ldots,n_v$, due to the landmark-$j$, $j=1,\ldots,n_l$, is given by 
\begin{equation}
    p_{ij} = \sum_{s \in \mathcal{S}} \frac{1}{\epsilon_s},
\end{equation}
where $s=1,\ldots,n_e$, $\mathcal{S}$ is the set of edges that forms a path from vehicle-$i$ to the landmark-$j$, $n_v$ is the number of vehicles, $n_l$ is the number of landmarks, and $n_e$ is the number of edges in the RPMG.
\end{theorem}
\begin{proof}
The covariances associated with each vehicle for a two-vehicle-two-landmark configuration is given by equations \eqref{eq:p2a} and \eqref{eq:p2b}, followed by three vehicles in \eqref{eq:p3a} and \eqref{eq:p3b}. The relation given in Theorem~\ref{thm:covariance} is clearly reflected in the elements of the corresponding covariance matrices. The generalization to $n_v$ vehicles and $n_l$ landmarks is straightforward from the previous analysis.

However, we prove the theorem through  contradiction. Consider Fig.~\ref{fig:3b}(ii). According to Theorem~\ref{thm:covariance}, the term/edge $\frac{1}{oa1^2}$ should be present in $p_{2a}$. Suppose we write the $P$ matrix without that term. The new $P$ matrix and the original $P$ matrix found by observability analysis given by \eqref{eq:p3a} is written side-by-side showing only the element corresponding to $p_{2a}$.  
\begin{equation}
 \begin{bmatrix}
	\cdots & \cdots  & \cdots\\
	\cdots & \frac{1}{o12^2} & \cdots\\
	\cdots & \cdots & \cdots  
\end{bmatrix},
 \begin{bmatrix}
	\cdots & \cdots  & \cdots\\
	\cdots & \frac{1}{o12^2}+\frac{1}{oa1^2} & \cdots\\
	\cdots & \cdots & \cdots  \label{eq:old_new_p3a}
\end{bmatrix}.
\end{equation}

The new $O^TO$ matrix for the system found by inverting the first $P$ matrix will be
\begin{equation}
	O^TO = \begin{bmatrix}
		\frac{oa1^4}{-o12^2+oa1^2} & \frac{o12^2 oa1^2}{o12^2-oa1^2}  & 0\\
		\frac{o12^2 oa1^2}{o12^2-oa1^2} & \frac{o12^2 oa1^2}{-o12^2+oa1^2} & 0\\
		0 & 0 & \frac{1}{oa3^2}  \label{eq:proof1}
	\end{bmatrix},
\end{equation}
which contradicts with the $O^TO$ matrix derived from equation~ \eqref{eq:ob_config3}, which is 
\begin{equation}
 \begin{bmatrix}
		o12^2+oa1^2 & -o12^2  & 0\\
		-o12^2& o12^2 & 0\\
		0 & 0 & oa3^2  
	\end{bmatrix}.
\label{eq:oto_proof}
\end{equation}
Similarly, if an additional term $\frac{1}{oa3^2}$ is present in $p_{2a}$, the corresponding $O^TO$ matrix for the system will be
\begin{equation}
	O^TO = \begin{bmatrix}
		oa1^2+\frac{o12^2oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2}  & 0\\
		-\frac{o12^2 oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2} & 0\\
		0 & 0 & oa3^2  \label{eq:proof2}
	\end{bmatrix},
\end{equation}
which also contradicts with the $O^TO$ matrix given in~\eqref{eq:oto_proof}.
Hence, the relation given in Theorem~\ref{thm:covariance} is always true.
\end{proof}

The following corollaries can be written from Theorem~\ref{thm:covariance}.

\begin{corollary}\label{cor:path}
If there is more than one path from a landmark to a vehicle, and these paths are numbered from $1$ to $g_{ij}$, where $g_{ij}$ is the total number of paths from the landmark-$j$ to the vehicle-$i$, then the total covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert  p_{ij} \right\rVert  \leq \sum_{\kappa=1}^{g_{ij}} \left\lVert p_{ij}^{\kappa} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_{ij} = \sum_{\kappa=1}^{g_{ij}} p_{ij}^{\kappa},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $p_{ij}^{\kappa}$ is the covariance of the vehicle-$i$ due to the landmark-$j$ considering only the path-$\kappa$.
\end{corollary}

\begin{corollary}\label{cor:landmark}
If there is more than one landmark connected to a vehicle, then the covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert p_i \right\rVert  \leq \sum_{j \in \mathcal{J}} \left\lVert p_{ij} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_i  = \sum_{j \in \mathcal{J}} p_{ij},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $\mathcal{J}$ is the set of landmarks connected to the vehicle-$i$.
\end{corollary}

\begin{proof}
The method to calculate covariances for Corollary~\ref{cor:path} and \ref{cor:landmark} is given in Theorem~\ref{thm:covariance}. The summation is based on the properties of the information matrix given as follows~\cite{fisher,zegers2015fisher} 
% When information matrices are added, the resulting value will be greater than or equal to the sum of values of the individual matrices. That is, information is not lost through addition. 

If $X=(X_1,X_2,\ldots,X_n)$ and $X_1,X_2,\ldots,X_n$ are independent random variables, then $I_X(\alpha)=I_{X_1}(\alpha)+I_{X_2}(\alpha)+\ldots I_{X_n}(\alpha)$, where $I_x(\alpha)$ is the information matrix defined as 
\begin{equation*}
	I_x(\alpha) = E_{\alpha}\left[ \left( \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right) ^2\right] = \mathrm{Var}_{\alpha}\left(  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right).
\end{equation*}
Since \[f(x|\alpha) = \prod_{i=1}^{n}f_i(x_i|\alpha),\] where $f_i(\cdot|\alpha)$ is the pdf of $X_i$,
\begin{eqnarray}
\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right] &=& \sum_{i=1}^{n}\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f_i(X_i|\alpha)\right], \nonumber \\
I_X(\alpha) &=& \sum_{i=1}^{n}I_{X_i}(\alpha). \nonumber 
\end{eqnarray} 

 Since covariance is the inverse of information, we can find the total covariance associated with each vehicle by adding the components from all the paths and landmarks.
\end{proof}

In the next sub-sections, we show how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements. 
% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config1.eps}
% 		\caption{Example configuration }
% 		\label{fig:config1}
% 	\end{figure}
% Consider an example configuration given in Fig.~\ref{fig:config1}. The vehicles $ 1 $ and $ 2 $ are connected to landmarks $a$ and $b$. The observability matrix for the system can be written as
% \begin{equation}
% O = \begin{bmatrix}
% O1a \\
% O2b \\
% O12
% \end{bmatrix},
% \end{equation}
% where 
% \begin{eqnarray}
% O1a &=& \begin{bmatrix}
% o1a & 0
% \end{bmatrix}, \\
% O2b &=& \begin{bmatrix}
% 0 & o2b
% \end{bmatrix}, \\
% O12 &=& \begin{bmatrix}
% o12 & -o12
% \end{bmatrix}.
% \end{eqnarray}  
% Assuming the measurement covariance matrix $ \Gamma = I $, the observability grammian can be defined as $ O^TO $ and the covariance matrix $ P $ can be found as \cite{hinson2014observability}
% \begin{equation}
% P = (O^TO)^{-1},
% \end{equation}
% which can be written as
% \begin{equation}
% P = \begin{bmatrix}
% P(1,1) & P(1,2) \\
% P(2,1) & P(2,2)
% \end{bmatrix},
% \end{equation}
% where
% %{\tiny
% \begin{eqnarray}
% P(1,1) &=& (o12^2 + o2b^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(1,2) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,1) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,2) &=& (o12^2 + o1a^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2).
% \end{eqnarray}
% %}%
% Looking at the elements of $P$, we can clearly see that the covariance is related to the connection/path. In the next sections, we try to find out how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements.   

\subsection{Range measurements}
%	\begin{figure}
%		\centering
%		\includegraphics[width=8cm]{figs/config1.eps}
%		\caption{Example configuration }
%		\label{fig:config1}
%	\end{figure}
Consider the configuration given in Fig.~\ref{fig:config2}(i). The vehicle kinematics are defined as
\begin{eqnarray}
\dot{x}_i &=& v \cos{\psi_1}, \nonumber \\
\dot{y}_i &=& v \sin{\psi_1}, 
%\dot{x}_2 &=& v \cos{\psi_2}, \\
%\dot{y}_2 &=& v \sin{\psi_2}, 
\end{eqnarray} 
where $i=1,2$ with range measurements
\begin{eqnarray}
h_{1a} &=& \sqrt{(x_1 - x_a)^2 + (y_1 - y_a)^2}, \\
h_{12} &=& \sqrt{(x_1 - x_2)^2 + (y_1 - y_2)^2}, \\
h_{2b} &=& \sqrt{(x_2 - x_b)^2 + (y_2 - y_b)^2},
\end{eqnarray}
and we derive the observability matrix using the Lie derivatives~ \cite{sharma2011graph}. To simplify the representation we denote $x_{1a}=(x_1 - x_a),x_{12}=(x_1 - x_2) ,x_{2b}=(x_2 - x_b)$, $y_{1a}=(y_1 -y_a),y_{12}=(y_1 - y_2) ,y_{2b}=(y_2 - y_b)$. 
Define 
\begin{equation}
f_L = \begin{bmatrix}
\cos{\psi_1} 
\sin{\psi_1} 
\cos{\psi_2} 
\sin{\psi_2} 
\end{bmatrix}',
\end{equation}
and the vehicle kinematics can be represented as
\begin{equation}
\dot{X} = vf_L.
\end{equation}
The gradient of zero\textsuperscript{th} order Lie derivatives are given as
\begin{eqnarray}
H_{1a} = \begin{bmatrix}
\frac{x_{1a}}{R_{1a}} & \frac{y_{1a}}{R_{1a}} & 0 & 0 
\end{bmatrix}, 
H_{2b} = \begin{bmatrix}
& 0 & 0 & \frac{x_{2b}}{R_{2b}} & \frac{y_{2b}}{R_{2b}}  
\end{bmatrix},\nonumber\\
H_{12} =\begin{bmatrix}
\frac{x_{12}}{R_{12}} & \frac{y_{12}}{R_{12}} & \frac{-(x_{12})}{R_{12}} & \frac{-(y_{12})}{R_{12}} 
\end{bmatrix}, \nonumber
\end{eqnarray}
where $R_{(\cdot)} $ is the distance between nodes.
The gradient of first order Lie derivatives are given as

%\begin{eqnarray}
%\frac{\partial }{\partial X}\left( \frac{\partial h_{1a}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
%\frac{(y_1-y_a)^2 C\psi_1 -(x_1-x_a)(y_1-y_a) S\psi_1}{R_{1a}^3} &
% \frac{(x_1-x_a)^2 S\psi_1-(x_1-x_a)(y_1-y_a) C\psi_1}{R_{1a}^3}& 0 & 0 
%\end{bmatrix},\nonumber\\
%\frac{\partial }{\partial X}\left( \frac{\partial h_{2b}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
%0 & 0 & \frac{(y_2-y_b)^2 C\psi_2 + (-x_2+x_b)(y_2-y_b) S\psi_2}{R_{2b}^3} &
%\frac{(x_2-x_b)^2 S\psi_2 + (-y_2+y_b)(x_2-x_b) C\psi_2}{R_{2b}^3} 
%\end{bmatrix},\\
%\frac{\partial }{\partial X}\left( \frac{\partial h_{12}}{\partial X}  \cdot f \right) &=& 
%[\begin{matrix}
%\frac{-2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix} \nonumber \\
%& & \begin{matrix} 
%\frac{2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \nonumber\\
%& & \begin{matrix}
%\frac{2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix} \nonumber \\
%& & \begin{matrix}
%\frac{-2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}]\nonumber,
%\end{eqnarray}}
%%%%%%%%%% revised to fit in the column
%\resizebox{\linewidth}{!}{
%	  \begin{minipage}{\linewidth}
%\begin{align*}
%\frac{\partial }{\partial X}\left( \frac{\partial h_{1a}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
%\frac{(y_1-y_a)^2 C\psi_1 -(x_1-x_a)(y_1-y_a) S\psi_1}{R_{1a}^3} &
%\frac{(x_1-x_a)^2 S\psi_1-(x_1-x_a)(y_1-y_a) C\psi_1}{R_{1a}^3}& 0 & 0 
%\end{bmatrix},\nonumber\\
%\frac{\partial }{\partial X}\left( \frac{\partial h_{2b}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
%0 & 0 & \frac{(y_2-y_b)^2 C\psi_2 + (-x_2+x_b)(y_2-y_b) S\psi_2}{R_{2b}^3} &
%\frac{(x_2-x_b)^2 S\psi_2 + (-y_2+y_b)(x_2-x_b) C\psi_2}{R_{2b}^3} 
%\end{bmatrix},\\
%\frac{\partial }{\partial X}\left( \frac{\partial h_{12}}{\partial X}  \cdot f \right) &=& 
%[\begin{matrix}
%\frac{-2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix} \nonumber \\
%& & \begin{matrix} 
%\frac{2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \nonumber\\
%& & \begin{matrix}
%\frac{2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix} \nonumber \\
%& & \begin{matrix}
%\frac{-2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}]\nonumber,
%\end{align*}
%  \end{minipage}
%}
		\begin{align}
		\frac{\partial }{\partial X}\left( \frac{\partial h_{1a}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
		\frac{(y_{1a})^2 C\psi_1 -(x_{1a})(y_{1a}) S\psi_1}{R_{1a}^3} \\
		\frac{(x_{1a})^2 S\psi_1-(x_{1a})(y_{1a}) C\psi_1}{R_{1a}^3}\\ 0 \\ 0 
		\end{bmatrix},\nonumber
				\end{align}
				\begin{align}
		\frac{\partial }{\partial X}\left( \frac{\partial h_{2b}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
		0 \\ 0 \\ \frac{(y_{2b})^2 C\psi_2 + (-x_{2b})(y_{2b}) S\psi_2}{R_{2b}^3} \\
		\frac{(x_{2b})^2 S\psi_2 + (-y_{2b})(x_{2b}) C\psi_2}{R_{2b}^3} 
		\end{bmatrix},\nonumber
				\end{align}{
						\begin{align}
		\frac{\partial }{\partial X}\left( \frac{\partial h_{12}}{\partial X}  \cdot f \right) &=& 
	\begin{bmatrix}
		\frac{-2(y_{12}) S(\frac{\Delta\psi^-}{2})((x_{12}) C(\frac{\Delta\psi^+}{2}) + (y_{12}) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \\
		\frac{2(x_{12}) S(\frac{\Delta\psi^-}{2})((x_{12}) C(\frac{\Delta\psi^+}{2}) + (y_{12}) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \\
		\frac{2(y_{12}) S(\frac{\Delta\psi^-}{2})((x_{12}) C(\frac{\Delta\psi^+}{2}) + (y_{12}) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \\
		\frac{-2(x_{12}) S(\frac{\Delta\psi^-}{2})((x_{12}) C(\frac{\Delta\psi^+}{2}) + (y_{12}) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{bmatrix}\nonumber,
		\end{align}}
where $ \sin $ and $ \cos $ are abbreviated as $S$ and $C$, $ \Delta\psi^- = \psi_1-\psi_2 $, and $ \Delta\psi^+ = \psi_1+\psi_2 $.

Observability matrix is formed by using Lie derivatives up to first order as
\begin{equation}
O = \begin{bmatrix}
\nabla L^0 \\
\nabla L^1
\end{bmatrix},
\end{equation} 
where $L^0$ and $L^1$ are the zero\textsuperscript{th} and first order Lie derivatives respectively. The covariance matrix $P$ is found by inverting $ O^TO $ with the assumption of $\Gamma=I$.

The standard deviation in $x$ direction for the first vehicle can be found by taking the square root of the first element of the $P$ matrix,
\begin{equation}
\sigma_{x_1} = \sqrt{P(1,1)}.
\end{equation} 
Similarly, the standard deviation in the $y$ direction and the combined position uncertainty can be found as
\begin{eqnarray}
\sigma_{y_1} &=& \sqrt{P(2,2)},\\
\sigma_{p_1} &=& \sqrt{\sigma_{x_1}^2 + \sigma_{y_1}^2}.
\end{eqnarray}

Since the derived $P$ matrix is very large with several terms, we consider some simplifying assumptions to formulate an approximate relation. All the distance terms were substituted with a single average value. The resulting relation is given as
\begin{equation}
\sigma_{p_1} = \sqrt{\frac{2}{3}+R_g^2 \csc^2{(\psi_1-\theta_g)}},
\label{eq:s_range}
\end{equation}
where $R_g,\theta_g$ are the average value of distance and LOS angle. It is evident from the relation that the covariance of vehicle depends on the distances from the landmarks and the LOS angles to them. As the distance increases, the covariance also increases. Similarly, $ \sigma_p $ of other vehicles can also be found. 
\subsection{Bearing measurements}\label{sec:b_measurement}
Let's extend the vehicle model to contain three states. The new model is given as
\begin{eqnarray}
\dot{x}_i &=& v \cos{\psi_i}, \nonumber\\
\dot{y}_1 &=& v \sin{\psi_i}, \nonumber\\
\dot{\psi}_i &=& \omega_i, \nonumber 
%\dot{x}_2 &=& v \cos{\psi_2}, \\
%\dot{y}_2 &=& v \sin{\psi_2}, \\
%\dot{\psi}_2 &=& \omega_2, 
\end{eqnarray}
where vehicle $i=1,2$. With the same configuration as in Fig.~\ref{fig:config2}(i), define bearing measurement equations as
\begin{eqnarray}
h_{a1} &=& \arctan\left( \frac{y_a-y_1}{x_a-x_1}\right) - \psi_1, \\
h_{b2} &=& \arctan\left( \frac{y_b-y_2}{x_b-x_2}\right) - \psi_2, \\
h_{12} &=& \arctan\left( \frac{y_1-y_2}{x_1-x_2}\right) - \psi_2, \\
h_{21} &=& \arctan\left( \frac{y_2-y_1}{x_2-x_1}\right) - \psi_1, 
\end{eqnarray}
the gradient of zeroth order Lie derivatives are given as
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{-(y_1 - y_a)}{R_{a1}^2} & \frac{x_1 - x_a}{R_{a1}^2} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{-(y_2 - y_b)}{R_{b2}^2} & \frac{x_2 - x_b}{R_{b2}^2} & -1  
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{12}^2} & \frac{x_1 - x_2}{R_{12}^2} & 0 & \frac{y_1 - y_2}{R_{12}^2} & \frac{x_2 - x_1}{R_{12}^2} & -1 
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{21}^2} & \frac{x_1 - x_2}{R_{21}^2} & -1 & \frac{y_1 - y_2}{R_{21}^2} & \frac{x_2 - x_1}{R_{21}^2} & 0 
\end{bmatrix}, \hspace{6mm}
\end{eqnarray} 
using the geometry, the equations are changed to make it in terms of LOS angles as follows
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{\sin\theta_{a1}}{R_{a1}} & \frac{-\cos\theta_{a1}}{R_{a1}} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{\sin\theta_{b2}}{R_{b2}} & \frac{-\cos\theta_{b2}}{R_{b2}} & -1 
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{-\sin\theta_{12}}{R_{12}} & \frac{\cos\theta_{12}}{R_{12}} & 0 & \frac{\sin\theta_{12}}{R_{12}} & \frac{-\cos\theta_{12}}{R_{12}} & -1  
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{\sin\theta_{21}}{R_{21}} & \frac{-\cos\theta_{21}}{R_{21}} & -1 & \frac{-\sin\theta_{21}}{R_{21}} & \frac{\cos\theta_{21}}{R_{21}} & 0  
\end{bmatrix}. \hspace{6mm}
\end{eqnarray} 
Define 
\begin{eqnarray}
f_v &=& \begin{bmatrix}
\cos{\psi_1}~ \sin{\psi_1} ~0~ \cos{\psi_2} ~\sin{\psi_2} ~0 
\end{bmatrix}',\nonumber\\
f_{\omega_1} &=& \begin{bmatrix}
0 \quad
0 \quad
1\quad
0 \quad
0\quad
0 
\end{bmatrix}',\nonumber\\
f_{\omega_2} &=& \begin{bmatrix}
0 \quad
0 \quad
0\quad
0 \quad
0\quad
1 
\end{bmatrix}',\nonumber
\end{eqnarray}
and the dynamics can be represented as
\begin{equation}
\dot{X} = \begin{bmatrix}
\dot{X}_1 \\
\dot{X}_2
\end{bmatrix}
= f_vv+f_{\omega_1}\omega_1 + f_{\omega_2}\omega_2,
\end{equation}
and a similar procedure to the range measurement case is followed to find the first order Lie derivatives, observability grammian and covariance matrix $P$. The covariance in position of the first vehicle is given by
\begin{eqnarray}
\sigma_{p_1}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_1-\theta_g))} \right)+\nonumber\\ (R_g^2+R_g^4)\csc^2(\psi_1-\theta_g). \nonumber
\label{eq:s_bearing}
\end{eqnarray} 
Similarly, $ \sigma_p $ of other vehicles can also be found. This approximate closed form covariance is used in the NMPC as Step 2 in Fig. \ref{fig:block}(a).

%\subsection{Results}
%
%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_range_new.eps}
%		\caption{}
%		\label{fig:s_range}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_bearing_new.eps}
%		\caption{}
%		\label{fig:s_bearing}
%	\end{subfigure}\hfil 
%		\caption{Comparison of the calculated and simulated uncertainty values. (a) Simulated and calculated values for the range measurements. (b) Simulated and calculated values for the bearing measurements.}
%		\label{fig:aclos_mpc}
%\end{figure}
%Monte Carlo simulations were carried out with different initial configurations for the range and the bearing measurements using EKF for estimation. The state covariance matrix $ Q $ and the measurement noise covariance matrix $ \Gamma $ for the EKF were selected as
%\begin{equation}
%	Q=\begin{bmatrix}
%	0.01 & 0 & 0 & 0\\
%	0 & 0.01 & 0 & 0\\
%	0 & 0 & 0.01 & 0\\
%	0 & 0 & 0 & 0.01
%	\end{bmatrix},
%	\Gamma=\begin{bmatrix}
%	0.01 & 0 & 0\\
%	0 & 0.01& 0 \\
%	0 & 0 & 0.01
%	\end{bmatrix},
%\end{equation}   
%for the range measurements and
%\begin{equation}
%Q=\begin{bmatrix}
%0.01 & 0 & 0 & 0 & 0 & 0\\
%0 & 0.01 & 0 & 0 & 0 & 0\\
%0 & 0 & 0.0001 & 0 & 0 & 0\\
%0 & 0 & 0 & 0.01 & 0 & 0\\
%0 & 0 & 0 & 0 & 0.01 & 0\\
%0 & 0 & 0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\Gamma=\begin{bmatrix}
%0.0001 & 0 & 0 & 0\\
%0 & 0.0001& 0 & 0 \\
%0 & 0 & 0.0001 & 0\\
%0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\end{equation}
%for the bearing measurements. $\sigma_{p_1}$ values obtained from the estimator and calculated using the equations (\ref{eq:s_range}) and (\ref{eq:s_bearing}) are plotted in Fig.~\ref{fig:s_range} and Fig.~\ref{fig:s_bearing} for range and bearing measurements. It can be seen that the calculated uncertainty increases with increase in average distance, and this trend is also followed by the estimated value. The calculation gives us an upper bound for the covariance of the vehicles.

Next section presents the complete NMPC formulation combining the MHE scheme given in Sec.~\ref{sec:MHE} and the uncertainty results derived from analysis given in Sec.~\ref{sec:analysis}. 

==> Cooperative localization MPC/observability.tex <==
\section{Covariance calculation}\label{sec:analysis}
% We show in Theorem.~\ref{thm:covariance} that the covariance of the vehicle states $ p_{ij} $ is proportional to the sum of edges leading to the landmarks as $ p_{ij} = \sum \frac{1}{\epsilon_s} $. Since information matrices can be added together (see the proof for Corollaries \ref{cor:path} and \ref{cor:landmark}), it is possible to combine the split sections of the graph, and hence the analysis carried out for the individual sections can be generalized for the complete graph.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config2.eps}
		\caption{Example configuration of two vehicles and two landmarks.}
		\label{fig:config2}
	\end{figure}

Consider an example configuration of two vehicles (represented by $1$ and $2$) and two landmarks (represented by $a$ and $b$) as shown in Fig.~\ref{fig:config2}(i). For understanding how the paths/connections/measurements from a landmark to a vehicle influence the uncertainty of the vehicle states, we take each landmark separately and analyze one at a time. We start the analysis by considering the section $a-1-2$ of the graph, shown in Fig.~\ref{fig:config2}(ii). The observability matrix for the system can be written as
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 \\
o12 & -o12
\end{bmatrix},
\end{equation}
where $oa1,o12$, and $-o12$ are the derivatives of the measurements with respect to the vehicle states. For example, $oa1$ is the derivative of the measurement between the landmark $a$ and the vehicle-$1$ with respect to the vehicle-$1$. Since there is no measurement between the landmark $a$ and the vehicle-$2$, the corresponding entry is zero. Assuming the measurement covariance matrix $ \Gamma = I $, and zero-mean white Gaussian noise, the observability grammian is defined as $ O^TO $ and the covariance matrix $ P $ is written as %\cite{hinson2014observability,crassidis2004optimal}
\begin{eqnarray}
P &\leq& (O^T\Gamma^{-1}O)^{-1}, \\
&\leq& (O^TO)^{-1},\\
 &\leq& \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2} \\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \label{eq:p2a}
\end{bmatrix}.
\end{eqnarray}
The first element of the $P$ matrix correspond to the vehicle-$1$ connecting to the landmark $a$, hence $oa1$ (let us discard the square and fraction for easy understanding). The element $ \frac{1}{o12^2}+\frac{1}{oa1^2} $ of the $P$ matrix corresponds to the vehicle-$2$. Observing that it is connected to the landmark $a$ through vehicle-$1$, we can see both $oa1$ and $o12$. Next, we consider the section $1-2-b$ of the graph, as shown in Fig.~\ref{fig:config2}(iii). The observability and covariance matrices for the system are written as
\begin{equation}
O = \begin{bmatrix}
0 & ob2 \\
o12 & -o12 
\end{bmatrix},
\end{equation}
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} \\
\frac{1}{ob2^2} & \frac{1}{ob2^2}  \label{eq:p2b}
\end{bmatrix}.
\end{equation}
Vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$, which is clearly resembled in the first element of $P$. Vehicle-$2$ is directly connected to the landmark $b$. Hence, the last element of $P$ contains only $ob2$. 

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config3.eps}
		\caption{Example configuration of three vehicles and two landmarks.}
		\label{fig:config3}
	\end{figure}

Next, we take a configuration involving three vehicles as shown in Fig.~\ref{fig:config3}(i). Consider the section $3-a-1-2$ of the graph, shown in Fig.~\ref{fig:config3}(ii). The observability matrix for this configuration is given by
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 & 0 \\
o12 & -o12 & 0\\
0 & 0 & oa3
\end{bmatrix}.
\label{eq:ob_config3}
\end{equation} 
The covariance matrix $ P $ is given by
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2}  & 0\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & 0\\
0 & 0 & \frac{1}{oa3^2}  \label{eq:p3a}
\end{bmatrix}.
\end{equation}
The first element of the $P$ matrix contain only $oa1$ since the vehicle-$1$ is directly connected to the landmark $a$. The vehicle-$2$ is connected to the landmark $a$ through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. Since vehicle-$3$ is directly connected to the landmark, the last element of $P$ contains only $oa3$ as expected. Now, let us take the section $1-2-b-3$ of the graph, shown in Fig.~\ref{fig:config3}(iii). The observability and covariance matrices are given by
\begin{equation}
O = \begin{bmatrix}
0 & ob2 & 0 \\
o12 & -o12 & 0 \\
0 & 0 & ob3
\end{bmatrix},
\end{equation}
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0 \\
\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0\\
0 & 0 & \frac{1}{ob3^2}  \label{eq:p3b}
\end{bmatrix}.
\end{equation}
Vehicle-$2$ and vehicle-$3$ are directly connected to the landmark $b$. Therefore, the corresponding entries in the $P$ matrix contains only $ob2$ and $ob3$. The vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$ and this information is clearly reflected in the first entry of $P$.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config4.eps}
		\caption{Example configuration of four vehicles and two landmarks.}
		\label{fig:config4}
	\end{figure}

We conclude this analysis by taking a configuration with four vehicles and two landmarks as shown in Fig.~\ref{fig:config4}(i). The observability matrix for the sub-configuration with the landmark $a$ and the vehicles $1,2,3,4$, shown in Fig.~\ref{fig:config4}(ii) is given by
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 & 0 & 0 \\
o12 & -o12 & 0 & 0\\
0 & o23 & -o23 & 0\\
0 & o24 & 0 & -o24
\end{bmatrix}.
\end{equation}  
The covariance matrix $ P $ is given by
\begin{equation}
P \leq \begin{bmatrix*}[l]
\frac{1}{oa1^2} & \frac{1}{oa1^2}  &  \frac{1}{oa1^2} & \frac{1}{oa1^2}\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2}\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o23^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \\ 
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{oa1^2}  
\end{bmatrix*}. \label{eq:p4a}
\end{equation}
The vehicle-$1$ is directly connected to the landmark $a$, hence the first element of the $P$ matrix contain only $oa1$. The vehicle-$2$ is connected to the landmark through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $1$ and $2$, which is reflected in the $P$ matrix by the presence of $o12,o23$, and $oa1$. It is to be noted that the term $o24$ is absent as expected since the vehicle-$4$ is not involved in the path for vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$4$, since it is connected to the landmark through the vehicles $2$ and $1$. The entry contains $o12,o24$, and $oa1$ corresponding to the path $4-2-1-a$. Next, consider the sub-configuration with the landmark $b$, shown in Fig.~\ref{fig:config4}(iii). The observability and covariance matrices for this configuration are given by
\begin{eqnarray}
O &=& \begin{bmatrix}
0 & 0 & 0 & ob4 \\
o12 & -o12 & 0 & 0 \\
0 & o23 & -o23 & 0 \\
0 & o24 & 0 & -o24
\end{bmatrix},\\
P &\leq& \begin{bmatrix*}[l]
\frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2}\\
\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o23^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
\frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2}
\end{bmatrix*}.   \label{eq:p4b}
\end{eqnarray}
The vehicle-$4$ is directly connected to the landmark $b$, hence the fourth diagonal element of the $P$ matrix contain only $ob4$. The vehicle-$2$ is connected to the landmark through vehicle-$4$, hence both $o24$ and $ob4$ can be seen in the second diagonal element of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $2$ and $4$, which is reflected in the third diagonal element of the $P$ matrix by the presence of $o23,024$, and $ob4$. We can see that the term $o12$ is absent as expected since the vehicle-$1$ is not involved in the path for the vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$1$, since it is connected to the landmark through the vehicles $2$ and $4$. The entry contains $o12,o24$, and $ob4$ correspondingly.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config5.eps}
		\caption{Notations for a general multi-vehicle-landmark RPMG.}
		\label{fig:config5}
	\end{figure}

For stating the general result for any number of vehicles and landmarks, consider the notations given in Fig.~\ref{fig:config5}. The landmarks are represented using stars, and the vehicles are represented using triangles. All the vehicles are numbered $i,i+1,\ldots,n_v$, landmarks $j,j+1,\ldots,n_l$, edges $\epsilon_s,\epsilon_{s+1},\ldots,\epsilon_{n_e}$, where $i=j=s=1$. The observability vector associated with an edge/measurement is represented using $\epsilon$ with the edge number as subscript for simplicity. For example, the observability vector between landmark-$j$ and vehicle-$i$, $oji$ is represented by $\epsilon_s$. Now, the following theorem for a general RPMG can be stated. 

\begin{theorem}\label{thm:covariance}
The covariance associated with the vehicle-$i$, $i=1,\ldots,n_v$, due to the landmark-$j$, $j=1,\ldots,n_l$, is given by 
\begin{equation}
    p_{ij} = \sum_{s \in \mathcal{S}} \frac{1}{\epsilon_s},
\end{equation}
where $s=1,\ldots,n_e$, $\mathcal{S}$ is the set of edges that forms a path from vehicle-$i$ to the landmark-$j$, $n_v$ is the number of vehicles, $n_l$ is the number of landmarks, and $n_e$ is the number of edges in the RPMG.
\end{theorem}
\begin{proof}
The covariances associated with each vehicle for a two-vehicle-two-landmark configuration is given by equations \eqref{eq:p2a} and \eqref{eq:p2b}, followed by three vehicles in \eqref{eq:p3a} and \eqref{eq:p3b}, and four vehicles in \eqref{eq:p4a} and \eqref{eq:p4b}. The relation given in Theorem~\ref{thm:covariance} is clearly reflected in the elements of the corresponding covariance matrices. The generalization to $n_v$ vehicles and $n_l$ landmarks is straightforward.

The relation can be verified by using contradiction. Consider Fig.~\ref{fig:config3}(ii). Suppose the term/edge $\frac{1}{oa1^2}$ is not present in $p_{2a}$. Then the corresponding $O^TO$ matrix for the system will be
\begin{equation}
	O^TO = \begin{bmatrix}
		\frac{oa1^4}{-o12^2+oa1^2} & \frac{o12^2 oa1^2}{o12^2-oa1^2}  & 0\\
		\frac{o12^2 oa1^2}{o12^2-oa1^2} & \frac{o12^2 oa1^2}{-o12^2+oa1^2} & 0\\
		0 & 0 & \frac{1}{oa3^2}  \label{eq:proof1}
	\end{bmatrix},
\end{equation}
which contradicts with the $O^TO$ matrix derived from equation~ \eqref{eq:ob_config3}, which is 
\begin{equation}
 \begin{bmatrix}
		o12^2+oa1^2 & -o12^2  & 0\\
		-o12^2& o12^2 & 0\\
		0 & 0 & oa3^2  
	\end{bmatrix}.
\label{eq:oto_proof}
\end{equation}
Similarly, if an additional term $\frac{1}{oa3^2}$ is present in $p_{2a}$, the corresponding $O^TO$ matrix for the system will be
\begin{equation}
	O^TO = \begin{bmatrix}
		oa1^2+\frac{o12^2oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2}  & 0\\
		-\frac{o12^2 oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2} & 0\\
		0 & 0 & oa3^2  \label{eq:proof2}
	\end{bmatrix},
\end{equation}
which also contradicts with the $O^TO$ matrix given in~\eqref{eq:oto_proof}.
Hence, the relation given in Theorem~\ref{thm:covariance} is always true.
\end{proof}

The following corollaries can be written from Theorem~\ref{thm:covariance}.

\begin{corollary}\label{cor:path}
If there is more than one path from a landmark to a vehicle, and these paths are numbered from $1$ to $g_{ij}$, where $g_{ij}$ is the total number of paths from the landmark-$j$ to the vehicle-$i$, then the total covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert  p_{ij} \right\rVert  \leq \sum_{\kappa=1}^{g_{ij}} \left\lVert p_{ij}^{\kappa} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_{ij} = \sum_{\kappa=1}^{g_{ij}} p_{ij}^{\kappa},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $p_{ij}^{\kappa}$ is the covariance of the vehicle-$i$ due to the landmark-$j$ considering only the path-$\kappa$.
\end{corollary}

\begin{corollary}\label{cor:landmark}
If there is more than one landmark connected to a vehicle, then the covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert p_i \right\rVert  \leq \sum_{j \in \mathcal{J}} \left\lVert p_{ij} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_i  = \sum_{j \in \mathcal{J}} p_{ij},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $\mathcal{J}$ is the set of landmarks connected to the vehicle-$i$.
\end{corollary}

\begin{proof}
The method to calculate covariances for Corollary~\ref{cor:path} and \ref{cor:landmark} is given in Theorem~\ref{thm:covariance}. The summation is based on the properties of the information matrix given as follows~\cite{fisher,zegers2015fisher} 
% When information matrices are added, the resulting value will be greater than or equal to the sum of values of the individual matrices. That is, information is not lost through addition. 

If $X=(X_1,X_2,\ldots,X_n)$ and $X_1,X_2,\ldots,X_n$ are independent random variables, then $I_X(\alpha)=I_{X_1}(\alpha)+I_{X_2}(\alpha)+\ldots I_{X_n}(\alpha)$, where $I_x(\alpha)$ is the information matrix defined as 
\begin{equation*}
	I_x(\alpha) = E_{\alpha}\left[ \left( \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right) ^2\right] = \mathrm{Var}_{\alpha}\left(  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right).
\end{equation*}
Since \[f(x|\alpha) = \prod_{i=1}^{n}f_i(x_i|\alpha),\] where $f_i(\cdot|\alpha)$ is the pdf of $X_i$,
\begin{eqnarray}
\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right] &=& \sum_{i=1}^{n}\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f_i(X_i|\alpha)\right], \nonumber \\
I_X(\alpha) &=& \sum_{i=1}^{n}I_{X_i}(\alpha). \nonumber 
\end{eqnarray} 

 Since covariance is the inverse of information, it is possible to find the total covariance associated with each vehicle by adding the components from all the paths and landmarks.
\end{proof}

In the next sub-sections, we show how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements. 
% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config1.eps}
% 		\caption{Example configuration }
% 		\label{fig:config1}
% 	\end{figure}
% Consider an example configuration given in Fig.~\ref{fig:config1}. The vehicles $ 1 $ and $ 2 $ are connected to landmarks $a$ and $b$. The observability matrix for the system can be written as
% \begin{equation}
% O = \begin{bmatrix}
% O1a \\
% O2b \\
% O12
% \end{bmatrix},
% \end{equation}
% where 
% \begin{eqnarray}
% O1a &=& \begin{bmatrix}
% o1a & 0
% \end{bmatrix}, \\
% O2b &=& \begin{bmatrix}
% 0 & o2b
% \end{bmatrix}, \\
% O12 &=& \begin{bmatrix}
% o12 & -o12
% \end{bmatrix}.
% \end{eqnarray}  
% Assuming the measurement covariance matrix $ \Gamma = I $, the observability grammian can be defined as $ O^TO $ and the covariance matrix $ P $ can be found as \cite{hinson2014observability}
% \begin{equation}
% P = (O^TO)^{-1},
% \end{equation}
% which can be written as
% \begin{equation}
% P = \begin{bmatrix}
% P(1,1) & P(1,2) \\
% P(2,1) & P(2,2)
% \end{bmatrix},
% \end{equation}
% where
% %{\tiny
% \begin{eqnarray}
% P(1,1) &=& (o12^2 + o2b^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(1,2) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,1) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,2) &=& (o12^2 + o1a^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2).
% \end{eqnarray}
% %}%
% Looking at the elements of $P$, we can clearly see that the covariance is related to the connection/path. In the next sections, we try to find out how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements.   

\subsection{Range measurements}
%	\begin{figure}
%		\centering
%		\includegraphics[width=8cm]{figs/config1.eps}
%		\caption{Example configuration }
%		\label{fig:config1}
%	\end{figure}
Consider the configuration given in Fig.~\ref{fig:config2}(i). The vehicle dynamics are defined as
\begin{eqnarray}
\dot{x}_1 &=& v \cos{\psi_1}, \\
\dot{y}_1 &=& v \sin{\psi_1}, \\
\dot{x}_2 &=& v \cos{\psi_2}, \\
\dot{y}_2 &=& v \sin{\psi_2}, 
\end{eqnarray} 
with range measurements
\begin{eqnarray}
h_{1a} &=& \sqrt{(x_1 - x_a)^2 + (y_1 - y_a)^2}, \\
h_{12} &=& \sqrt{(x_1 - x_2)^2 + (y_1 - y_2)^2}, \\
h_{2b} &=& \sqrt{(x_2 - x_b)^2 + (y_2 - y_b)^2},
\end{eqnarray}
and we derive the observability matrix using the Lie derivatives~ \cite{sharma2011graph}. 

Define 
\begin{equation}
f_L = \begin{bmatrix}
\cos{\psi_1} \\
\sin{\psi_1} \\
\cos{\psi_2} \\
\sin{\psi_2} 
\end{bmatrix},
\end{equation}
and the vehicle dynamics can be represented as
\begin{equation}
\dot{X} = vf_L.
\end{equation}
The gradient of zero\textsuperscript{th} order Lie derivatives are given as
\begin{eqnarray}
H_{1a} &=& \begin{bmatrix}
\frac{x_1 - x_a}{R_{1a}} & \frac{y_1 - y_a}{R_{1a}} & 0 & 0 
\end{bmatrix}, \\
H_{2b} &=& \begin{bmatrix}
& 0 & 0 & \frac{x_2 - x_b}{R_{2b}} & \frac{y_2 - y_b}{R_{2b}}  
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{x_1 - x_2}{R_{12}} & \frac{y_1 - y_2}{R_{12}} & \frac{-(x_1 - x_2)}{R_{12}} & \frac{-(y_1 - y_2)}{R_{12}} 
\end{bmatrix}, \\
\end{eqnarray}
where $R_{(\cdot)} $ is the distance between nodes.
The gradient of first order Lie derivatives are given as
\begin{eqnarray}
\frac{\partial }{\partial X}\left( \frac{\partial h_{1a}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
\frac{(y_1-y_a)^2 C\psi_1 -(x_1-x_a)(y_1-y_a) S\psi_1}{R_{1a}^3} &
 \frac{(x_1-x_a)^2 S\psi_1-(x_1-x_a)(y_1-y_a) C\psi_1}{R_{1a}^3}& 0 & 0 
\end{bmatrix},\nonumber\\
\frac{\partial }{\partial X}\left( \frac{\partial h_{2b}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
0 & 0 & \frac{(y_2-y_b)^2 C\psi_2 + (-x_2+x_b)(y_2-y_b) S\psi_2}{R_{2b}^3} &
\frac{(x_2-x_b)^2 S\psi_2 + (-y_2+y_b)(x_2-x_b) C\psi_2}{R_{2b}^3} 
\end{bmatrix},\\
\frac{\partial }{\partial X}\left( \frac{\partial h_{12}}{\partial X}  \cdot f \right) &=& 
[\begin{matrix}
\frac{-2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix} 
\frac{2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix}
\frac{2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix}
\frac{-2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}],
\end{eqnarray}
where $ \sin $ and $ \cos $ are abbreviated as $S$ and $C$, $ \Delta\psi^- = \psi_1-\psi_2 $, and $ \Delta\psi^+ = \psi_1+\psi_2 $.

Observability matrix is formed by using Lie derivatives up to first order as
\begin{equation}
O = \begin{bmatrix}
\nabla L^0 \\
\nabla L^1
\end{bmatrix},
\end{equation} 
where $L^0$ and $L^1$ are the zero\textsuperscript{th} and first order Lie derivatives respectively. The covariance matrix $P$ is found by inverting $ O^TO $ with the assumption of $\Gamma=I$.

The standard deviation in $x$ direction for the first vehicle can be found by taking the square root of the first element of the $P$ matrix,
\begin{equation}
\sigma_{x_1} = \sqrt{P(1,1)}.
\end{equation} 
Similarly, the standard deviation in the $y$ direction and the combined position uncertainty can be found as
\begin{eqnarray}
\sigma_{y_1} &=& \sqrt{P(2,2)},\\
\sigma_{p_1} &=& \sqrt{\sigma_{x_1}^2 + \sigma_{y_1}^2}.
\end{eqnarray}

Since the derived $P$ matrix is very large with several terms, we consider some simplifying assumptions to formulate an approximate relation. All the distance terms were substituted with a single average value. The resulting relation is given as
\begin{equation}
\sigma_{p_1} = \sqrt{\frac{2}{3}+R_g^2 \csc^2{(\psi_1-\theta_g)}},
\label{eq:s_range}
\end{equation}
where $R_g,\theta_g$ are the average value of distance and LOS angle. It is evident from the relation that the covariance of vehicle depends on the distances from the landmarks and the LOS angles to them. As the distance increases, the covariance also increases. Similarly, $ \sigma_p $ of other vehicles can also be found. 
\subsection{Bearing measurements}\label{sec:b_measurement}
Let's extend the vehicle model to contain three states. The new model is given as
\begin{eqnarray}
\dot{x}_1 &=& v \cos{\psi_1}, \\
\dot{y}_1 &=& v \sin{\psi_1}, \\
\dot{\psi}_1 &=& \omega_1, \\ 
\dot{x}_2 &=& v \cos{\psi_2}, \\
\dot{y}_2 &=& v \sin{\psi_2}, \\
\dot{\psi}_2 &=& \omega_2, 
\end{eqnarray} 
With the same configuration as in Fig.~\ref{fig:config2}(i), define bearing measurement equations as
\begin{eqnarray}
h_{a1} &=& \arctan\left( \frac{y_a-y_1}{x_a-x_1}\right) - \psi_1, \\
h_{b2} &=& \arctan\left( \frac{y_b-y_2}{x_b-x_2}\right) - \psi_2, \\
h_{12} &=& \arctan\left( \frac{y_1-y_2}{x_1-x_2}\right) - \psi_2, \\
h_{21} &=& \arctan\left( \frac{y_2-y_1}{x_2-x_1}\right) - \psi_1, 
\end{eqnarray}
the gradient of zeroth order Lie derivatives are given as
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{-(y_1 - y_a)}{R_{a1}^2} & \frac{x_1 - x_a}{R_{a1}^2} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{-(y_2 - y_b)}{R_{b2}^2} & \frac{x_2 - x_b}{R_{b2}^2} & -1  
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{12}^2} & \frac{x_1 - x_2}{R_{12}^2} & 0 & \frac{y_1 - y_2}{R_{12}^2} & \frac{x_2 - x_1}{R_{12}^2} & -1 
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{21}^2} & \frac{x_1 - x_2}{R_{21}^2} & -1 & \frac{y_1 - y_2}{R_{21}^2} & \frac{x_2 - x_1}{R_{21}^2} & 0 
\end{bmatrix}, \hspace{6mm}
\end{eqnarray} 
using the geometry, the equations are changed to make it in terms of LOS angles as follows
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{\sin\theta_{a1}}{R_{a1}} & \frac{-\cos\theta_{a1}}{R_{a1}} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{\sin\theta_{b2}}{R_{b2}} & \frac{-\cos\theta_{b2}}{R_{b2}} & -1 
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{-\sin\theta_{12}}{R_{12}} & \frac{\cos\theta_{12}}{R_{12}} & 0 & \frac{\sin\theta_{12}}{R_{12}} & \frac{-\cos\theta_{12}}{R_{12}} & -1  
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{\sin\theta_{21}}{R_{21}} & \frac{-\cos\theta_{21}}{R_{21}} & -1 & \frac{-\sin\theta_{21}}{R_{21}} & \frac{\cos\theta_{21}}{R_{21}} & 0  
\end{bmatrix}. \hspace{6mm}
\end{eqnarray} 
Define 
\begin{equation}
f_v = \begin{bmatrix}
\cos{\psi_1} \\
\sin{\psi_1} \\
0\\
\cos{\psi_2} \\
\sin{\psi_2}\\
0 
\end{bmatrix},
f_{\omega_1} = \begin{bmatrix}
0 \\
0 \\
1\\
0 \\
0\\
0 
\end{bmatrix},
f_{\omega_2} = \begin{bmatrix}
0 \\
0 \\
0\\
0 \\
0\\
1 
\end{bmatrix},
\end{equation}
and the dynamics can be represented as
\begin{equation}
\dot{X} = \begin{bmatrix}
\dot{X}_1 \\
\dot{X}_2
\end{bmatrix}
= f_vv+f_{\omega_1}\omega_1 + f_{\omega_2}\omega_2,
\end{equation}
and a similar procedure to the range measurement case is followed to find the first order Lie derivatives, observability grammian and covariance matrix $P$. The covariance in position of the first vehicle is given by
\begin{equation}
\sigma_{p_1}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_1-\theta_g))} \right)+(R_g^2+R_g^4)\csc^2(\psi_1-\theta_g). 
\label{eq:s_bearing}
\end{equation} 
Similarly, $ \sigma_p $ of other vehicles can also be found.

%\subsection{Results}
%
%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_range_new.eps}
%		\caption{}
%		\label{fig:s_range}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_bearing_new.eps}
%		\caption{}
%		\label{fig:s_bearing}
%	\end{subfigure}\hfil 
%		\caption{Comparison of the calculated and simulated uncertainty values. (a) Simulated and calculated values for the range measurements. (b) Simulated and calculated values for the bearing measurements.}
%		\label{fig:aclos_mpc}
%\end{figure}
%Monte Carlo simulations were carried out with different initial configurations for the range and the bearing measurements using EKF for estimation. The state covariance matrix $ Q $ and the measurement noise covariance matrix $ \Gamma $ for the EKF were selected as
%\begin{equation}
%	Q=\begin{bmatrix}
%	0.01 & 0 & 0 & 0\\
%	0 & 0.01 & 0 & 0\\
%	0 & 0 & 0.01 & 0\\
%	0 & 0 & 0 & 0.01
%	\end{bmatrix},
%	\Gamma=\begin{bmatrix}
%	0.01 & 0 & 0\\
%	0 & 0.01& 0 \\
%	0 & 0 & 0.01
%	\end{bmatrix},
%\end{equation}   
%for the range measurements and
%\begin{equation}
%Q=\begin{bmatrix}
%0.01 & 0 & 0 & 0 & 0 & 0\\
%0 & 0.01 & 0 & 0 & 0 & 0\\
%0 & 0 & 0.0001 & 0 & 0 & 0\\
%0 & 0 & 0 & 0.01 & 0 & 0\\
%0 & 0 & 0 & 0 & 0.01 & 0\\
%0 & 0 & 0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\Gamma=\begin{bmatrix}
%0.0001 & 0 & 0 & 0\\
%0 & 0.0001& 0 & 0 \\
%0 & 0 & 0.0001 & 0\\
%0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\end{equation}
%for the bearing measurements. $\sigma_{p_1}$ values obtained from the estimator and calculated using the equations (\ref{eq:s_range}) and (\ref{eq:s_bearing}) are plotted in Fig.~\ref{fig:s_range} and Fig.~\ref{fig:s_bearing} for range and bearing measurements. It can be seen that the calculated uncertainty increases with increase in average distance, and this trend is also followed by the estimated value. The calculation gives us an upper bound for the covariance of the vehicles.

Next section presents the complete NMPC formulation combining the MHE scheme given in Sec.~\ref{sec:MHE} and the uncertainty results derived from analysis given in Sec.~\ref{sec:analysis}. 

==> Cooperative localization MPC/results.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
		\caption{$\tau_h=20$\,s}
		\label{fig:h200}
	\end{subfigure}
	
%	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
		\caption{$\tau_h=35$\,s}
		\label{fig:h350}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure}
\subsection{EKF vs calculated sigma values}
A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf150.eps}
		\caption{EKF trajectory.}
		\label{fig:ekf_traj}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/calc150.eps}
		\caption{Calculated trajectory.}
		\label{fig:calc_traj}
	\end{subfigure}\hfil 
	
	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
		\caption{vehicle 1}
		\label{fig:ekf_calc_sigmap1}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
		\caption{vehicle 2}
		\label{fig:ekf_calc_sigmap2}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
		\caption{vehicle 3}
		\label{fig:ekf_calc_sigmap3}
	\end{subfigure}
	\caption{EKF vs calculated sigma values.}
	\label{fig:EKF_calc}
\end{figure} 

\subsection{MHE vs EKF}
The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/EKF_pc.eps}
		\caption{EKF trajectory.}
		\label{fig:ekf_pc}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/MHE_pc.eps}
		\caption{MHE trajectory.}
		\label{fig:mhe_pc}
	\end{subfigure}\hfil 
	
	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp1.eps}
		\caption{Error in position of vehicle 1}
		\label{fig:ekfp1}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp2.eps}
		\caption{Error in position of vehicle 2}
		\label{fig:ekfp2}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp3.eps}
		\caption{Error in position of vehicle 3}
		\label{fig:ekfp3}
	\end{subfigure}
	\caption{EKF vs MHE.}
	\label{fig:EKF_MHE}
\end{figure}      

\begin{table}
	\centering
	\begin{tabular}{ |c|c|c| } 
		\hline
		& MHE & EKF \\
		\hline
		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
		Time required per iteration (s)  &  1.388   &  1.144   \\
		\hline
	\end{tabular}
	\caption{EKF vs MHE.}
	\label{table:ekf_mhe}
\end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_coop.eps}
		\caption{Trajectory of vehicles with cooperation.}
		\label{fig:multi_c}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_nc1.eps}
		\caption{Trajectory of vehicles without cooperation.}
		\label{fig:multi_nc}
	\end{subfigure}\hfil 
	\caption{Effect of cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
		\caption{Example 1.}
		\label{fig:multi10j}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
		\caption{Example 2.}
		\label{fig:multi10j1}
	\end{subfigure}\hfil 
		\caption{Trajectories of 10 vehicles with NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> Cooperative localization MPC/results_2c.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. We use the total path length  and average estimation error as metric for analyzing the performance of the proposed approach. We perform the following analysis (i) effect of horizon length in the NMPC on the path length and estimation error (ii) effect of cooperation  (iii) comparison with the approach proposed in \cite{manoharan2019nonlinear} and (iv) effect of increasing the number of vehicles in the region to 10. Before presenting the analysis, we will describe the simulation setting.

\subsection{Simulation setup}
We consider an environment of 200m $\times$ 200m, where 20 landmarks are randomly placed. Each vehicle starts at a given location and has a desired goal location. The vehicles have a constant velocity of 5\,m/s.
% Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. 
The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ is selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m.  The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. Each time step is $0.1$s for all the simulations. The simulations were carried out on a Ubuntu 18.04, Intel i9 workstation with 64GB RAM. 
\subsection{Effect of NMPC horizon length}
In NMPC, the horizon length plays a key role between path optimality and computational time. The larger the horizon, better the path obtained at the cost of increased computational time. This effect can be seen in Fig. \ref{fig:h10}, where the computation time for prediction horizon of $\tau_h=1$\,s is 0.056\,s, however, the paths are not optimal. With increase in $\tau_h$ to 15s, there is significant improvement in the path of vehicle 1 at increased computational time of 0.42s per iteration. With further increase in horizon length to $\tau_h=40$\,s, the average time to compute an iteration is 3.43\,s, but the obtained path length for the vehicles  is near-optimal. The path length for $\tau_h=25s$ is close to that obtained with $\tau_h=40$ but takes only 1.2s.

Further, we conducted Monte-Carlo simulation to see the effect of placement of landmarks on the vehicle paths. Figure \ref{fig:monte} shows the effect of change in landmark placement for different $\tau_h$. From the Fig.\ref{fig:monte}(a), we can see that the computation time for $\tau_h=1$s is very less but the vehicle which reaches the destination at the last on average is also high as shown in \ref{fig:monte}(b). Note that, on average, the times taken by the last agent reaching its goal for $\tau_h=$25s and $\tau_h=$40s are almost similar, however, $\tau_25$ takes far less time. 
Hence we consider $\tau_h=25$s for the  rest of the simulations
%Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure*}
	\centering 
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.25cm]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.5cm]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}\hspace{2mm}
	%	\begin{subfigure}{0.3\textwidth}
	%		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
	%		\caption{$\tau_h=20$\,s}
	%		\label{fig:h200}
	%	\end{subfigure}\\
	%	\medskip
	\begin{subfigure}{4.25cm}
		\includegraphics[ width=4.25cm]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}
	%	\begin{subfigure}{0.3\textwidth}
	%		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
	%		\caption{$\tau_h=35$\,s}
	%		\label{fig:h350}
	%	\end{subfigure}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.25cm]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
%	\begin{subfigure}{5cm}
%	\includegraphics[clip,trim=10mm 0 0 0 0, width=6cm]{figs/monte.eps}
%	\caption{Monte-Carlo simulation}
%	\label{fig:h150}
%\end{subfigure}\hspace{2mm}

	\caption{The average computational time taken per iteration for different $\tau_h$. (a) 0.05\,s (b) 0.42\,s (c) 1.21\,s (d) 3.43\,s.}
	\label{fig:sim_horizon}
\end{figure*}


\begin{figure}
	\centering
	\begin{subfigure}{4.25cm}
	\includegraphics[width=4.4cm,height=2cm]{figs/time_per_iter.png}
	\caption{}	
	\end{subfigure}\hspace{2mm}
	\begin{subfigure}{4.25cm}
	\includegraphics[width=4.4cm,height=2cm]{figs/mc_time}
	\caption{}	
	\end{subfigure}
	\caption{Monte-Carlo simulation for prediction horizon $\tau_h=1,25,40$. (a) Average computational time per iteration (b) Average time taken by all the agents to reach their destinations.} \label{fig:monte}
\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[clip, trim=10mm 5mm 13mm 8mm, width=5cm]{figs/monte.eps}
%	\label{fig:monte}
%	\caption{Monte-Carlo simulation}
%\end{figure}


% \subsection{EKF vs calculated sigma values}
% A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

% \begin{figure*}
% 	\centering 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf150.eps}
% 		\caption{EKF trajectory.}
% 		\label{fig:ekf_traj}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/calc150.eps}
% 		\caption{Calculated trajectory.}
% 		\label{fig:calc_traj}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
% 		\caption{vehicle 1}
% 		\label{fig:ekf_calc_sigmap1}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
% 		\caption{vehicle 2}
% 		\label{fig:ekf_calc_sigmap2}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
% 		\caption{vehicle 3}
% 		\label{fig:ekf_calc_sigmap3}
% 	\end{subfigure}
% 	\caption{EKF vs calculated sigma values.}
% 	\label{fig:EKF_calc}
% \end{figure*} 

\subsection{Effect of cooperation}
One of the main contributions of this paper is to show that with cooperation, the vehicles can jointly determine minimal distance paths to their goal locations while meeting localization accuracy. To show the effect of cooperation, we consider a specific scenario as shown in Fig.~\ref{fig:multi_coop}, where the landmarks are located at the top of the scenario. 
%A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. 
Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. We consider  $\tau_h$ = 25\,s, and $R_s=$ 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_coop}(a) that the vehicles with cooperation determined a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_coop}(b). The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}
	\centering 
	\includegraphics[width=4.3cm]{figs/multi10_coop.eps}
	\includegraphics[width=4.3cm]{figs/multi10_nc1.eps}
	%	\begin{subfigure}{0.25\textwidth}
	%		\includegraphics[width=3cm]{figs/multi10_coop.eps}
	%		\caption{Trajectory of vehicles with cooperation.}
	%		\label{fig:multi_c}
	%	\end{subfigure}\hfil 
	%	\begin{subfigure}{0.25\textwidth}
	%		\includegraphics[width=3cm]{figs/multi10_nc1.eps}
	%		\caption{Trajectory of vehicles without cooperation.}
	%		\label{fig:multi_nc}
	%	\end{subfigure}\hfil 
	\caption{Effect of cooperation. (a) Trajectory of vehicles with cooperation. (b) Trajectory of vehicles without cooperation.}
	\label{fig:multi_coop}
\end{figure} 


 \subsection{MHE vs EKF}
 The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. In Fig. \ref{fig:block}, the step 1 sub-block of the MHE is replaced by the EKF. The horizon length for the MHE is selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The vehicles' mean square error (MSE) for the MHE is 0.46\,m and that with the EKF is 0.79\,m. The computation time requirement for the MHE is 1.21\,s, while the EKF takes 1.10\,s. Although the MHE takes 9\% more computational time than the EKF, its accuracy is 72\% better than the EKF. 

\begin{figure*}
	\centering 
	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.5cm]{figs/EKF_pc6.eps}
		\caption{}
		\label{fig:ekf_pc}
	\end{subfigure}
	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.5cm]{figs/MHE_pc5.eps}
		\caption{}
		\label{fig:mhe_pc}
	\end{subfigure}
	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.5cm]{figs/ekf_mhe_p1.eps}
		\caption{}
		\label{fig:ekfp1}
	\end{subfigure}
	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.5cm]{figs/ekf_mhe_p2.eps}
		\caption{}
		\label{fig:ekfp2}
	\end{subfigure}
	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.5cm]{figs/ekf_mhe_p3.eps}
		\caption{}
		\label{fig:ekfp3}
	\end{subfigure}
	\caption{(a) NMPC solution with EKF based estimation (b) NMPC solution with MHE (c) Error in position of vehicle 1 (d) Error in position of vehicle 2  (e)  Error in position of vehicle 3}
	\label{fig:EKF_MHE}
\end{figure*}      
     

% \begin{table}
% 	\centering
% 	\begin{tabular}{ |c|c|c| } 
% 		\hline
% 		& MHE & EKF \\
% 		\hline
% 		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
% 		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
% 		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
% 		Time required per iteration (s)  &  1.388   &  1.144   \\
% 		\hline
% 	\end{tabular}
% 	\caption{EKF vs MHE.}
% 	\label{table:ekf_mhe}
% \end{table}



\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles in a 500m $\times$ 500m plane with all the vehicles moving at a velocity of 10\,m/s was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all the ten vehicles. The average computation time per iteration was 7.25\,s due to the increase in the size of state matrix for 10 vehicles.

\begin{figure}
	\centering 
			\includegraphics[width=4.3cm]{figs/multi10_j.eps}
					\includegraphics[width=4.3cm]{figs/multi10_j1.eps}
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
%		\caption{Example 1.}
%		\label{fig:multi10j}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
%		\caption{Example 2.}
%		\label{fig:multi10j1}
%	\end{subfigure}\hfil 
		\caption{Trajectories of 10 vehicles using NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> Cooperative localization MPC/results_2c1.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. We use the total path length  and average estimation error as metric for analyzing the performance of the proposed approach. We perform the following analysis (i) effect of horizon length in the NMPC on the path length and estimation error (ii) effect of cooperation  (iii) Comparison with the approach proposed in \cite{manoharan2019nonlinear} and (iv) effect of increasing the number of vehicles in the region 10. Before presenting the analysis, we will describe the simulation setting.

\subsection{Simulation setup}
%Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. 
The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure*}
	\centering 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
		\caption{$\tau_h=20$\,s}
		\label{fig:h200}
	\end{subfigure}\\
	
%	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
		\caption{$\tau_h=35$\,s}
		\label{fig:h350}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure*}
% \subsection{EKF vs calculated sigma values}
% A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

% \begin{figure*}
% 	\centering 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf150.eps}
% 		\caption{EKF trajectory.}
% 		\label{fig:ekf_traj}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/calc150.eps}
% 		\caption{Calculated trajectory.}
% 		\label{fig:calc_traj}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
% 		\caption{vehicle 1}
% 		\label{fig:ekf_calc_sigmap1}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
% 		\caption{vehicle 2}
% 		\label{fig:ekf_calc_sigmap2}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
% 		\caption{vehicle 3}
% 		\label{fig:ekf_calc_sigmap3}
% 	\end{subfigure}
% 	\caption{EKF vs calculated sigma values.}
% 	\label{fig:EKF_calc}
% \end{figure*} 

 \subsection{MHE vs EKF}
 The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

 \begin{figure*}[h]
 	\centering 
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKF_pc.eps}
 		\caption{}
 		\label{fig:ekf_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/MHE_pc.eps}
 		\caption{}
 		\label{fig:mhe_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp1.eps}
 		\caption{}
 		\label{fig:ekfp1}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.75cm]{figs/EKFp2.eps}
 		\caption{}
 		\label{fig:ekfp2}
 	\end{subfigure}\hspace{0.2cm}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp3.eps}
 		\caption{}
 		\label{fig:ekfp3}
 	\end{subfigure}
 	\caption{(a) NMPC solution with EKF based estimation (b) NMPC solution with MHE (c) Error in position of vehicle 1 (d) Error in position of vehicle 2  (e)  Error in position of vehicle 3}
 	\label{fig:EKF_MHE}
 \end{figure*}      

% \begin{table}
% 	\centering
% 	\begin{tabular}{ |c|c|c| } 
% 		\hline
% 		& MHE & EKF \\
% 		\hline
% 		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
% 		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
% 		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
% 		Time required per iteration (s)  &  1.388   &  1.144   \\
% 		\hline
% 	\end{tabular}
% 	\caption{EKF vs MHE.}
% 	\label{table:ekf_mhe}
% \end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}
	\centering 
	\includegraphics[width=4.5cm]{figs/multi10_coop.eps}\hspace{-5mm}
	\includegraphics[width=4.5cm]{figs/multi10_nc1.eps}
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_coop.eps}
%		\caption{Trajectory of vehicles with cooperation.}
%		\label{fig:multi_c}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_nc1.eps}
%		\caption{Trajectory of vehicles without cooperation.}
%		\label{fig:multi_nc}
%	\end{subfigure}\hfil 
	\caption{Effect of cooperation. (a) Trajectory of vehicles with cooperation.(b) Trajectory of vehicles without cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}
	\centering 
			\includegraphics[width=4.5cm]{figs/multi10_j.eps}\hspace{-5mm}
					\includegraphics[width=4.5cm]{figs/multi10_j1.eps}
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
%		\caption{Example 1.}
%		\label{fig:multi10j}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
%		\caption{Example 2.}
%		\label{fig:multi10j1}
%	\end{subfigure}\hfil 
		\caption{Examples for 10 vehicles path computed using NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> Cooperative localization MPC/results_2c2.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure*}
	\centering 
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.25cm]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}\hspace{2mm}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.5cm]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}\hspace{2mm}
%	\begin{subfigure}{0.3\textwidth}
%		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
%		\caption{$\tau_h=20$\,s}
%		\label{fig:h200}
%	\end{subfigure}\\
%	\medskip
	\begin{subfigure}{4.25cm}
		\includegraphics[ width=4.5cm]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}\hspace{2mm}
%	\begin{subfigure}{0.3\textwidth}
%		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
%		\caption{$\tau_h=35$\,s}
%		\label{fig:h350}
%	\end{subfigure}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.5cm]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure*}
% \subsection{EKF vs calculated sigma values}
% A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

% \begin{figure*}
% 	\centering 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf150.eps}
% 		\caption{EKF trajectory.}
% 		\label{fig:ekf_traj}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/calc150.eps}
% 		\caption{Calculated trajectory.}
% 		\label{fig:calc_traj}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
% 		\caption{vehicle 1}
% 		\label{fig:ekf_calc_sigmap1}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
% 		\caption{vehicle 2}
% 		\label{fig:ekf_calc_sigmap2}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
% 		\caption{vehicle 3}
% 		\label{fig:ekf_calc_sigmap3}
% 	\end{subfigure}
% 	\caption{EKF vs calculated sigma values.}
% 	\label{fig:EKF_calc}
% \end{figure*} 

 \subsection{MHE vs EKF}
 The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

 \begin{figure*}
 	\centering 
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKF_pc.eps}
 		\caption{}
 		\label{fig:ekf_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/MHE_pc.eps}
 		\caption{}
 		\label{fig:mhe_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp1.eps}
 		\caption{}
 		\label{fig:ekfp1}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.75cm]{figs/EKFp2.eps}
 		\caption{}
 		\label{fig:ekfp2}
 	\end{subfigure}\hspace{0.2cm}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp3.eps}
 		\caption{}
 		\label{fig:ekfp3}
 	\end{subfigure}
 	\caption{(a) NMPC solution with EKF based estimation (b) NMPC solution with MHE (c) Error in position of vehicle 1 (d) Error in position of vehicle 2  (e)  Error in position of vehicle 3}
 	\label{fig:EKF_MHE}
 \end{figure*}      

% \begin{table}
% 	\centering
% 	\begin{tabular}{ |c|c|c| } 
% 		\hline
% 		& MHE & EKF \\
% 		\hline
% 		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
% 		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
% 		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
% 		Time required per iteration (s)  &  1.388   &  1.144   \\
% 		\hline
% 	\end{tabular}
% 	\caption{EKF vs MHE.}
% 	\label{table:ekf_mhe}
% \end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}
	\centering 
	\includegraphics[width=4.3cm]{figs/multi10_coop.eps}
	\includegraphics[width=4.3cm]{figs/multi10_nc1.eps}
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_coop.eps}
%		\caption{Trajectory of vehicles with cooperation.}
%		\label{fig:multi_c}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_nc1.eps}
%		\caption{Trajectory of vehicles without cooperation.}
%		\label{fig:multi_nc}
%	\end{subfigure}\hfil 
	\caption{Effect of cooperation. (a) Trajectory of vehicles with cooperation.(b) Trajectory of vehicles without cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}
	\centering 
			\includegraphics[width=4.3cm]{figs/multi10_j.eps}
					\includegraphics[width=4.3cm]{figs/multi10_j1.eps}
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
%		\caption{Example 1.}
%		\label{fig:multi10j}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
%		\caption{Example 2.}
%		\label{fig:multi10j1}
%	\end{subfigure}\hfil 
		\caption{Examples for 10 vehicles path computed using NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> Introduction.tex <==
\section{Introduction}\label{sec:intro}
Urban air mobility (UAM) is expected to have highly automated, cooperative, passenger, and cargo-carrying aerial vehicles in urban areas \cite{faa}, and the use of autonomous aerial vehicles (AAVs) for various activities are expected to rise substantially in the near future \cite{sesar}. Cargo delivery drones operate in urban canyons with high-rise buildings and other obstructions, which calls for significant localization accuracy. However, operating in such environments pose an additional challenge in localization since Global navigation satellite systems (GNSS) are unreliable in such scenarios. A solution to this problem is to use alternate localization schemes such as relative localization \cite{betke1997mobile,thrun1998finding}, vision-based methods \cite{lategahn2014vision,kim2005vision}, and ultra-wide-band (UWB) localization schemes \cite{krishnan2007uwb,zhang2018linear}. As the urban airspace is expected to contain a large number of AAVs, relative localization between vehicles can also be used in addition to localization with respect to known landmarks. 

Cooperative path planning with localization constraints involves the following components: (i) localization -- vehicles estimate their position by using relative measurements obtained with respect to other vehicles or landmarks, and (ii) cooperative path planning -- localization constraints have to be considered while planning the optimal path from source to destination, and hence the agents must cooperate with each other to  generate motion commands that  improve the localization accuracy of the entire group while reducing the path length to reach their destination. Several works have studied the problem separately. For instance, \cite{Kurazume1998,Roumeliotis2000,Spletzer2001,Mourikis2006,Nerurkar2009,wan2014cooperative,minaeian2016vision,frohle2018cooperative,pierre2018range,liu2018multi,guo2019ultra,zhu2019cooperative} on cooperative localization and \cite{zheng2005evolutionary,Agha-Mohammadi2014,Mathew2015,mac2016heuristic} on path planning. However, the collection of works on cooperative path planning with the localization constraints is limited, which we will review below.

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
		\caption{}
		\label{fig:scenario}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
		\caption{}
		\label{fig:rpmg}
	\end{subfigure}\hfil 
	\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
	\label{fig:path_graph}
\end{figure}  

Bopardikar et al.~\cite{bopardikar2015multiobjective} presented a graph-based probabilistic roadmap approach to tackle the path planning problem subject to localization constraints. A time-optimal path planner satisfying the covariance bounds was given in \cite{singh2016landmarks} using a swarm optimization technique coupled with a rabbit-carrot based path follower. An approach to optimally place landmarks to satisfy localization constraints was proposed in \cite{sundar2019path}. The algorithm computes an optimal path for the vehicle and the locations where the landmarks should be placed. A localizability constrained path planning method for autonomous vehicles which takes into account the laser range finder (LRF) sensor model of the vehicle is proposed in \cite{irani2018localizability} to maintain a satisfactory level of localizability throughout the path. Kassas et al. \cite{kassas2021uav} present a multi-objective motion planning algorithm in which the vehicle tries to balance the objectives of navigating to the waypoint and reducing its position estimate uncertainty. In \cite{manoharan2019nonlinear}, a nonlinear model predictive control scheme was used to find optimal paths that ensured the required localization accuracy for a group of cooperative UAVs without analysis.

Urban air mobility calls for improved localization accuracy due to its innate nature involving close structures, narrow pathways, and a large number of vehicles. Moving horizon estimation (MHE) has been suggested as an alternate to EKF for increasing the accuracy of nonlinear estimation problems by \cite{rawlings2006particle,wang2014optimization,mehrez2017optimization}. Erunsal et al. \cite{erunsal2019decentralized} proposed an approach combining NMPC and pose-graph-MHE for 3D formation control of micro aerial vehicles with relative sensing capability. In \cite{liu2020decentralized}, a decentralized MHE technique is proposed for networked navigation with packet dropouts.    

In this paper, we extend the  work in ~\cite{manoharan2019nonlinear} and propose a complete cooperative localization and path planning framework with moving horizon estimation (MHE) for estimating the vehicle position, and a nonlinear model predictive control (NMPC) framework for cooperative path planning, and a closed formulation for covariance calculation to  predicting the uncertainty. This framework uses a nonlinear vehicle model in both the controller and the estimator, which mitigates the linearization errors. The analytical expression used for the covariance calculation speeds up the computations and is derived by exploiting the relationship between the vehicle-landmark path lengths to the localization uncertainty. In most of the literature for multi-agent systems, the studies are formulated either as a control problem or an estimation problem \cite{Mourikis2006,Nerurkar2009,Roumeliotis2000,wan2014cooperative,wang2014optimization}. We propose a method that combines both and looks at the multi-agent problem in a holistic sense.

Previous studies \cite{Agha-Mohammadi2014,Mathew2015,wan2014cooperative} used algorithms that were not optimal and were based on conventional path planners, whereas nonlinear model predictive control (NMPC) provides optimal paths while satisfying imposed state and input constraints. The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. Also, most of the works based on graph-based planning give discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, eliminating the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2006maximizing} and \cite{de2006decentralized}. We also use a Laplacian matrix based solution, but we calculate Laplacian matrices for each vehicle instead of forming a single matrix for the whole group. This helps in identifying connectivity at an individual level, and each vehicle can decide to maintain, lose, or gain connections depending on their covariance estimates. This is not possible in the single matrix case because a single vehicle with more connections will increase the Laplacian, even though the other vehicles may be out of the required number of connections. 
Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy. The works on path planning with localization constraints \cite{singh2016landmarks,sundar2019path,kassas2021uav,irani2018localizability} consider only single vehicles and fixed landmarks in most cases, whereas our approach includes multiple vehicles, and each vehicle is considered a moving landmark. Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobians, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. Now, we can summarize the major contributions of this paper as follows:
\begin{itemize}
	\item A complete framework for control and estimation of multi-vehicle cooperative path planning problem with localization constraints using NMPC and MHE.
	\item An analysis on the relation of path lengths between vehicles and landmarks on the estimation covariance, from which an approximate expression for predicting the uncertainty was derived.
\end{itemize}

The rest of the paper is organized as follows. The problem formulation is given in Section \ref{sec:problem}. Moving horizon estimation (MHE) is explained in Section \ref{sec:MHE}. The derivation of the analytic expression for covariance is given in Section \ref{sec:analysis}. The NMPC formulation is given in Section \ref{sec:NMPC}. Simulation results are presented in Section \ref{sec:results}, and the conclusions are given in Section \ref{sec:conclusions}. 

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%	\caption{Block diagram showing the proposed NMPC-MHE control scheme.}
%	\label{fig:block}
%\end{figure} 

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=8cm]{figs/BlockDiagram.eps}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=8cm]{figs/covariance.eps}		
	\end{subfigure}\hfil 
	\caption{Block diagram and a graphical representation of the proposed NMPC-MHE control scheme. }
	\label{fig:block}
\end{figure}  

\section{Problem formulation}\label{sec:problem}	
%Around-the-clock delivery of essential supplies like medicines from one location to another is an important application of autonomous aerial vehicles \cite{ups2}. 
We consider a scenario where a group of AAVs need to navigate from their source location ($S$) to destination ($D$), as shown in Fig.~\ref{fig:scenario}. These vehicles need to transit in a GPS-denied area and we assume that any kind of GNSS are not available. In such scenarios, known landmarks or other vehicles in the area can be used for relative localization using range or bearing measurements. This structure involving landmarks and vehicles can be modeled as a dynamic relative position measurement graph (RPMG) \cite{sharma2011graph} with vehicles and landmarks as nodes and connections/measurements as edges.
\begin{definition}
	A relative position measurement graph (RPMG) for $n_v(t)$ vehicles with $n_l(t)$ landmarks is a graph $G_{n_v}^{n_l}(t)~\triangleq~\{\mathcal{V}_{n_v}^{n_l}(t),\mathcal{E}_{n_v}^{n_l}(t) \}$, where $\mathcal{V}_{n_v}^{n_l}$ is the node set consisting of $n_v(t)$ vehicle nodes and $n_l(t)$ landmark nodes (which makes a total of $n_v(t)+n_l(t)$ nodes), and $\mathcal{E}_{n_v}^{n_l}(t)$ is the edge set representing available relative measurements. The number of edges is denoted by $n_e(t)= |\mathcal{E}_{n_v}^{n_l}(t)|$.   
\end{definition}
\begin{definition}
	A path from a vehicle node to a landmark node is a finite sequence of edges which joins a sequence of distinct vertices between them. Let $\mathcal{G} \triangleq \{\mathcal{V},\mathcal{E},\phi\} $ be a graph. A path $\phi$ from vertex $i$ to vertex $j$ is a sequence of edges $\{\epsilon_1,\epsilon_2, \ldots, \epsilon_{n-1} \}$ for which there is a sequence of distinct vertices $\{\nu_1,\nu_2, \ldots, \nu_n \}$ such that $\phi \triangleq \{ \nu_1,\nu_n \}$ where $\nu_1 = i$ and $\nu_n = j$.
\end{definition}
An example RPMG ($G_{5}^{3}$ with $n_e=7$) is shown in Fig.~\ref{fig:rpmg}. A path from the vehicle $5$ to the landmark $a$ is represented by the edge set $\phi \triangleq \{\epsilon_6,\epsilon_5,\epsilon_3 \}$ which can also be represented using the vertices as $5-4-2-a$. 

Previous studies show that for cooperative localization to work, each vehicle should have a direct or indirect path to at least two known landmarks \cite{sharma2014observability}. This condition is very limiting in environments with a low number of landmarks. Hence in this paper, we find a relationship between vehicle uncertainty and path length to the landmarks and then use that relationship to formulate and solve an NMPC problem to guarantee that the covariance does not exceed a specified threshold and desired localization accuracy is achieved while performing individual missions. A moving horizon estimation (MHE) scheme is used to estimate the vehicle states. A block diagram and a graphical representation of the proposed solution using nonlinear model predictive control (NMPC) combined with MHE to tackle the cooperative localization and path planning problem is shown in Fig.~\ref{fig:block}. The optimal path is different from the shortest path since the latter does not satisfy localization constraints. The components of the block diagram are explained in the subsequent sections. In the first step of the control scheme, vehicle states are estimated by the MHE block using available measurements from the sensors (Sec.~\ref{sec:MHE}). The second step is the calculation of estimation covariances for the NMPC prediction window, which is accomplished by the covariance calculator block that contains the derived analytical expression (Sec.~\ref{sec:analysis}). In the third and final step, the NMPC controller computes the control actions for the vehicles (Sec.~\ref{sec:NMPC}). 


% 	\begin{figure}
	% 		\centering
	% 		\includegraphics[width=8cm]{figs/coop_scenario.eps}
	% 		\caption{Path planning scenario. }
	% 		\label{fig:scenario}
	% 	\end{figure}

%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
	%		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
	%		\caption{}
	%		\label{fig:scenario}
	%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
	%		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
	%		\caption{}
	%		\label{fig:rpmg}
	%	\end{subfigure}\hfil 
%		\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
%		\label{fig:path_graph}
%\end{figure}  

==> Introduction_old.tex <==
\section{Introduction}\label{sec:intro}
Urban air mobility (UAM) deals with highly automated, cooperative, passenger, and cargo-carrying aerial vehicles in urban areas \cite{faa}. Major companies like UPS \cite{ups1}, DHL \cite{dhl}, Amazon \cite{prime}, and Wing \cite{wing} are developing autonomous transportation systems for delivering cargo and medicines.
% Uber \cite{uber} and Airbus \cite{airbus} are working on autonomous aerial systems that can transport people. 
The use of autonomous aerial vehicles (AAVs) for various activities is expected to rise substantially in the near future \cite{sesar}.   

AAVs depend on Global navigation satellite systems (GNSS) for localization. However, there are situations in which GNSS is either unreliable or unavailable, such as urban canyon environments, intentional denial/jamming
of GNSS services \cite{van1996selective}, etc. In such scenarios, alternative localization schemes such as relative localization with respect to known landmarks \cite{betke1997mobile,thrun1998finding}, vision-based localization schemes \cite{lategahn2014vision,kim2005vision}, radio-frequency (RF), and ultra-wide-band (UWB) based methods \cite{seco2016robot,krishnan2007uwb,zhang2018linear}, and techniques using lidar \cite{xu2019indoor,wang2020intelligent,levinson2010robust} become important for AAVs to accomplish their tasks. The urban airspace is expected to contain a large number of AAVs, making the multi-vehicle localization and path planning a challenging task. Cooperative localization for multiple vehicles and path planning for a single vehicle with localization constraints have been studied~\cite{Kurazume1998,Roumeliotis2000,Spletzer2001,minaeian2016vision,sundar2019path,zheng2005evolutionary,mac2016heuristic}. However, cooperative path planning with localization constraints for multiple vehicles has not been adequately addressed in the literature.

\begin{figure}
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=0.45\linewidth]{figs/coop_scenario.eps}
		\caption{}
		\label{fig:scenario}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=0.45\linewidth]{figs/rpmg.eps}		
		\caption{}
		\label{fig:rpmg}
	\end{subfigure}
	\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
	\label{fig:path_graph}
\end{figure}  

In Cooperative localization, the agents localize using measurements obtained with respect to other agents or known features. The agents move in such a fashion as to help each other and improve the localization accuracy of the entire group. This idea has been studied by several researchers for the past decade and different techniques like treating the other agents as moving landmarks \cite{Kurazume1998,Roumeliotis2000,Spletzer2001,minaeian2016vision}, using features in the environment \cite{frohle2018cooperative}, and combining both static and moving objects for relative measurements \cite{pierre2018range} have been employed to achieve cooperative localization. Kurazume and Hirose \cite{Kurazume1998} proposed a localization scheme for multi-robot systems in which the robots alternatively act as landmarks and moving agents. When one group is in motion, the other group remains stationary and acts as landmarks for the other group. Roumeliotis and Bekey \cite{Roumeliotis2000} used a decentralized Kalman filter to optimally combine sensor information from each robot to localize a group of cooperative robots moving in a given space.
% Vision-based techniques were used in \cite{Spletzer2001} to localize a group of robots moving in a formation. 
Minaeian et al. \cite{minaeian2016vision} used a vision-based localization system for target detection and tracking. The formulation involves AAVs and ground vehicles in which the latter is used as moving landmarks for localizing the AAVs.
% Koohifar et al. \cite{koohifar2017receding} used a receding horizon scheme, which employs the Fisher information matrix to localize a moving target using AAVs. In \cite{frohle2018cooperative}, a cooperative localization method without explicit inter-vehicle measurements is proposed, where vehicles track mobile features in the environment to improve localization accuracy. 
% The papers \cite{liu2018multi,pierre2018range} proposed a cooperative localization algorithm based on range measurements using ultra wide band (UWB) sensors, where \cite{liu2018multi} used EKF for estimation, and in \cite{pierre2018range}, every static or mobile object was considered beacons for localization, and a split intersection covariance filter was used to estimate the poses. 
In \cite{liu2018multi}, a cooperative localization algorithm based on range measurements using ultra wide band (UWB) sensors and EKF for estimation is developed. In \cite{guo2019ultra}, a cooperative relative localization technique for AAVs based on UWB and odometry is proposed for multi-AAV formation control. An approach for cooperative localization under limited connectivity for multi-agent systems is given in \cite{zhu2019cooperative}. Each agent localizes in a global frame using a local filter, which uses local dead reckoning and intermittent absolute measurement updates and corrects its pose estimate whenever relative measurements with respect to
other agents are received. Rathinam and Sharma \cite{Rathinam2015}, and Wang et al. \cite{wang2019landmark} proposed an approach to optimally place landmarks to aid cooperative localization. The path from the source to the goal is fixed, and the algorithm is used to place the minimum number of landmarks along the way to achieve the required localization accuracy. In \cite{Mourikis2006}, the accuracy of position estimation
for groups of mobile robots performing cooperative localization is studied. The analysis is based on the eigenvalues of the relative position measurement graph (RPMG) of the system. 
% In \cite{piperigkos2020graph}, a graph-based cooperative localization scheme is given for semi-autonomous vehicles.
% The network of cars is modeled as an undirected relative position graph, and the solution is based on the Laplacian method. Our approach is also based on the relative position measurement graph, with relative bearing measurements obtained from vehicles and landmarks. But, instead of using a single adjacency matrix and Laplacian for all the vehicles, we define individual adjacency matrices for each vehicle. This helps in identifying connectivity at individual level, and each vehicle can decide to maintain, loose or gain connections depending on their covariance estimates. This is not possible in the single matrix case, because a single vehicle with more number of connections will increase the Laplacian, even though the other vehicles maybe out of required number of connections. 
 
% Previous studies on path planning were mainly based on genetic algorithms \cite{ismail2008mobile,dai2009path,albab2017path,panda2015effective,lu2016path,germi2018adaptive,roberge2012comparison}, artificial potential fields \cite{rimon1992exact,barraquand1992numerical,ge2000new,chen2016uav}, rapidly-exploring random trees (RRT) \cite{kuffner2000rrt}, and A* methods \cite{dolgov2010path,wang2018partitioning}. Kavraki et al. \cite{kavraki1996probabilistic} gave a solution based on probabilistic road-maps for path planning of holonomic robots. A broad survey on classical and heuristic path planning techniques is given in \cite{mac2016heuristic}.

%Sundar et al. \cite{sundar2019path} presented a path planning algorithm with localization constraints which ensured the vehicle is always connected to the required number of landmarks for localization. Scenarios involving multiple vehicles pose additional constraints/opportunities in the path planning problem, such as keeping a formation while in transit. Sometimes, vehicles need to maintain connections for information sharing or do cooperative tasks that a single vehicle cannot achieve.      
 
After the vehicle is accurately localized, the next challenge in urban mobility is planning the optimal path from one point to another. In \cite{Agha-Mohammadi2014,Mathew2015,bopardikar2015multiobjective}, the AAV transportation problem where the vehicles move between waypoints subject to different constraints were studied. Agha-Mohammadi et al.~\cite{Agha-Mohammadi2014} used graph based methods and forward search to generate real-time policies for the delivery drones, Mathew et al.~\cite{Mathew2015} proposed a solution using a novel reduction to the generalized traveling salesman problem, and Bopardikar et al.~\cite{bopardikar2015multiobjective} presented a graph-based probabilistic roadmap approach to tackle the multi-agent path planning problem.  
% Yun et al. \cite{Yun2013} also formulated an integrated navigation system to tackle the unavailability of GNSS by combining various sensor measurements. Another strategy for localization without GPS is given in \cite{wan2014cooperative}, where the AAVs exchanged relative range measurement information, and a posterior distribution was calculated using a dynamic nonparametric belief propagation (DNBP) scheme. In \cite{he2008planning}, a belief road map (BRM) algorithm was used to plan trajectories for a quadcopter without GPS. In \cite{zheng2005evolutionary}, a genetic algorithm-based route planner is proposed for cooperative path planning of AAVs.     

% Cooperative multi-agent algorithms need connectivity between agents for measurements, which is not easy to maintain over time due to constraints such as sensor range and goal-reaching objective. In \cite{kim2005maximizing}, an algorithm for maximizing the second smallest eigenvalue (algebraic connectivity) of the proximity graph Laplacian for multi-agent systems was proposed. A similar approach based on algebraic connectivity was proposed in \cite{de2006decentralized} to increase the connectivity of a multi-robot system. A decentralized potential-based control law was used to achieve the inter-robot distances dictated by a supergradient
% algorithm.
 
% Another critical aspect of the cooperative estimation problem is to satisfy the conditions for observability of the system. Perera et al. \cite{Perera2009} provide rigorous proofs for the observability properties of the general two dimensional SLAM problem with a number of landmarks in the context of piece-wise constant systems theory and non-linear Lie derivative theory. Yu et al.~\cite{yu2011observability} proposed an observability-based path planning algorithm for AAV navigation with obstacle avoidance. A nonlinear observability analysis was performed to obtain the necessary conditions for complete observability of the system, and these conditions were used to explicitly design a path that enhances observability while simultaneously avoiding collisions with obstacles.   
 
Urban air mobility calls for improved localization accuracy due to its innate nature involving close structures, narrow pathways, and a large number of vehicles. Moving horizon estimation (MHE) has been suggested as an alternate to EKF for increasing the accuracy of nonlinear estimation problems by \cite{rawlings2006particle,wang2014optimization,kayacan2014learning,mehrez2017optimization}.
% with \cite{wang2014optimization} proposing a cooperative localization approach for autonomous underwater vehicles, and \cite{mehrez2017optimization} for multi-robot systems.
Erunsal et al. \cite{erunsal2019decentralized} proposed an approach combining NMPC and pose-graph-MHE for 3D formation control of micro aerial vehicles with relative sensing capability. In \cite{liu2020decentralized}, a decentralized MHE technique is proposed for networked navigation with packet dropouts.    

% Cooperative localization with multiple vehicles and path planning with localization constraints is not adequately addressed in the literature. 
In this paper, we extend our work presented in \cite{manoharan2019nonlinear} on cooperative localization and path planning using NMPC by combining a moving horizon estimation (MHE) scheme for determining the vehicle states. Through this mechanism, the nonlinear vehicle model can be used on both the controller and the estimator, while mitigating linearization errors. Also, we replace the covariance calculation using the EKF-update with an analytical expression derived by exploiting the relationship between the vehicle-landmark path lengths to the localization uncertainty to speed up the computations. In most of the literature for multi-agent systems, the studies are formulated either as a control problem or an estimation problem \cite{Mourikis2006,Nerurkar2009,Roumeliotis2000,wan2014cooperative,wang2014optimization,brinon2014cooperative,shi2015cooperative,dong2008cooperative,khazaeni2016event,movric2013cooperative}. We propose a method that combines both and tries to look at the multi-agent problem in a holistic sense. Also, model predictive control is generally used to track a reference created using an auxiliary path planner. In contrast, we try to exploit the full potential of the NMPC as a planner and a controller without using any low-level controllers or auxiliary path planners. 
 
Previous studies \cite{Agha-Mohammadi2014,Mathew2015,Rathinam2015,Yun2013,wan2014cooperative} used algorithms that are not optimal and were based on conventional path planners, whereas nonlinear model predictive control (NMPC) provides optimal paths while satisfying imposed state and input constraints. The feedback and re-planing at each step help find accurate solutions in dynamically changing environments like moving landmarks. Also, most of the works based on graph-based planning gives discrete (node-to-node) paths \cite{bopardikar2015multiobjective}. Our design gives a continuous path, which eliminates the shortcomings of former approaches. The agent connectivity is maintained by ensuring nonzero eigenvalue of the graph Laplacian in \cite{kim2005maximizing} and \cite{de2006decentralized}. We also use a graph-based solution, but with smaller sub-graphs instead of a single graph. This helps in identifying connectivity at individual level, and each vehicle can decide to maintain, loose or gain connections depending on their covariance estimates. This is not possible in the single matrix case, because a single vehicle with more number of connections will increase the Laplacian, even though the other vehicles maybe out of required number of connections. 
Another advantage of the proposed scheme is that we relax the constraint of always maintaining connections with two landmarks \cite{Rathinam2015,wang2019landmark,sundar2019path} since sometimes it might be impossible to obtain a solution in environments with a lower number of landmarks. Also, if the observability condition is violated for a short time, the vehicles would be able to re-localize if it comes in the vicinity of another landmark. So we formulate a condition in the controller which tries to increase connections with the landmarks only if the estimation covariance of the vehicle increase beyond a given threshold. This formulation helps in obtaining solutions to the path planning problem while ensuring the required localization accuracy.         

Since the NMPC computes predictions for a time window, the anticipated covariances need to be calculated for the entire prediction horizon. Existing methods of propagating covariance through an EKF-like update equation will drastically increase the computation time since it involves the calculation of Jacobians, and for long prediction horizons, this will result in a significant increase in the computation time. Hence, an approximate analytic expression was derived for finding the vehicles' estimation covariances by analyzing how the path lengths between the vehicles and the landmarks in the relative position measurement graph (RPMG) affect the covariance values. 
The rest of the paper is organized as follows. The problem formulation is given in Section \ref{sec:problem}. Moving horizon estimation (MHE) is explained in Section \ref{sec:MHE}. The derivation of the analytic expression for covariance is given in Section \ref{sec:analysis}. The NMPC formulation is given in Section \ref{sec:NMPC}. Simulation results are presented in Section \ref{sec:results}, and the conclusions are given in Section \ref{sec:conclusions}. 

	\begin{figure}[h]
	\centering
	\includegraphics[width=8cm]{figs/BlockDiagram.eps}
	\caption{Block diagram showing the proposed NMPC-MHE control scheme.}
	\label{fig:block}
\end{figure} 

\section{Problem formulation}\label{sec:problem}	
%Around-the-clock delivery of essential supplies like medicines from one location to another is an important application of autonomous aerial vehicles \cite{ups2}. 
We consider a scenario where a group of AAVs need to navigate from their source location ($S$) to destination ($D$), as shown in Fig.~\ref{fig:scenario}. These vehicles need to transit in a GPS-denied area and we assume that any kind of GNSS are not available. In such scenarios, known landmarks or other vehicles in the area can be used for relative localization using range or bearing measurements. This structure involving landmarks and vehicles can be modeled as a dynamic relative position measurement graph (RPMG) \cite{sharma2011graph} with vehicles and landmarks as nodes and connections/measurements as edges.
\begin{definition}
A relative position measurement graph (RPMG) for $n_v(t)$ vehicles with $n_l(t)$ landmarks is a graph $G_{n_v}^{n_l}(t)~\triangleq~\{\mathcal{V}_{n_v}^{n_l}(t),\mathcal{E}_{n_v}^{n_l}(t) \}$, where $\mathcal{V}_{n_v}^{n_l}$ is the node set consisting of $n_v(t)$ vehicle nodes and $n_l(t)$ landmark nodes (which makes a total of $n_v(t)+n_l(t)$ nodes), and $\mathcal{E}_{n_v}^{n_l}(t)$ is the edge set representing available relative measurements. The number of edges is denoted by $n_e(t)= |\mathcal{E}_{n_v}^{n_l}(t)|$.   
\end{definition}
\begin{definition}
A path from a vehicle node to a landmark node is a finite sequence of edges which joins a sequence of distinct vertices between them. Let $\mathcal{G} \triangleq \{\mathcal{V},\mathcal{E},\phi\} $ be a graph. A path $\phi$ from vertex $i$ to vertex $j$ is a sequence of edges $\{\epsilon_1,\epsilon_2, \ldots, \epsilon_{n-1} \}$ for which there is a sequence of distinct vertices $\{\nu_1,\nu_2, \ldots, \nu_n \}$ such that $\phi \triangleq \{ \nu_1,\nu_n \}$ where $\nu_1 = i$ and $\nu_n = j$.
\end{definition}
An example RPMG ($G_{5}^{3}$ with $n_e=7$) is shown in Fig.~\ref{fig:rpmg}. A path from the vehicle $5$ to the landmark $a$ is represented by the edge set $\phi \triangleq \{\epsilon_6,\epsilon_5,\epsilon_3 \}$ which can also be represented using the vertices as $5-4-2-a$. 

Previous studies show that for cooperative localization to work, each vehicle should have a direct or indirect path to at least two known landmarks \cite{sharma2014observability}. This condition is very limiting in environments with a low number of landmarks. Hence in this paper, we find a relationship between vehicle uncertainty and path length to the landmarks and then use that relationship to formulate and solve an NMPC problem to guarantee that the covariance does not go beyond a specified threshold and desired localization accuracy is achieved while performing individual missions. A moving horizon estimation (MHE) scheme is used to estimate the vehicle states. A block diagram of the proposed solution using nonlinear model predictive control (NMPC) combined with MHE to tackle the cooperative path planning and localization problem is shown in Fig.~\ref{fig:block}, and is explained in the subsequent sections. In the first step of the control scheme, vehicle states are estimated by the MHE block using available measurements from the sensors (Sec.~\ref{sec:MHE}). Second step is the calculation of estimation covariances for the NMPC prediction window. This is accomplished by the covariance calculator block, which contains the derived analytical expression (Sec.~\ref{sec:analysis}). In the third and final step, the NMPC controller computes the control actions for the vehicles (Sec.~\ref{sec:NMPC}). 


% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/coop_scenario.eps}
% 		\caption{Path planning scenario. }
% 		\label{fig:scenario}
% 	\end{figure}

%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/coop_scenario.eps}
%		\caption{}
%		\label{fig:scenario}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/rpmg.eps}		
%		\caption{}
%		\label{fig:rpmg}
%	\end{subfigure}\hfil 
%		\caption{(a) Path planning scenario. (b) Relative position measurement graph with vehicles and landmarks as nodes and measurements as edges. }
%		\label{fig:path_graph}
%\end{figure}  

==> MHE.tex <==
\section{Moving horizon estimation}\label{sec:MHE}
Moving horizon estimation (MHE) uses optimization techniques to find state trajectories that best fit a series of measurements acquired over a finite time interval. It uses the exact nonlinear models of the available measurements and system dynamics for estimation. Also, there is another advantage of including the state/control constraints in the formulation, which helps in bounding the estimates. Like NMPC, MHE also has three main components, 1) an internal dynamic model of the process, 2) a history of past measurements, and 3) an optimization cost function over the estimation horizon.
%In MHE, an iterative approach based on linear or nonlinear programming is used to find the estimates. 
%MHE is superior to the extended Kalman filter (EKF), the most commonly used nonlinear estimator for multi-agent systems~\cite{haseltine2005critical} since the EKF linearizes nonlinear models at operating points.  
%Also, EKF is based on the Markov assumption that the current state estimate is based only on the most recent measurements and the previous state estimate. Since the MHE minimizes the deviation of the model from the past interval of measurements, the Markov assumption is relaxed.  

The model used for estimation is given as:
\begin{eqnarray}
X(k)&=&f\left( X(k-1),\boldsymbol{\omega}(k),k\right) +q(k), \label{eq:f}\\
z(k)&=&h\left( X(k),\boldsymbol{\omega}(k),k\right) + \mu(k), \label{eq:z}
\end{eqnarray}	
where, $f(\cdot)$ and $h(\cdot) $ represent the state model and the observation model respectively. ${X}(k)$ and $ z(k) $ are the system states and measurements at the $k^{\mathrm{th}}$ time instant. The vectors $ q(k) $ and $ \mu(k) $ are the process and measurement noises which are assumed to be additive and zero mean white Gaussian noises with covariance $ Q $ and $ \Gamma $ respectively. $ f(\cdot) $ is defined as
	\begin{equation}
	f=\begin{bmatrix}
	x_{1}(k)\\
	y_{1}(k)\\
	\psi_{1}(k)\\
	\vdots\\
	x_{n_v}(k)\\
	y_{n_v}(k)\\
	\psi_{n_v}(k)
	\end{bmatrix}=
	\begin{bmatrix}
	x_{1}(k-1)+T_sv\cos\psi_{1}(k-1)\\
	y_{1}(k-1)+T_sv\sin\psi_{1}(k-1)\\
	\psi_{1}(k-1)+T_s\omega_1(k-1)\\
	\vdots\\
	x_{n_v}(k-1)+T_sv\cos\psi_{n_v}(k-1)\\
	y_{n_v}(k-1)+T_sv\sin\psi_{n_v}(k-1)\\
	\psi_{n_v}(k-1)+T_s\omega_{n_v}(k-1)
	\end{bmatrix},
	\end{equation}
where $ T_s $ is the sampling time used for discretization.

The moving horizon estimation problem can be formulated as:
\begin{equation}
\min_{X}J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{P^{-1}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2 , 
\label{eq:MHE_cost}
\end{equation} 
	subject to:
	\begin{align*}
	X_{k+1}&= f(X_{k},\boldsymbol{\omega}_{k}),\\
	\boldsymbol{\omega}&\in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
where $m$ is the current time step, $N_E$ is the estimation horizon, $\hat{X}$ is the estimated states, $P$ is the estimation covariance matrix, and $\Gamma$ is the measurement covariance. It is assumed that each vehicle can measure relative bearing to other vehicles and landmarks that are in the sensor's field-of-view. Relative bearing from the $i^{th}$ vehicle to the $j^{th}$ vehicle or landmark is given by the measurement model:
\begin{equation}
h(X)=\tan^{-1} \left( \frac{y_{j}-y_{i}}{x_{j}-x_{i}}\right)-\psi_i.
\end{equation} 

The first term in (\ref{eq:MHE_cost}) is known as the arrival cost and it plays an important role in stabilizing the estimator. It penalizes the deviation of the first state in the moving horizon window and its previous estimate $ \hat{X}_{m-N_E} $. The weighting matrix $ P $ is given by~\cite{rao2003constrained}
\begin{equation}
P_{k+1}=Q+\nabla F_{X}( P_k-  P_k\nabla H_{X}^{T}( \nabla H_{X}P_k\nabla H_{X}^{T}+\Gamma) ^{-1}\nabla H_{X}P_k) \nabla F_{X}^{T},
\end{equation}
where $Q$ is the state covariance matrix, and $ \nabla F_{X},\nabla H_{X} $ are the Jacobians of $ f $ and $ h $. 
%given by
%	\begin{equation}
%	\nabla F_{X}=\frac{\partial f}{\partial X_i}=
%	\begin{bmatrix}
%	1 & 0 & -T_sv\sin\psi_{i}\\
%	0 & 1 & T_sv\cos\psi_{i}\\
%	0& 0&1
%	\end{bmatrix},
%	\end{equation}
%		\begin{equation}
%		\nabla H_{X}=\frac{\partial h}{\partial X_i}=\begin{bmatrix}
%		\frac{y_{j}-y_{i}}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}&
%		\frac{-(x_{j}-x_{i})}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}& -1
%		\end{bmatrix}.
%		\end{equation}
The second term in (\ref{eq:MHE_cost}) penalizes the change in predicted measurements $ h(X_{k}) $ from the actual measurements $ z_{k} $.

Now, we look into the stability of the moving horizon estimator. The following assumptions are required for proving the stability result.

%\subsection{Assumptions}
\begin{assumption}
The initial state $X_0$ and the control input $\omega$ are such that, for any noise $q$, the system trajectory $X$ lies in a compact set $\chi$ and $\omega$ in a compact set $U$.
\label{assump:MHE1}	
\end{assumption}
\begin{assumption}
	The functions $f$ and $h$ are $C^2$ functions w.r.t $X$ on $ co(\chi) $ for every $\omega \in U$, where $co(\chi)$ is the convex closure of $ \chi $.
	\label{assump:MHE2}
\end{assumption}

Observation map for a horizon $N_E+1$ can be defined as 
\begin{equation}
F^{N_E}(X,\omega,q) = \begin{bmatrix}
h(X_{m-N_E}) \\
h \circ f^{m-N_E}(X_{m-N_E})\\
\cdot\\
\cdot\\
\cdot\\
h \circ f^{m-1} \circ \cdot \cdot \cdot f^{m-N_E}(X_{m-N_E})
\end{bmatrix},
\end{equation}
where $\circ$ is function composition. Then it is possible to re-write equation (\ref{eq:z}) as
\begin{equation}
z_{m-N_E} = F^{N_E}(X,\omega,q) + \mu_{m-N_E},
\end{equation} 
and modify the cost function as
\begin{multline}
J_m(X_{m-N_E,\hat{X}_{m-N_E}})= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \lVert F^{N_E}(X_{m-N_E},\omega_{m-N_E},q_{m-N_E}) - z_{m-N_E} \rVert_{\mathbf{\Gamma}}^2,       
\end{multline} 
$ \mathbf{\Gamma} = I_{N_E+1} \otimes \Gamma^{-1} $, where $\otimes$ is the Kronecker product.

Now, let's consider the following remarks:
\begin{remark}
	System (\ref{eq:f}), (\ref{eq:z}) is said to be observable in $N_E+1$ steps if there exists a $K$-function $\phi(\cdot)$ such that
	$
		\phi\left( \lVert x_1-x_2 \rVert^2 \right) \leq \lVert F^{N_E}(x_1,\omega,0) - F^{N_E}(x_2,\omega,0) \rVert^2,  
	$   
	$\forall x_1,x_2 \in \chi$ and $\forall \omega \in U^{N_E}$.
	\label{rem:MHE1}
\end{remark}
\begin{remark}
	 If the observability matrix $ \frac{\partial F^{N_E}(X,\omega,0)}{\partial X} $ has full rank, then the system is said to be observable in $N_E+1$ steps with finite sensitivity $1/\delta$ if the $K$-function $\phi(\cdot)$ satisfies the following condition
	\begin{equation}
		\delta = \inf_{x_1,x_2\in \chi;x_1 \neq x_2} \frac{\phi\left( \lVert x_1-x_2 \rVert^2 \right)}{ \lVert x_1-x_2 \rVert^2 } \geq 0.
	\end{equation}
\label{rem:MHE2}
\end{remark} 
Let $k_f$ be an upper bound on the Lipschitz constant of $f(X,\omega)$ w.r.t $X$ on $\chi$ for every $\omega \in U$ and $\mathbb{P}$ is diagonal with $ \mathbb{P} = pI_n, p>0 $. Let
\begin{equation}
r_{\mu} = \max_{\mu\in M} \lVert \mu \rVert^2,
\end{equation}
where $M$ is a compact set with $0\in M$. 

%\subsection{Stability}
Stability of the estimator is proved using the results from \cite{alessandri1999neural,rao2003constrained,alessandri2008moving,alessandri2010advances}. 
Consider the cost function defined as: 
\begin{equation}
	J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2,
	\label{eq:stab_cost}
\end{equation}
then we can state the following theorem~\cite{alessandri2008moving,alessandri2010advances}.

\begin{theorem}
If the Assumptions \ref{assump:MHE1},\ref{assump:MHE2} are satisfied and the Remarks \ref{rem:MHE1},\ref{rem:MHE2} hold, then there exists an upper bound defined by
\begin{equation}
\lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert^2 \leq \zeta_{m-N_E},
\end{equation} 
where $\zeta_m$ is found using the equation
\begin{equation}
\zeta_{m+1} = \left(\frac{c_1k_fp}{p+c_2\delta}\right)\zeta_m + \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu},
\label{eq:bound}
\end{equation}
$c_1,c_2$, and $c_3$ are positive constants. Let
\begin{equation}
a(p,\delta) = \frac{c_1k_fp}{(p+c_2\delta)},
\end{equation}
and if $p$ is selected such that $ a(p,\delta) <1 $, then the dynamics of (\ref{eq:bound}) is asymptotically stable. 
\end{theorem}
\begin{proof}
	A summary of the proof given by~\cite{alessandri2008moving} is detailed here for completeness. The proof is based on defining upper and lower bounds on the optimal cost $J_{m}^*$, which is the cost corresponding to an optimal estimate $\hat{X}_{m-N_E}^{*}$. First, the upper bound on $J_{m}^*$ should be defined. Let us define $X_{m}^o$ as the true value of the state $X$ at time $m$ and assume that $\Gamma = I$. We have that
	\begin{equation}
	    J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert F^{N_E}(X_{k}^o) - z_{k} \rVert^2,
	\end{equation}
	which can be modified as
	\begin{equation}
	   J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C, \label{eqn:lower_bound}  
	\end{equation}
	where $C$ is a positive constant (please see Lemma. 1 from \cite{alessandri2008moving}). Next, the upper bound on $J_{m}^*$ is defined. We can write
	\begin{eqnarray*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 &=& \lVert [z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E})] - [z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,\\
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 & \leq &2 \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 + 2 \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2, \\
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 & \geq & \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2.
	\end{eqnarray*}
	From (\ref{eqn:lower_bound}), we can write
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2 < C.
	\end{equation}
	Hence, we obtain
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 \geq \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - C. 
	\end{equation}
	By using a similar procedure, we can write
	\begin{equation}
	    \lVert X_{m-N_E}^* - \hat{X}_{m-N_E} \rVert^2 \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E} \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2. 
	\end{equation}
	Now the upper bound can be defined as
	\begin{equation}
	    J_{m}^* \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C. \label{eqn:upper_bound}
	\end{equation}
	Now, by combining the bounds (\ref{eqn:lower_bound}) and (\ref{eqn:upper_bound}) we get
	\begin{multline}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C \\ \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C,
	\end{multline}
	which can be written as
	\begin{equation}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 \leq 2 \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + 2C.
	\end{equation}
	According to the Remarks \ref{rem:MHE1} and \ref{rem:MHE2}, it can be written that
	\begin{equation*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 = \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right),
	\end{equation*}
	and
	\begin{equation*}
	    \delta \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right).
	\end{equation*}
	Now, it is possible to define the bound on the estimation error as
	\begin{equation}
	    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \frac{4p}{p+\delta}\lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 + \frac{4}{p+\delta}C.
	\end{equation}
	Using the Lipschitz continuity of $f(\cdot)$, it can be written that
	\begin{equation}
	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 = 2k_f \lVert X_{m-N_E-1}^o - \hat{X}_{m-N_E-1}^* \rVert^2 + 2r_{\mu}.
	\end{equation}
Hence,
\begin{equation*}
    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \zeta_{m-N_E}.
\end{equation*}
It can also be deduced that if $\zeta_m < \zeta_{m-1}$ and $a(p,\delta)<1$, then $\zeta_m$ tends to $\frac{\beta}{1-a(p,\delta)}$ as $m \longrightarrow +\infty$ (please see Theorem~1 from~\cite{alessandri1999neural}), where $\beta~=~ \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu} $. 	
\end{proof}

The following section presents the derivation of the analytical expression for calculating the covariances using the path information. This result will be later used for predicting covariances for the NMPC cost function.

==> NMPC.tex <==
\section{NMPC formulation}\label{sec:NMPC}
Nonlinear model predictive control (NMPC) is a state-of-the-art technique for real-time optimal control. At each time step, the constrained optimization problem is solved based on the plant model for a finite time horizon, and the procedure is repeated with states updated through feedback in the next iteration~\cite{MPCbook}. Fig.~\ref{fig:block} shows the block diagram of the NMPC scheme used in this paper. The optimal control sequence is computed for the prediction horizon $ \tau_h $ from which only the first action is applied to the system at each time step. 
	 
%	\begin{figure}[h]
%		\centering
%		\includegraphics[width=8cm]{figs/BlockDiagram.eps}
%		\caption{NMPC block diagram }
%		\label{fig:block}
%	\end{figure}
	
 A point mass kinematic model is considered for the vehicles. We assume that the altitude and velocities of the AAVs remain constant during transit. 
	\begin{equation}
	\dot{X} =
	\begin{bmatrix}
	v\cos \psi_1   \\
	v\sin \psi_1\\
	\omega_1 \\
	\vdots \\
	v\cos \psi_{n_v}   \\
	v\sin \psi_{n_v}\\
	\omega_{n_v} \\        
	\end{bmatrix},
	\end{equation}  
 where  $ v $ is the linear velocity, $ \psi $ the heading angle, $ \omega $ the angular velocity, and $ n_v $ is the number of vehicles.
	
The objective function for the NMPC is defined as
	\begin{equation}
	\min_{\boldsymbol{\omega_1 \cdots \omega_{n_v}} \in \mathcal{PC}(t,t+\tau_h)}J=\int_{t}^{t+\tau_h}\sum_{i=1}^{n_v} \left[ C_{1_i}+W_iC_{2_i}\right], 
	\label{eq:PI}
	\end{equation}	
	subject to:
	\begin{align*}
	\dot{X} &= f(X,\boldsymbol{\omega}),\\
	\boldsymbol{\omega} & \in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
	where 
	\begin{equation}
	C_{1_i}=(x_i-x_{D_i})^{2}+(y_i-y_{D_i})^{2}, 
	\end{equation}
is the cost associated with minimizing the distance between the vehicle and the destination. $(x_i,y_i) $ is the position of the $ i^{th} $ vehicle and $ (x_{D_i},y_{D_i}) $ are their respective destination points. $ \boldsymbol{\omega}^{-} $ and $ \boldsymbol{\omega}^{+}$ are the lower and upper bounds of $\boldsymbol{\omega}$, and $ \mathcal{PC}(t,t+\tau_h) $ denotes the space of piece-wise continuous function defined over the time interval $ \left[ t,t+\tau_h\right]  $.
	
$C_{2_i}$ is the cost associated with keeping the estimation covariance under bound, which is defined as:
	\begin{equation}
	C_{2_i}=\begin{cases}
	0, & \text{if $\lambda_i \geq \eta$}.\\
	(\eta-\lambda_i)^{2}, & \text{ otherwise}.
	\end{cases} \label{eq:C2}
	\end{equation} 
where $ \eta $ is a tuning parameter related to the number of connections required. Increasing $ \eta $ will result in vehicles moving closer to the landmarks and increase the connections. For satisfactory localization, observability conditions should be satisfied, which require connections with at least two landmarks~\cite{sharma2014observability}. Hence, the value of $\eta$ should be selected as~$ \eta \geq 2 $. The parameter $\lambda_i $ is the second smallest eigenvalue of the Laplacian matrix which is formed as:
	\begin{equation}
	L_i(X)=\Delta_i(X)-A_i(X),
	\end{equation} 
where $ A_i(X) $ is the adjacency matrix defined similar to~\cite{de2006decentralized} as
	\begin{equation}
	A_{i_{mn}}=\begin{cases}
	e^{\frac{-\kappa(||R_{mn}||-\rho)}{R_{s}-\rho}}, & \text{$\left| \left| R_{mn}\right| \right| \leq R_s$}.\\
	0, & \text{$\left| \left| R_{mn}\right| \right| > R_s$}.
	\end{cases}
	\end{equation} 
	and
	$ \Delta_i(X) $ is a diagonal matrix with elements
	\begin{equation}
	\Delta_{i_{mm}}=\sum_{n=1}^{N}A_{i_{mn}}
	\end{equation}
where $ m,n= 1  $ to $ N $, and $ N $ is the number of nodes of the graph connecting the vehicles and landmarks. $ \kappa $ is a constant which determines the convergence rate of the exponential function, and $\rho$ is used to set a minimum distance between the landmarks and the vehicles to avoid collisions. $ ||R_{mn}|| $ is the distance between the $ m^{th} $ and $ n^{th} $ nodes, and $ R_s $ is the sensor range of the vehicles. This formulation of the adjacency matrices, rather than updating it with binary values, helps drive the vehicles closer to the landmarks than just maintaining the connections by keeping them in the sensor range and lowering the distance between the landmarks and the vehicles help in decreasing the estimation covariance as explained in sec.~\ref{sec:analysis}. The maximum value $ \lambda_i $ can take is equal to the number of connections of each vehicle, and this insight is used in formulating (\ref{eq:C2}).   
	
The weight $W_i$ associated with $ C_{2_i} $ is defined in the following way
	\begin{equation}
	W_i=\begin{cases}
	W, & \text{if $3\sigma_{p_i} \geq \sigma_c$}.\\
	0, & \text{ otherwise}.
	\end{cases}
	\end{equation} 
where $\sigma_{p_i}$ is the standard deviation in the estimated position of the $ i^{th} $ vehicle and the constant $\sigma_c$ is the specified critical value. This adaptive weight formulation is used to get a trade-off between the two objectives. $\sigma_{p_i} $s are calculated using the expression
\begin{equation}
\sigma_{p_i}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_i-\theta_g))} \right)+(R_g^2+R_g^4)\csc^2(\psi_i-\theta_g), 
\label{eq:s_bearing_i}
\end{equation} 
which is explained in detail in section \ref{sec:b_measurement}. The terms $C_1$ and $ C_2 $ of the objective function (\ref{eq:PI}) is normalized as follows:
	\begin{eqnarray}
	C_1(t)&=&\left(\frac{C_1(t) - \min(C_1(t))}{\max(C_1(t)) - \min(C_1(t))}\right),\\
	C_2(t)&=&\left(\frac{C_2(t) - \min(C_2(t))}{\max(C_2(t)) - \min(C_2(t))}\right).
	\end{eqnarray}
	

==> mhe_2c.tex <==
\section{Moving horizon estimation}\label{sec:MHE}
Moving horizon estimation (MHE) uses optimization techniques to find state trajectories that best fit a series of measurements acquired over a finite time interval. It uses the exact nonlinear models of the available measurements and system dynamics for estimation. Also, there is another advantage of including the state/control constraints in the formulation, which helps in bounding the estimates. Like NMPC, MHE also has three main components, 1) an internal dynamic model of the process, 2) a history of past measurements, and 3) an optimization cost function over the estimation horizon.
%In MHE, an iterative approach based on linear or nonlinear programming is used to find the estimates. 
%MHE is superior to the extended Kalman filter (EKF), the most commonly used nonlinear estimator for multi-agent systems~\cite{haseltine2005critical} since the EKF linearizes nonlinear models at operating points.  
%Also, EKF is based on the Markov assumption that the current state estimate is based only on the most recent measurements and the previous state estimate. Since the MHE minimizes the deviation of the model from the past interval of measurements, the Markov assumption is relaxed.  

The model used for estimation is given as:
\begin{eqnarray}
X(k)&=&f\left( X(k-1),\boldsymbol{\omega}(k),k\right) +q(k), \label{eq:f}\\
z(k)&=&h\left( X(k),\boldsymbol{\omega}(k),k\right) + \mu(k), \label{eq:z}
\end{eqnarray}	
where, $f(\cdot)$ and $h(\cdot) $ represent the state model and the observation model respectively. ${X}(k)$ and $ z(k) $ are the system states and measurements at the $k^{\mathrm{th}}$ time instant. The vectors $ q(k) $ and $ \mu(k) $ are the process and measurement noises which are assumed to be additive and zero mean white Gaussian noises with covariance $ Q $ and $ \Gamma $ respectively. $ f(\cdot) $ is defined as
	\begin{equation}
	f=\begin{bmatrix}
	x_{1}(k)\\
	y_{1}(k)\\
	\psi_{1}(k)\\
	\vdots\\
	x_{n_v}(k)\\
	y_{n_v}(k)\\
	\psi_{n_v}(k)
	\end{bmatrix}=
	\begin{bmatrix}
	x_{1}(k-1)+T_sv\cos\psi_{1}(k-1)\\
	y_{1}(k-1)+T_sv\sin\psi_{1}(k-1)\\
	\psi_{1}(k-1)+T_s\omega_1(k-1)\\
	\vdots\\
	x_{n_v}(k-1)+T_sv\cos\psi_{n_v}(k-1)\\
	y_{n_v}(k-1)+T_sv\sin\psi_{n_v}(k-1)\\
	\psi_{n_v}(k-1)+T_s\omega_{n_v}(k-1)
	\end{bmatrix},
	\end{equation}
where $ T_s $ is the sampling time used for discretization.

The moving horizon estimation problem can be formulated as:
\begin{equation}
\min_{X}J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{P^{-1}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2 , 
\label{eq:MHE_cost}\nonumber
\end{equation} 
	subject to:
	\begin{align*}
	X_{k+1}&= f(X_{k},\boldsymbol{\omega}_{k}),\\
	\boldsymbol{\omega}&\in\left[ \boldsymbol{\omega}^{-},\boldsymbol{\omega}^{+}\right], 
	\end{align*}
where $m$ is the current time step, $N_E$ is the estimation horizon, $\hat{X}$ is the estimated states, $P$ is the estimation covariance matrix, and $\Gamma$ is the measurement covariance. It is assumed that each vehicle can measure relative bearing to other vehicles and landmarks that are in the sensor's field-of-view. Relative bearing from the $i^{th}$ vehicle to the $j^{th}$ vehicle or landmark is given by the measurement model:
\begin{equation}
h(X)=\tan^{-1} \left( \frac{y_{j}-y_{i}}{x_{j}-x_{i}}\right)-\psi_i.
\end{equation} 

The first term in (\ref{eq:MHE_cost}) is known as the arrival cost and it plays an important role in stabilizing the estimator. It penalizes the deviation of the first state in the moving horizon window and its previous estimate $ \hat{X}_{m-N_E} $. The weighting matrix $ P $ is given by~\cite{rao2003constrained}
\begin{eqnarray}
P_{k+1}&=&Q+\nabla F_{X}( P_k-  P_k\nabla H_{X}^{T}( \nabla H_{X}P_k\nabla H_{X}^{T}+\Gamma) ^{-1}\nonumber\\
&&\nabla H_{X}P_k) \nabla F_{X}^{T},\nonumber
\end{eqnarray}
where $Q$ is the state covariance matrix, and $ \nabla F_{X},\nabla H_{X} $ are the Jacobians of $ f $ and $ h $. 
%given by
%	\begin{equation}
%	\nabla F_{X}=\frac{\partial f}{\partial X_i}=
%	\begin{bmatrix}
%	1 & 0 & -T_sv\sin\psi_{i}\\
%	0 & 1 & T_sv\cos\psi_{i}\\
%	0& 0&1
%	\end{bmatrix},
%	\end{equation}
%		\begin{equation}
%		\nabla H_{X}=\frac{\partial h}{\partial X_i}=\begin{bmatrix}
%		\frac{y_{j}-y_{i}}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}&
%		\frac{-(x_{j}-x_{i})}{\left( x_{j}-x_{i}\right) ^{2}+\left( y_{j}-y_{i}\right) ^{2}}& -1
%		\end{bmatrix}.
%		\end{equation}
The second term in (\ref{eq:MHE_cost}) penalizes the change in predicted measurements $ h(X_{k}) $ from the actual measurements $ z_{k} $.

Now, we look into the stability of the moving horizon estimator. The following assumptions are required for proving the stability result.

%\subsection{Assumptions}
\begin{assumption}
The initial state $X_0$ and the control input $\omega$ are such that, for any noise $q$, the system trajectory $X$ lies in a compact set $\chi$ and $\omega$ in a compact set $U$.
\label{assump:MHE1}	
\end{assumption}
\begin{assumption}
	The functions $f$ and $h$ are $C^2$ functions w.r.t $X$ on $ co(\chi) $ for every $\omega \in U$, where $co(\chi)$ is the convex closure of $ \chi $.
	\label{assump:MHE2}
\end{assumption}

Observation map for a horizon $N_E+1$ can be defined as 
\begin{equation}
F^{N_E}(X,\omega,q) = \begin{bmatrix}
h(X_{m-N_E}) \\
h \circ f^{m-N_E}(X_{m-N_E})\\
\cdot\\
\cdot\\
\cdot\\
h \circ f^{m-1} \circ \cdot \cdot \cdot f^{m-N_E}(X_{m-N_E})
\end{bmatrix},
\end{equation}
where $\circ$ is function composition. Then it is possible to re-write equation (\ref{eq:z}) as
\begin{equation}
z_{m-N_E} = F^{N_E}(X,\omega,q) + \mu_{m-N_E},
\end{equation} 
and modify the cost function as
\begin{multline}
J_m(X_{m-N_E,\hat{X}_{m-N_E}})= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  +\\ \lVert F^{N_E}(X_{m-N_E},\omega_{m-N_E},q_{m-N_E}) - z_{m-N_E} \rVert_{\mathbf{\Gamma}}^2,       
\end{multline} 
$ \mathbf{\Gamma} = I_{N_E+1} \otimes \Gamma^{-1} $, where $\otimes$ is the Kronecker product.

Now, let's consider the following remarks:
\begin{remark}
	System (\ref{eq:f}), (\ref{eq:z}) is said to be observable in $N_E+1$ steps if there exists a $K$-function $\phi(\cdot)$ such that
	$
		\phi\left( \lVert x_1-x_2 \rVert^2 \right) \leq \lVert F^{N_E}(x_1,\omega,0) - F^{N_E}(x_2,\omega,0) \rVert^2,  
	$   
	$\forall x_1,x_2 \in \chi$ and $\forall \omega \in U^{N_E}$.
	\label{rem:MHE1}
\end{remark}
\begin{remark}
	 If the observability matrix $ \frac{\partial F^{N_E}(X,\omega,0)}{\partial X} $ has full rank, then the system is said to be observable in $N_E+1$ steps with finite sensitivity $1/\delta$ if the $K$-function $\phi(\cdot)$ satisfies the following condition
	\begin{equation}
		\delta = \inf_{x_1,x_2\in \chi;x_1 \neq x_2} \frac{\phi\left( \lVert x_1-x_2 \rVert^2 \right)}{ \lVert x_1-x_2 \rVert^2 } \geq 0.
	\end{equation}
\label{rem:MHE2}
\end{remark} 
Let $k_f$ be an upper bound on the Lipschitz constant of $f(X,\omega)$ w.r.t $X$ on $\chi$ for every $\omega \in U$ and $\mathbb{P}$ is diagonal with $ \mathbb{P} = pI_n, p>0 $. Let
\begin{equation}
r_{\mu} = \max_{\mu\in M} \lVert \mu \rVert^2,
\end{equation}
where $M$ is a compact set with $0\in M$. 

%\subsection{Stability}
Stability of the estimator is proved using the results from \cite{alessandri1999neural,rao2003constrained,alessandri2008moving,alessandri2010advances}. 
Consider the cost function defined as: 
\begin{equation}
	J= \lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert h(X_{k}) - z_{k} \rVert_{\Gamma^{-1}}^2,
	\label{eq:stab_cost}
\end{equation}
then we can state the following theorem~\cite{alessandri2008moving,alessandri2010advances}.

\begin{theorem}
If the Assumptions \ref{assump:MHE1},\ref{assump:MHE2} are satisfied and the Remarks \ref{rem:MHE1},\ref{rem:MHE2} hold, then there exists an upper bound defined by
\begin{equation}
\lVert X_{m-N_E} - \hat{X}_{m-N_E} \rVert^2 \leq \zeta_{m-N_E},
\end{equation} 
where $\zeta_m$ is found using the equation
\begin{equation}
\zeta_{m+1} = \left(\frac{c_1k_fp}{p+c_2\delta}\right)\zeta_m + \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu},
\label{eq:bound}
\end{equation}
$c_1,c_2$, and $c_3$ are positive constants. Let
\begin{equation}
a(p,\delta) = \frac{c_1k_fp}{(p+c_2\delta)},
\end{equation}
and if $p$ is selected such that $ a(p,\delta) <1 $, then the dynamics of (\ref{eq:bound}) is asymptotically stable. 
\end{theorem}
\begin{proof}
	A summary of the proof given by~\cite{alessandri2008moving} is detailed here for completeness. The proof is based on defining upper and lower bounds on the optimal cost $J_{m}^*$, which is the cost corresponding to an optimal estimate $\hat{X}_{m-N_E}^{*}$. First, the upper bound on $J_{m}^*$ should be defined. Let us define $X_{m}^o$ as the true value of the state $X$ at time $m$ and assume that $\Gamma = I$. We have that
	\begin{equation}
	    J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2  + \sum_{k=m-N_E}^{m} \lVert F^{N_E}(X_{k}^o) - z_{k} \rVert^2,
	\end{equation}
	which can be modified as
	\begin{equation}
	   J_{m}^* \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C, \label{eqn:lower_bound}  
	\end{equation}
	where $C$ is a positive constant (please see Lemma. 1 from \cite{alessandri2008moving}). Next, the upper bound on $J_{m}^*$ is defined. We can write
	{\tiny
	\begin{eqnarray}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 =&& \nonumber\\
	    \lVert [z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E})] - [z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,&&\\
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2  \leq&& \nonumber\\ 2 \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 + 2 \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2,&& \\
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2  \geq&& \nonumber \\ \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2.&&
	\end{eqnarray}
}
	From (\ref{eqn:lower_bound}), we can write
	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(X_{m-N_E}^o)] \rVert^2 < C.
	\end{equation}
	Hence, we obtain
	{\scriptsize	\begin{equation}
	    \lVert z_{m-N_E} - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 \geq \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}) \rVert^2 - C. \nonumber
	\end{equation}}
	By using a similar procedure, we can write
		{\scriptsize
	\begin{equation}
	    \lVert X_{m-N_E}^* - \hat{X}_{m-N_E} \rVert^2 \geq \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E} \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2. \nonumber
	\end{equation}}
	Now the upper bound can be defined as
	\begin{eqnarray}
	    J_{m}^* &\geq& \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \nonumber \\&&\frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \nonumber \\
&&	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C. \label{eqn:upper_bound}
	\end{eqnarray}
	Now, by combining the bounds (\ref{eqn:lower_bound}) and (\ref{eqn:upper_bound}), and rewriting we get
%	\begin{multline}
%	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 - \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 - C \\ \leq \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + C,
%	\end{multline}
%	which can be written as
{\scriptsize
	\begin{eqnarray}
	    \frac{1}{2} \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 +  \frac{1}{2} \lVert F^{N_E}(X_{m-N_E}^o) -  F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 \nonumber && \\\leq 2 \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert_{\mathbb{P}_{m-N_E}}^2 + 2C.\nonumber
	\end{eqnarray}}
	According to the Remarks \ref{rem:MHE1} and \ref{rem:MHE2}, the above equation can be written as
	{\footnotesize
	\begin{equation*}
	    \lVert F^{N_E}(X_{m-N_E}^o) - F^{N_E}(\hat{X}_{m-N_E}^*) \rVert^2 = \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right),
	\end{equation*}}
	and
	\begin{equation*}
	    \delta \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \phi \left( \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \right).\nonumber
	\end{equation*}
	Now, it is possible to define the bound on the estimation error as
	\begin{equation}
	    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \frac{4p}{p+\delta}\lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 + \frac{4}{p+\delta}C.\nonumber
	\end{equation}
	Using the Lipschitz continuity of $f(\cdot)$, it can be written that
	\begin{equation}
	    \lVert X_{m-N_E}^o - X_{m-N_E}^* \rVert^2 = 2k_f \lVert X_{m-N_E-1}^o - \hat{X}_{m-N_E-1}^* \rVert^2 + 2r_{\mu}.\nonumber
	\end{equation}
Hence,
\begin{equation*}
    \lVert X_{m-N_E}^o - \hat{X}_{m-N_E}^* \rVert^2 \leq \zeta_{m-N_E}.
\end{equation*}
It can also be deduced that if $\zeta_m < \zeta_{m-1}$ and $a(p,\delta)<1$, then $\zeta_m$ tends to $\frac{\beta}{1-a(p,\delta)}$ as $m \longrightarrow +\infty$ (please see Theorem~1 from~\cite{alessandri1999neural}), where $\beta~=~ \left(\frac{c_3}{p+c_2\delta}\right)r_{\mu} $. 	
\end{proof}

The following section presents the derivation of the analytical expression for calculating the covariances using the path information. This result will be later used for predicting covariances for the NMPC cost function.

==> observability.tex <==
\section{Covariance calculation}\label{sec:analysis}
% We show in Theorem.~\ref{thm:covariance} that the covariance of the vehicle states $ p_{ij} $ is proportional to the sum of edges leading to the landmarks as $ p_{ij} = \sum \frac{1}{\epsilon_s} $. Since information matrices can be added together (see the proof for Corollaries \ref{cor:path} and \ref{cor:landmark}), it is possible to combine the split sections of the graph, and hence the analysis carried out for the individual sections can be generalized for the complete graph.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config2.eps}
		\caption{Example configuration of two vehicles and two landmarks.}
		\label{fig:config2}
	\end{figure}

Consider an example configuration of two vehicles (represented by $1$ and $2$) and two landmarks (represented by $a$ and $b$) as shown in Fig.~\ref{fig:config2}(i). For understanding how the paths/connections/measurements from a landmark to a vehicle influence the uncertainty of the vehicle states, we take each landmark separately and analyze one at a time. We start the analysis by considering the section $a-1-2$ of the graph, shown in Fig.~\ref{fig:config2}(ii). The observability matrix for the system can be written as
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 \\
o12 & -o12
\end{bmatrix},
\end{equation}
where $oa1,o12$, and $-o12$ are the derivatives of the measurements with respect to the vehicle states. For example, $oa1$ is the derivative of the measurement between the landmark $a$ and the vehicle-$1$ with respect to the vehicle-$1$. Since there is no measurement between the landmark $a$ and the vehicle-$2$, the corresponding entry is zero. Assuming the measurement covariance matrix $ \Gamma = I $, and zero-mean white Gaussian noise, the observability grammian is defined as $ O^TO $ and the covariance matrix $ P $ is written as %\cite{hinson2014observability,crassidis2004optimal}
\begin{eqnarray}
P &\leq& (O^T\Gamma^{-1}O)^{-1}, \\
&\leq& (O^TO)^{-1},\\
 &\leq& \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2} \\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \label{eq:p2a}
\end{bmatrix}.
\end{eqnarray}
The first element of the $P$ matrix correspond to the vehicle-$1$ connecting to the landmark $a$, hence $oa1$ (let us discard the square and fraction for easy understanding). The element $ \frac{1}{o12^2}+\frac{1}{oa1^2} $ of the $P$ matrix corresponds to the vehicle-$2$. Observing that it is connected to the landmark $a$ through vehicle-$1$, we can see both $oa1$ and $o12$. Next, we consider the section $1-2-b$ of the graph, as shown in Fig.~\ref{fig:config2}(iii). The observability and covariance matrices for the system are written as
\begin{equation}
O = \begin{bmatrix}
0 & ob2 \\
o12 & -o12 
\end{bmatrix},
\end{equation}
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} \\
\frac{1}{ob2^2} & \frac{1}{ob2^2}  \label{eq:p2b}
\end{bmatrix}.
\end{equation}
Vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$, which is clearly resembled in the first element of $P$. Vehicle-$2$ is directly connected to the landmark $b$. Hence, the last element of $P$ contains only $ob2$. 

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config3.eps}
		\caption{Example configuration of three vehicles and two landmarks.}
		\label{fig:config3}
	\end{figure}

Next, we take a configuration involving three vehicles as shown in Fig.~\ref{fig:config3}(i). Consider the section $3-a-1-2$ of the graph, shown in Fig.~\ref{fig:config3}(ii). The observability matrix for this configuration is given by
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 & 0 \\
o12 & -o12 & 0\\
0 & 0 & oa3
\end{bmatrix}.
\label{eq:ob_config3}
\end{equation} 
The covariance matrix $ P $ is given by
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{oa1^2} & \frac{1}{oa1^2}  & 0\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & 0\\
0 & 0 & \frac{1}{oa3^2}  \label{eq:p3a}
\end{bmatrix}.
\end{equation}
The first element of the $P$ matrix contain only $oa1$ since the vehicle-$1$ is directly connected to the landmark $a$. The vehicle-$2$ is connected to the landmark $a$ through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. Since vehicle-$3$ is directly connected to the landmark, the last element of $P$ contains only $oa3$ as expected. Now, let us take the section $1-2-b-3$ of the graph, shown in Fig.~\ref{fig:config3}(iii). The observability and covariance matrices are given by
\begin{equation}
O = \begin{bmatrix}
0 & ob2 & 0 \\
o12 & -o12 & 0 \\
0 & 0 & ob3
\end{bmatrix},
\end{equation}
\begin{equation}
P \leq \begin{bmatrix}
\frac{1}{o12^2}+\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0 \\
\frac{1}{ob2^2} & \frac{1}{ob2^2} & 0\\
0 & 0 & \frac{1}{ob3^2}  \label{eq:p3b}
\end{bmatrix}.
\end{equation}
Vehicle-$2$ and vehicle-$3$ are directly connected to the landmark $b$. Therefore, the corresponding entries in the $P$ matrix contains only $ob2$ and $ob3$. The vehicle-$1$ is connected to the landmark $b$ through vehicle-$2$ and this information is clearly reflected in the first entry of $P$.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config4.eps}
		\caption{Example configuration of four vehicles and two landmarks.}
		\label{fig:config4}
	\end{figure}

We conclude this analysis by taking a configuration with four vehicles and two landmarks as shown in Fig.~\ref{fig:config4}(i). The observability matrix for the sub-configuration with the landmark $a$ and the vehicles $1,2,3,4$, shown in Fig.~\ref{fig:config4}(ii) is given by
\begin{equation}
O = \begin{bmatrix}
oa1 & 0 & 0 & 0 \\
o12 & -o12 & 0 & 0\\
0 & o23 & -o23 & 0\\
0 & o24 & 0 & -o24
\end{bmatrix}.
\end{equation}  
The covariance matrix $ P $ is given by
\begin{equation}
P \leq \begin{bmatrix*}[l]
\frac{1}{oa1^2} & \frac{1}{oa1^2}  &  \frac{1}{oa1^2} & \frac{1}{oa1^2}\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2}\\
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o23^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} \\ 
\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{oa1^2} & \frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{oa1^2}  
\end{bmatrix*}. \label{eq:p4a}
\end{equation}
The vehicle-$1$ is directly connected to the landmark $a$, hence the first element of the $P$ matrix contain only $oa1$. The vehicle-$2$ is connected to the landmark through vehicle-$1$, hence both $oa1$ and $o12$ can be seen in the corresponding entry of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $1$ and $2$, which is reflected in the $P$ matrix by the presence of $o12,o23$, and $oa1$. It is to be noted that the term $o24$ is absent as expected since the vehicle-$4$ is not involved in the path for vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$4$, since it is connected to the landmark through the vehicles $2$ and $1$. The entry contains $o12,o24$, and $oa1$ corresponding to the path $4-2-1-a$. Next, consider the sub-configuration with the landmark $b$, shown in Fig.~\ref{fig:config4}(iii). The observability and covariance matrices for this configuration are given by
\begin{eqnarray}
O &=& \begin{bmatrix}
0 & 0 & 0 & ob4 \\
o12 & -o12 & 0 & 0 \\
0 & o23 & -o23 & 0 \\
0 & o24 & 0 & -o24
\end{bmatrix},\\
P &\leq& \begin{bmatrix*}[l]
\frac{1}{o12^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2}\\
\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{o23^2}+\frac{1}{o24^2}+\frac{1}{ob4^2} & \frac{1}{ob4^2} \\
\frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2} & \frac{1}{ob4^2}
\end{bmatrix*}.   \label{eq:p4b}
\end{eqnarray}
The vehicle-$4$ is directly connected to the landmark $b$, hence the fourth diagonal element of the $P$ matrix contain only $ob4$. The vehicle-$2$ is connected to the landmark through vehicle-$4$, hence both $o24$ and $ob4$ can be seen in the second diagonal element of the $P$ matrix. The vehicle-$3$ is connected to the landmark through the vehicles $2$ and $4$, which is reflected in the third diagonal element of the $P$ matrix by the presence of $o23,024$, and $ob4$. We can see that the term $o12$ is absent as expected since the vehicle-$1$ is not involved in the path for the vehicle-$3$. Similarly, the term $o23$ is not present in the entry for the vehicle-$1$, since it is connected to the landmark through the vehicles $2$ and $4$. The entry contains $o12,o24$, and $ob4$ correspondingly.

	\begin{figure}
		\centering
		\includegraphics[width=8cm]{figs/config5.eps}
		\caption{Notations for a general multi-vehicle-landmark RPMG.}
		\label{fig:config5}
	\end{figure}

For stating the general result for any number of vehicles and landmarks, consider the notations given in Fig.~\ref{fig:config5}. The landmarks are represented using stars, and the vehicles are represented using triangles. All the vehicles are numbered $i,i+1,\ldots,n_v$, landmarks $j,j+1,\ldots,n_l$, edges $\epsilon_s,\epsilon_{s+1},\ldots,\epsilon_{n_e}$, where $i=j=s=1$. The observability vector associated with an edge/measurement is represented using $\epsilon$ with the edge number as subscript for simplicity. For example, the observability vector between landmark-$j$ and vehicle-$i$, $oji$ is represented by $\epsilon_s$. Now, the following theorem for a general RPMG can be stated. 

\begin{theorem}\label{thm:covariance}
The covariance associated with the vehicle-$i$, $i=1,\ldots,n_v$, due to the landmark-$j$, $j=1,\ldots,n_l$, is given by 
\begin{equation}
    p_{ij} = \sum_{s \in \mathcal{S}} \frac{1}{\epsilon_s},
\end{equation}
where $s=1,\ldots,n_e$, $\mathcal{S}$ is the set of edges that forms a path from vehicle-$i$ to the landmark-$j$, $n_v$ is the number of vehicles, $n_l$ is the number of landmarks, and $n_e$ is the number of edges in the RPMG.
\end{theorem}
\begin{proof}
The covariances associated with each vehicle for a two-vehicle-two-landmark configuration is given by equations \eqref{eq:p2a} and \eqref{eq:p2b}, followed by three vehicles in \eqref{eq:p3a} and \eqref{eq:p3b}, and four vehicles in \eqref{eq:p4a} and \eqref{eq:p4b}. The relation given in Theorem~\ref{thm:covariance} is clearly reflected in the elements of the corresponding covariance matrices. The generalization to $n_v$ vehicles and $n_l$ landmarks is straightforward.

The relation can be verified by using contradiction. Consider Fig.~\ref{fig:config3}(ii). Suppose the term/edge $\frac{1}{oa1^2}$ is not present in $p_{2a}$. Then the corresponding $O^TO$ matrix for the system will be
\begin{equation}
	O^TO = \begin{bmatrix}
		\frac{oa1^4}{-o12^2+oa1^2} & \frac{o12^2 oa1^2}{o12^2-oa1^2}  & 0\\
		\frac{o12^2 oa1^2}{o12^2-oa1^2} & \frac{o12^2 oa1^2}{-o12^2+oa1^2} & 0\\
		0 & 0 & \frac{1}{oa3^2}  \label{eq:proof1}
	\end{bmatrix},
\end{equation}
which contradicts with the $O^TO$ matrix derived from equation~ \eqref{eq:ob_config3}, which is 
\begin{equation}
 \begin{bmatrix}
		o12^2+oa1^2 & -o12^2  & 0\\
		-o12^2& o12^2 & 0\\
		0 & 0 & oa3^2  
	\end{bmatrix}.
\label{eq:oto_proof}
\end{equation}
Similarly, if an additional term $\frac{1}{oa3^2}$ is present in $p_{2a}$, the corresponding $O^TO$ matrix for the system will be
\begin{equation}
	O^TO = \begin{bmatrix}
		oa1^2+\frac{o12^2oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2}  & 0\\
		-\frac{o12^2 oa3^2}{o12^2+oa3^2} & \frac{o12^2 oa3^2}{o12^2+oa3^2} & 0\\
		0 & 0 & oa3^2  \label{eq:proof2}
	\end{bmatrix},
\end{equation}
which also contradicts with the $O^TO$ matrix given in~\eqref{eq:oto_proof}.
Hence, the relation given in Theorem~\ref{thm:covariance} is always true.
\end{proof}

The following corollaries can be written from Theorem~\ref{thm:covariance}.

\begin{corollary}\label{cor:path}
If there is more than one path from a landmark to a vehicle, and these paths are numbered from $1$ to $g_{ij}$, where $g_{ij}$ is the total number of paths from the landmark-$j$ to the vehicle-$i$, then the total covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert  p_{ij} \right\rVert  \leq \sum_{\kappa=1}^{g_{ij}} \left\lVert p_{ij}^{\kappa} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_{ij} = \sum_{\kappa=1}^{g_{ij}} p_{ij}^{\kappa},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $p_{ij}^{\kappa}$ is the covariance of the vehicle-$i$ due to the landmark-$j$ considering only the path-$\kappa$.
\end{corollary}

\begin{corollary}\label{cor:landmark}
If there is more than one landmark connected to a vehicle, then the covariance of the vehicle is given by
%\begin{equation}
%   \left\lVert p_i \right\rVert  \leq \sum_{j \in \mathcal{J}} \left\lVert p_{ij} \right\rVert ,
%\end{equation}
\begin{equation}
	 p_i  = \sum_{j \in \mathcal{J}} p_{ij},
\end{equation}
where $i=1,\ldots,n_v$, $j=1,\ldots,n_l$, and $\mathcal{J}$ is the set of landmarks connected to the vehicle-$i$.
\end{corollary}

\begin{proof}
The method to calculate covariances for Corollary~\ref{cor:path} and \ref{cor:landmark} is given in Theorem~\ref{thm:covariance}. The summation is based on the properties of the information matrix given as follows~\cite{fisher,zegers2015fisher} 
% When information matrices are added, the resulting value will be greater than or equal to the sum of values of the individual matrices. That is, information is not lost through addition. 

If $X=(X_1,X_2,\ldots,X_n)$ and $X_1,X_2,\ldots,X_n$ are independent random variables, then $I_X(\alpha)=I_{X_1}(\alpha)+I_{X_2}(\alpha)+\ldots I_{X_n}(\alpha)$, where $I_x(\alpha)$ is the information matrix defined as 
\begin{equation*}
	I_x(\alpha) = E_{\alpha}\left[ \left( \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right) ^2\right] = \mathrm{Var}_{\alpha}\left(  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right).
\end{equation*}
Since \[f(x|\alpha) = \prod_{i=1}^{n}f_i(x_i|\alpha),\] where $f_i(\cdot|\alpha)$ is the pdf of $X_i$,
\begin{eqnarray}
\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f(X|\alpha)\right] &=& \sum_{i=1}^{n}\mathrm{Var}\left[  \frac{\partial}{\partial\alpha}\log f_i(X_i|\alpha)\right], \nonumber \\
I_X(\alpha) &=& \sum_{i=1}^{n}I_{X_i}(\alpha). \nonumber 
\end{eqnarray} 

 Since covariance is the inverse of information, it is possible to find the total covariance associated with each vehicle by adding the components from all the paths and landmarks.
\end{proof}

In the next sub-sections, we show how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements. 
% 	\begin{figure}
% 		\centering
% 		\includegraphics[width=8cm]{figs/config1.eps}
% 		\caption{Example configuration }
% 		\label{fig:config1}
% 	\end{figure}
% Consider an example configuration given in Fig.~\ref{fig:config1}. The vehicles $ 1 $ and $ 2 $ are connected to landmarks $a$ and $b$. The observability matrix for the system can be written as
% \begin{equation}
% O = \begin{bmatrix}
% O1a \\
% O2b \\
% O12
% \end{bmatrix},
% \end{equation}
% where 
% \begin{eqnarray}
% O1a &=& \begin{bmatrix}
% o1a & 0
% \end{bmatrix}, \\
% O2b &=& \begin{bmatrix}
% 0 & o2b
% \end{bmatrix}, \\
% O12 &=& \begin{bmatrix}
% o12 & -o12
% \end{bmatrix}.
% \end{eqnarray}  
% Assuming the measurement covariance matrix $ \Gamma = I $, the observability grammian can be defined as $ O^TO $ and the covariance matrix $ P $ can be found as \cite{hinson2014observability}
% \begin{equation}
% P = (O^TO)^{-1},
% \end{equation}
% which can be written as
% \begin{equation}
% P = \begin{bmatrix}
% P(1,1) & P(1,2) \\
% P(2,1) & P(2,2)
% \end{bmatrix},
% \end{equation}
% where
% %{\tiny
% \begin{eqnarray}
% P(1,1) &=& (o12^2 + o2b^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(1,2) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,1) &=& o12^2/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2), \\
% P(2,2) &=& (o12^2 + o1a^2)/(o12^2 o1a^2 + o12^2 o2b^2 + o1a^2 o2b^2).
% \end{eqnarray}
% %}%
% Looking at the elements of $P$, we can clearly see that the covariance is related to the connection/path. In the next sections, we try to find out how this information can be used to analyze the evolution of covariance in multi-vehicle-landmark systems with range and bearing measurements.   

\subsection{Range measurements}
%	\begin{figure}
%		\centering
%		\includegraphics[width=8cm]{figs/config1.eps}
%		\caption{Example configuration }
%		\label{fig:config1}
%	\end{figure}
Consider the configuration given in Fig.~\ref{fig:config2}(i). The vehicle dynamics are defined as
\begin{eqnarray}
\dot{x}_1 &=& v \cos{\psi_1}, \\
\dot{y}_1 &=& v \sin{\psi_1}, \\
\dot{x}_2 &=& v \cos{\psi_2}, \\
\dot{y}_2 &=& v \sin{\psi_2}, 
\end{eqnarray} 
with range measurements
\begin{eqnarray}
h_{1a} &=& \sqrt{(x_1 - x_a)^2 + (y_1 - y_a)^2}, \\
h_{12} &=& \sqrt{(x_1 - x_2)^2 + (y_1 - y_2)^2}, \\
h_{2b} &=& \sqrt{(x_2 - x_b)^2 + (y_2 - y_b)^2},
\end{eqnarray}
and we derive the observability matrix using the Lie derivatives~ \cite{sharma2011graph}. 

Define 
\begin{equation}
f_L = \begin{bmatrix}
\cos{\psi_1} \\
\sin{\psi_1} \\
\cos{\psi_2} \\
\sin{\psi_2} 
\end{bmatrix},
\end{equation}
and the vehicle dynamics can be represented as
\begin{equation}
\dot{X} = vf_L.
\end{equation}
The gradient of zero\textsuperscript{th} order Lie derivatives are given as
\begin{eqnarray}
H_{1a} &=& \begin{bmatrix}
\frac{x_1 - x_a}{R_{1a}} & \frac{y_1 - y_a}{R_{1a}} & 0 & 0 
\end{bmatrix}, \\
H_{2b} &=& \begin{bmatrix}
& 0 & 0 & \frac{x_2 - x_b}{R_{2b}} & \frac{y_2 - y_b}{R_{2b}}  
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{x_1 - x_2}{R_{12}} & \frac{y_1 - y_2}{R_{12}} & \frac{-(x_1 - x_2)}{R_{12}} & \frac{-(y_1 - y_2)}{R_{12}} 
\end{bmatrix}, \\
\end{eqnarray}
where $R_{(\cdot)} $ is the distance between nodes.
The gradient of first order Lie derivatives are given as
\begin{eqnarray}
\frac{\partial }{\partial X}\left( \frac{\partial h_{1a}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
\frac{(y_1-y_a)^2 C\psi_1 -(x_1-x_a)(y_1-y_a) S\psi_1}{R_{1a}^3} &
 \frac{(x_1-x_a)^2 S\psi_1-(x_1-x_a)(y_1-y_a) C\psi_1}{R_{1a}^3}& 0 & 0 
\end{bmatrix},\nonumber\\
\frac{\partial }{\partial X}\left( \frac{\partial h_{2b}}{\partial X}  \cdot f \right) &=& \begin{bmatrix}
0 & 0 & \frac{(y_2-y_b)^2 C\psi_2 + (-x_2+x_b)(y_2-y_b) S\psi_2}{R_{2b}^3} &
\frac{(x_2-x_b)^2 S\psi_2 + (-y_2+y_b)(x_2-x_b) C\psi_2}{R_{2b}^3} 
\end{bmatrix},\\
\frac{\partial }{\partial X}\left( \frac{\partial h_{12}}{\partial X}  \cdot f \right) &=& 
[\begin{matrix}
\frac{-2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix} 
\frac{2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix}
\frac{2(y_1-y_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}  \\
& & \begin{matrix}
\frac{-2(x_1-x_2) S(\frac{\Delta\psi^-}{2})((x_1-x_2) C(\frac{\Delta\psi^+}{2}) + (y_1-y_2) S(\frac{\Delta\psi^+}{2}))}{R_{12}^3} \end{matrix}],
\end{eqnarray}
where $ \sin $ and $ \cos $ are abbreviated as $S$ and $C$, $ \Delta\psi^- = \psi_1-\psi_2 $, and $ \Delta\psi^+ = \psi_1+\psi_2 $.

Observability matrix is formed by using Lie derivatives up to first order as
\begin{equation}
O = \begin{bmatrix}
\nabla L^0 \\
\nabla L^1
\end{bmatrix},
\end{equation} 
where $L^0$ and $L^1$ are the zero\textsuperscript{th} and first order Lie derivatives respectively. The covariance matrix $P$ is found by inverting $ O^TO $ with the assumption of $\Gamma=I$.

The standard deviation in $x$ direction for the first vehicle can be found by taking the square root of the first element of the $P$ matrix,
\begin{equation}
\sigma_{x_1} = \sqrt{P(1,1)}.
\end{equation} 
Similarly, the standard deviation in the $y$ direction and the combined position uncertainty can be found as
\begin{eqnarray}
\sigma_{y_1} &=& \sqrt{P(2,2)},\\
\sigma_{p_1} &=& \sqrt{\sigma_{x_1}^2 + \sigma_{y_1}^2}.
\end{eqnarray}

Since the derived $P$ matrix is very large with several terms, we consider some simplifying assumptions to formulate an approximate relation. All the distance terms were substituted with a single average value. The resulting relation is given as
\begin{equation}
\sigma_{p_1} = \sqrt{\frac{2}{3}+R_g^2 \csc^2{(\psi_1-\theta_g)}},
\label{eq:s_range}
\end{equation}
where $R_g,\theta_g$ are the average value of distance and LOS angle. It is evident from the relation that the covariance of vehicle depends on the distances from the landmarks and the LOS angles to them. As the distance increases, the covariance also increases. Similarly, $ \sigma_p $ of other vehicles can also be found. 
\subsection{Bearing measurements}\label{sec:b_measurement}
Let's extend the vehicle model to contain three states. The new model is given as
\begin{eqnarray}
\dot{x}_1 &=& v \cos{\psi_1}, \\
\dot{y}_1 &=& v \sin{\psi_1}, \\
\dot{\psi}_1 &=& \omega_1, \\ 
\dot{x}_2 &=& v \cos{\psi_2}, \\
\dot{y}_2 &=& v \sin{\psi_2}, \\
\dot{\psi}_2 &=& \omega_2, 
\end{eqnarray} 
With the same configuration as in Fig.~\ref{fig:config2}(i), define bearing measurement equations as
\begin{eqnarray}
h_{a1} &=& \arctan\left( \frac{y_a-y_1}{x_a-x_1}\right) - \psi_1, \\
h_{b2} &=& \arctan\left( \frac{y_b-y_2}{x_b-x_2}\right) - \psi_2, \\
h_{12} &=& \arctan\left( \frac{y_1-y_2}{x_1-x_2}\right) - \psi_2, \\
h_{21} &=& \arctan\left( \frac{y_2-y_1}{x_2-x_1}\right) - \psi_1, 
\end{eqnarray}
the gradient of zeroth order Lie derivatives are given as
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{-(y_1 - y_a)}{R_{a1}^2} & \frac{x_1 - x_a}{R_{a1}^2} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{-(y_2 - y_b)}{R_{b2}^2} & \frac{x_2 - x_b}{R_{b2}^2} & -1  
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{12}^2} & \frac{x_1 - x_2}{R_{12}^2} & 0 & \frac{y_1 - y_2}{R_{12}^2} & \frac{x_2 - x_1}{R_{12}^2} & -1 
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{y_2 - y_1}{R_{21}^2} & \frac{x_1 - x_2}{R_{21}^2} & -1 & \frac{y_1 - y_2}{R_{21}^2} & \frac{x_2 - x_1}{R_{21}^2} & 0 
\end{bmatrix}, \hspace{6mm}
\end{eqnarray} 
using the geometry, the equations are changed to make it in terms of LOS angles as follows
\begin{eqnarray}
H_{a1} &=& \begin{bmatrix}
\frac{\sin\theta_{a1}}{R_{a1}} & \frac{-\cos\theta_{a1}}{R_{a1}} & -1 & 0 & 0 & 0 
\end{bmatrix}, \\
H_{b2} &=& \begin{bmatrix}
0&0&0&\frac{\sin\theta_{b2}}{R_{b2}} & \frac{-\cos\theta_{b2}}{R_{b2}} & -1 
\end{bmatrix}, \\
H_{12} &=& \begin{bmatrix}
\frac{-\sin\theta_{12}}{R_{12}} & \frac{\cos\theta_{12}}{R_{12}} & 0 & \frac{\sin\theta_{12}}{R_{12}} & \frac{-\cos\theta_{12}}{R_{12}} & -1  
\end{bmatrix}, \hspace{6mm} \\
H_{21} &=& \begin{bmatrix}
\frac{\sin\theta_{21}}{R_{21}} & \frac{-\cos\theta_{21}}{R_{21}} & -1 & \frac{-\sin\theta_{21}}{R_{21}} & \frac{\cos\theta_{21}}{R_{21}} & 0  
\end{bmatrix}. \hspace{6mm}
\end{eqnarray} 
Define 
\begin{equation}
f_v = \begin{bmatrix}
\cos{\psi_1} \\
\sin{\psi_1} \\
0\\
\cos{\psi_2} \\
\sin{\psi_2}\\
0 
\end{bmatrix},
f_{\omega_1} = \begin{bmatrix}
0 \\
0 \\
1\\
0 \\
0\\
0 
\end{bmatrix},
f_{\omega_2} = \begin{bmatrix}
0 \\
0 \\
0\\
0 \\
0\\
1 
\end{bmatrix},
\end{equation}
and the dynamics can be represented as
\begin{equation}
\dot{X} = \begin{bmatrix}
\dot{X}_1 \\
\dot{X}_2
\end{bmatrix}
= f_vv+f_{\omega_1}\omega_1 + f_{\omega_2}\omega_2,
\end{equation}
and a similar procedure to the range measurement case is followed to find the first order Lie derivatives, observability grammian and covariance matrix $P$. The covariance in position of the first vehicle is given by
\begin{equation}
\sigma_{p_1}^2 = \frac{9}{2}R_g^2\left(1+\frac{R_g^2}{2+R_g^2+2\cos(2(\psi_1-\theta_g))} \right)+(R_g^2+R_g^4)\csc^2(\psi_1-\theta_g). 
\label{eq:s_bearing}
\end{equation} 
Similarly, $ \sigma_p $ of other vehicles can also be found.

%\subsection{Results}
%
%\begin{figure}
%	\centering 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_range_new.eps}
%		\caption{}
%		\label{fig:s_range}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/sigma_bearing_new.eps}
%		\caption{}
%		\label{fig:s_bearing}
%	\end{subfigure}\hfil 
%		\caption{Comparison of the calculated and simulated uncertainty values. (a) Simulated and calculated values for the range measurements. (b) Simulated and calculated values for the bearing measurements.}
%		\label{fig:aclos_mpc}
%\end{figure}
%Monte Carlo simulations were carried out with different initial configurations for the range and the bearing measurements using EKF for estimation. The state covariance matrix $ Q $ and the measurement noise covariance matrix $ \Gamma $ for the EKF were selected as
%\begin{equation}
%	Q=\begin{bmatrix}
%	0.01 & 0 & 0 & 0\\
%	0 & 0.01 & 0 & 0\\
%	0 & 0 & 0.01 & 0\\
%	0 & 0 & 0 & 0.01
%	\end{bmatrix},
%	\Gamma=\begin{bmatrix}
%	0.01 & 0 & 0\\
%	0 & 0.01& 0 \\
%	0 & 0 & 0.01
%	\end{bmatrix},
%\end{equation}   
%for the range measurements and
%\begin{equation}
%Q=\begin{bmatrix}
%0.01 & 0 & 0 & 0 & 0 & 0\\
%0 & 0.01 & 0 & 0 & 0 & 0\\
%0 & 0 & 0.0001 & 0 & 0 & 0\\
%0 & 0 & 0 & 0.01 & 0 & 0\\
%0 & 0 & 0 & 0 & 0.01 & 0\\
%0 & 0 & 0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\Gamma=\begin{bmatrix}
%0.0001 & 0 & 0 & 0\\
%0 & 0.0001& 0 & 0 \\
%0 & 0 & 0.0001 & 0\\
%0 & 0 & 0 & 0.0001
%\end{bmatrix},
%\end{equation}
%for the bearing measurements. $\sigma_{p_1}$ values obtained from the estimator and calculated using the equations (\ref{eq:s_range}) and (\ref{eq:s_bearing}) are plotted in Fig.~\ref{fig:s_range} and Fig.~\ref{fig:s_bearing} for range and bearing measurements. It can be seen that the calculated uncertainty increases with increase in average distance, and this trend is also followed by the estimated value. The calculation gives us an upper bound for the covariance of the vehicles.

Next section presents the complete NMPC formulation combining the MHE scheme given in Sec.~\ref{sec:MHE} and the uncertainty results derived from analysis given in Sec.~\ref{sec:analysis}. 

==> results.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
		\caption{$\tau_h=20$\,s}
		\label{fig:h200}
	\end{subfigure}
	
%	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
		\caption{$\tau_h=35$\,s}
		\label{fig:h350}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure}
\subsection{EKF vs calculated sigma values}
A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf150.eps}
		\caption{EKF trajectory.}
		\label{fig:ekf_traj}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/calc150.eps}
		\caption{Calculated trajectory.}
		\label{fig:calc_traj}
	\end{subfigure}\hfil 
	
	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
		\caption{vehicle 1}
		\label{fig:ekf_calc_sigmap1}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
		\caption{vehicle 2}
		\label{fig:ekf_calc_sigmap2}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
		\caption{vehicle 3}
		\label{fig:ekf_calc_sigmap3}
	\end{subfigure}
	\caption{EKF vs calculated sigma values.}
	\label{fig:EKF_calc}
\end{figure} 

\subsection{MHE vs EKF}
The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/EKF_pc.eps}
		\caption{EKF trajectory.}
		\label{fig:ekf_pc}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{figs/MHE_pc.eps}
		\caption{MHE trajectory.}
		\label{fig:mhe_pc}
	\end{subfigure}\hfil 
	
	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp1.eps}
		\caption{Error in position of vehicle 1}
		\label{fig:ekfp1}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp2.eps}
		\caption{Error in position of vehicle 2}
		\label{fig:ekfp2}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/EKFp3.eps}
		\caption{Error in position of vehicle 3}
		\label{fig:ekfp3}
	\end{subfigure}
	\caption{EKF vs MHE.}
	\label{fig:EKF_MHE}
\end{figure}      

\begin{table}
	\centering
	\begin{tabular}{ |c|c|c| } 
		\hline
		& MHE & EKF \\
		\hline
		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
		Time required per iteration (s)  &  1.388   &  1.144   \\
		\hline
	\end{tabular}
	\caption{EKF vs MHE.}
	\label{table:ekf_mhe}
\end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_coop.eps}
		\caption{Trajectory of vehicles with cooperation.}
		\label{fig:multi_c}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_nc1.eps}
		\caption{Trajectory of vehicles without cooperation.}
		\label{fig:multi_nc}
	\end{subfigure}\hfil 
	\caption{Effect of cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}[h]
	\centering 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
		\caption{Example 1.}
		\label{fig:multi10j}
	\end{subfigure}\hfil 
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
		\caption{Example 2.}
		\label{fig:multi10j1}
	\end{subfigure}\hfil 
		\caption{Trajectories of 10 vehicles with NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> results_2c1.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. We use the total path length  and average estimation error as metric for analyzing the performance of the proposed approach. We perform the following analysis (i) effect of horizon length in the NMPC on the path length and estimation error (ii) effect of cooperation  (iii) Comparison with the approach proposed in \cite{manoharan2019nonlinear} and (iv) effect of increasing the number of vehicles in the region 10. Before presenting the analysis, we will describe the simulation setting.

\subsection{Simulation setup}
%Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. 
The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure*}
	\centering 
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
		\caption{$\tau_h=20$\,s}
		\label{fig:h200}
	\end{subfigure}\\
	
%	\medskip
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
		\caption{$\tau_h=35$\,s}
		\label{fig:h350}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=\linewidth]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure*}
% \subsection{EKF vs calculated sigma values}
% A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

% \begin{figure*}
% 	\centering 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf150.eps}
% 		\caption{EKF trajectory.}
% 		\label{fig:ekf_traj}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/calc150.eps}
% 		\caption{Calculated trajectory.}
% 		\label{fig:calc_traj}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
% 		\caption{vehicle 1}
% 		\label{fig:ekf_calc_sigmap1}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
% 		\caption{vehicle 2}
% 		\label{fig:ekf_calc_sigmap2}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
% 		\caption{vehicle 3}
% 		\label{fig:ekf_calc_sigmap3}
% 	\end{subfigure}
% 	\caption{EKF vs calculated sigma values.}
% 	\label{fig:EKF_calc}
% \end{figure*} 

 \subsection{MHE vs EKF}
 The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

 \begin{figure*}[h]
 	\centering 
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKF_pc.eps}
 		\caption{}
 		\label{fig:ekf_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/MHE_pc.eps}
 		\caption{}
 		\label{fig:mhe_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp1.eps}
 		\caption{}
 		\label{fig:ekfp1}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.75cm]{figs/EKFp2.eps}
 		\caption{}
 		\label{fig:ekfp2}
 	\end{subfigure}\hspace{0.2cm}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp3.eps}
 		\caption{}
 		\label{fig:ekfp3}
 	\end{subfigure}
 	\caption{(a) NMPC solution with EKF based estimation (b) NMPC solution with MHE (c) Error in position of vehicle 1 (d) Error in position of vehicle 2  (e)  Error in position of vehicle 3}
 	\label{fig:EKF_MHE}
 \end{figure*}      

% \begin{table}
% 	\centering
% 	\begin{tabular}{ |c|c|c| } 
% 		\hline
% 		& MHE & EKF \\
% 		\hline
% 		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
% 		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
% 		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
% 		Time required per iteration (s)  &  1.388   &  1.144   \\
% 		\hline
% 	\end{tabular}
% 	\caption{EKF vs MHE.}
% 	\label{table:ekf_mhe}
% \end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}
	\centering 
	\includegraphics[width=4.5cm]{figs/multi10_coop.eps}\hspace{-5mm}
	\includegraphics[width=4.5cm]{figs/multi10_nc1.eps}
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_coop.eps}
%		\caption{Trajectory of vehicles with cooperation.}
%		\label{fig:multi_c}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_nc1.eps}
%		\caption{Trajectory of vehicles without cooperation.}
%		\label{fig:multi_nc}
%	\end{subfigure}\hfil 
	\caption{Effect of cooperation. (a) Trajectory of vehicles with cooperation.(b) Trajectory of vehicles without cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}
	\centering 
			\includegraphics[width=4.5cm]{figs/multi10_j.eps}\hspace{-5mm}
					\includegraphics[width=4.5cm]{figs/multi10_j1.eps}
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
%		\caption{Example 1.}
%		\label{fig:multi10j}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
%		\caption{Example 2.}
%		\label{fig:multi10j1}
%	\end{subfigure}\hfil 
		\caption{Examples for 10 vehicles path computed using NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    

==> results_2c2.tex <==
\section{Results and Discussion}\label{sec:results}
Extensive numerical simulations were carried out for validating the proposed scheme using CasADi-Python~\cite{Andersson2019}. Also, the performance of the NMPC--MHE formulation was compared against an EKF formulation from the authors' previous paper~\cite{manoharan2019nonlinear}. The angular velocities of the agents are constrained by $[-\pi/2,\pi/2]$\,rad/s due to the practical considerations on the turn rate of the agents. The value of $\eta$ is selected as 2, and the values of $k$ and $\rho$ are selected as 5 and 0.5, respectively. The weight $W$ was selected as 10000, sensor range of the vehicles, $R_s$ = 50\,m, and $\sigma_c$ = 3\,m. The vehicles have a constant velocity of 5\,m/s. The measurement noise covariance matrix $\Gamma$ is selected as a $n_\Gamma \times n_\Gamma$ matrix with 0.01 in its diagonals, where $n_\Gamma$ is the number of received measurements. The red circles represent the source points, and the green circles represent the goal points. The red 'x' marks represent the landmarks.  
\subsection{Effect of NMPC horizon length}
The horizon length for NMPC should be chosen such that the trade-off between optimality and computation time is balanced. Simulations were carried out to find the effect of horizon length on the trajectories of three vehicles, and the results are shown in Fig.~\ref{fig:sim_horizon}. The prediction horizon $ \tau_h $ was varied from 1\,s to 40\,s, and it can be seen that the paths change from sub-optimal to optimal as the horizon increases. The average computation time required for one NMPC iteration was 0.094\,s for $\tau_h=1$\,s and 22.84\,s for $\tau_h=40$\,s.      
\begin{figure*}
	\centering 
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.25cm]{figs/horizon10_2.eps}
		\caption{$\tau_h=1$\,s}
		\label{fig:h10}
	\end{subfigure}\hspace{2mm}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.5cm]{figs/horizon150_2.eps}
		\caption{$\tau_h=15$\,s}
		\label{fig:h150}
	\end{subfigure}\hspace{2mm}
%	\begin{subfigure}{0.3\textwidth}
%		\includegraphics[width=\linewidth]{figs/horizon200_2.eps}
%		\caption{$\tau_h=20$\,s}
%		\label{fig:h200}
%	\end{subfigure}\\
%	\medskip
	\begin{subfigure}{4.25cm}
		\includegraphics[ width=4.5cm]{figs/horizon250_2.eps}
		\caption{$\tau_h=25$\,s}
		\label{fig:h250}
	\end{subfigure}\hspace{2mm}
%	\begin{subfigure}{0.3\textwidth}
%		\includegraphics[width=\linewidth]{figs/horizon350_2.eps}
%		\caption{$\tau_h=35$\,s}
%		\label{fig:h350}
%	\end{subfigure}
	\begin{subfigure}{4.25cm}
		\includegraphics[width=4.5cm]{figs/horizon400_2.eps}
		\caption{$\tau_h=40$\,s}
		\label{fig:h400}
	\end{subfigure}
	\caption{Effect of horizon length.}
	\label{fig:sim_horizon}
\end{figure*}
% \subsection{EKF vs calculated sigma values}
% A comparison between sigma values obtained from EKF and calculated using the derived equation (\ref{eq:s_bearing}) was performed to see the difference in computation time requirement and the behavior of the vehicles. It was seen that the trajectories of the vehicles were similar for EKF and calculated values, with the EKF performing three times slower than the derived result. The trajectories and the standard deviations in the position of the vehicles are given in Fig.~\ref{fig:EKF_calc}. The calculated sigma values show a similar pattern to that obtained from the EKF. The calculated sigma values become singular at some points, but it is not an issue of concern since it is a theoretical upper bound. The EKF took an average of 0.616\,s per iteration, whereas the calculation using the derived equation needed only 0.219\,s.  

% \begin{figure*}
% 	\centering 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf150.eps}
% 		\caption{EKF trajectory.}
% 		\label{fig:ekf_traj}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.4\textwidth}
% 		\includegraphics[width=\linewidth]{figs/calc150.eps}
% 		\caption{Calculated trajectory.}
% 		\label{fig:calc_traj}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap1.eps}
% 		\caption{vehicle 1}
% 		\label{fig:ekf_calc_sigmap1}
% 	\end{subfigure}
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap2.eps}
% 		\caption{vehicle 2}
% 		\label{fig:ekf_calc_sigmap2}
% 	\end{subfigure}\hfil 
% 	\begin{subfigure}{0.3\textwidth}
% 		\includegraphics[width=\linewidth]{figs/ekf_calc_sigmap3.eps}
% 		\caption{vehicle 3}
% 		\label{fig:ekf_calc_sigmap3}
% 	\end{subfigure}
% 	\caption{EKF vs calculated sigma values.}
% 	\label{fig:EKF_calc}
% \end{figure*} 

 \subsection{MHE vs EKF}
 The performance of the MHE estimator was compared against a standard EKF formulation to validate the superiority of the proposed scheme. The horizon length for MHE was selected as $ N_e=20 $, and all other initial parameters are taken the same for the MHE and the EKF. The estimated trajectories of the vehicles, true trajectories, and the errors in position for both the MHE and the EKF are given in Fig.~\ref{fig:EKF_MHE}. It can be seen that the estimation errors are less for the MHE, and it is also more stable compared to the EKF. The mean square error (MSE) values and the computation time requirement are given in Table.~\ref{table:ekf_mhe}. 

 \begin{figure*}
 	\centering 
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKF_pc.eps}
 		\caption{}
 		\label{fig:ekf_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/MHE_pc.eps}
 		\caption{}
 		\label{fig:mhe_pc}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp1.eps}
 		\caption{}
 		\label{fig:ekfp1}
 	\end{subfigure}
 	\begin{subfigure}{3.5cm}
		\includegraphics[width=3.75cm]{figs/EKFp2.eps}
 		\caption{}
 		\label{fig:ekfp2}
 	\end{subfigure}\hspace{0.2cm}
 	\begin{subfigure}{3.5cm}
 		\includegraphics[width=3.5cm]{figs/EKFp3.eps}
 		\caption{}
 		\label{fig:ekfp3}
 	\end{subfigure}
 	\caption{(a) NMPC solution with EKF based estimation (b) NMPC solution with MHE (c) Error in position of vehicle 1 (d) Error in position of vehicle 2  (e)  Error in position of vehicle 3}
 	\label{fig:EKF_MHE}
 \end{figure*}      

% \begin{table}
% 	\centering
% 	\begin{tabular}{ |c|c|c| } 
% 		\hline
% 		& MHE & EKF \\
% 		\hline
% 		MSE of vehicle 1 (m) & 0.45 & 0.46 \\
% 		MSE of vehicle 2 (m) & 0.50 & 1.08 \\
% 		MSE of vehicle 3 (m)  &  0.50   &  0.95   \\
% 		Time required per iteration (s)  &  1.388   &  1.144   \\
% 		\hline
% 	\end{tabular}
% 	\caption{EKF vs MHE.}
% 	\label{table:ekf_mhe}
% \end{table}

\subsection{Effect of cooperation}
A specific configuration of landmarks, initial points, and goal points was created to see the effect of cooperative localization of vehicles. Two simulations were carried out with five vehicles, in which one scenario involved cooperative vehicles and the other without cooperation. NMPC prediction horizon was selected as $\tau_h$=15\,s, and the vehicles have a sensor range of 30\,m. The trajectories taken by the vehicles in both the cases are shown in Fig.~\ref{fig:multi_coop}. It can be seen from Fig.~\ref{fig:multi_c} that the vehicles with cooperation took a shorter path since they used adjacent vehicles for localization, whereas the non-cooperative vehicles took a longer path to go near the landmarks for localization, as shown in Fig.~\ref{fig:multi_nc}. The estimation errors are a bit high for the cooperative case due to the mutual localization of the vehicles.  

\begin{figure}
	\centering 
	\includegraphics[width=4.3cm]{figs/multi10_coop.eps}
	\includegraphics[width=4.3cm]{figs/multi10_nc1.eps}
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_coop.eps}
%		\caption{Trajectory of vehicles with cooperation.}
%		\label{fig:multi_c}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.25\textwidth}
%		\includegraphics[width=3cm]{figs/multi10_nc1.eps}
%		\caption{Trajectory of vehicles without cooperation.}
%		\label{fig:multi_nc}
%	\end{subfigure}\hfil 
	\caption{Effect of cooperation. (a) Trajectory of vehicles with cooperation.(b) Trajectory of vehicles without cooperation.}
	\label{fig:multi_coop}
\end{figure} 

\subsection{10 vehicles}
To test the performance of the scheme for larger systems, a scenario involving ten vehicles was considered. Multiple simulations were carried out with random configurations of the landmarks, initial positions, and goal points. Two example results are shown in Fig.~\ref{fig:multi10}. It can be seen that the estimator performance was satisfactory since the actual states and the estimated states are well aligned for all ten vehicles.

\begin{figure}
	\centering 
			\includegraphics[width=4.3cm]{figs/multi10_j.eps}
					\includegraphics[width=4.3cm]{figs/multi10_j1.eps}
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j.eps}
%		\caption{Example 1.}
%		\label{fig:multi10j}
%	\end{subfigure}\hfil 
%	\begin{subfigure}{0.5\textwidth}
%		\includegraphics[width=\linewidth]{figs/multi10_j1.eps}
%		\caption{Example 2.}
%		\label{fig:multi10j1}
%	\end{subfigure}\hfil 
		\caption{Examples for 10 vehicles path computed using NMPC-MHE scheme.}
		\label{fig:multi10}
\end{figure}    
